Zero-Sum Stochastic Stackelberg Games

Zero-sum stochastic games have found important applications in a variety of fields, from machine learning to economics. Work on this model has primarily focused on the computation of Nash equilibrium due to its effectiveness in solving adversarial board and video games. Unfortunately, a Nash equilibrium is not guaranteed to exist in zero-sum stochastic games when the payoffs at each state are not convex-concave in the players' actions. A Stackelberg equilibrium, however, is guaranteed to exist. Consequently, in this paper, we study zero-sum stochastic Stackelberg games. Going beyond known existence results for (non-stationary) Stackelberg equilibria, we prove the existence of recursive (i.e., Markov perfect) Stackelberg equilibria (recSE) in these games, provide necessary and sufficient conditions for a policy profile to be a recSE, and show that recSE can be computed in (weakly) polynomial time via value iteration. Finally, we show that zero-sum stochastic Stackelberg games can model the problem of pricing and allocating goods across agents and time. More specifically, we propose a zero-sum stochastic Stackelberg game whose recSE correspond to the recursive competitive equilibria of a large class of stochastic Fisher markets. We close with a series of experiments that showcase how our methodology can be used to solve the consumption-savings problem in stochastic Fisher markets.

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/abstract.tex <==
\begin{abstract}
    Zero-sum stochastic games have found important applications in a variety of fields, from machine learning to economics. Work on this model has primarily focused on the computation of Nash equilibrium due to its effectiveness in solving adversarial board and video games. Unfortunately, a Nash equilibrium is not guaranteed to exist in zero-sum stochastic games when the payoffs at each state are not convex-concave in the players' actions. A Stackelberg equilibrium, however, is guaranteed to exist. Consequently, in this paper, we study zero-sum stochastic Stackelberg games. Going beyond known existence results for (non-stationary) Stackelberg equilibria, we prove the existence of recursive (i.e., Markov perfect) Stackelberg equilibria (recSE) in these games, provide necessary and sufficient conditions for a policy profile to be a recSE, and show that recSE can be computed in (weakly) polynomial time via value iteration. Finally, we show that zero-sum stochastic Stackelberg games can model the problem of pricing and allocating goods across agents and time. More specifically, we propose a zero-sum stochastic Stackelberg game whose recSE correspond to the recursive competitive equilibria of a large class of stochastic Fisher markets. We close with a series of experiments that showcase how our methodology can be used to solve the consumption-savings problem in stochastic Fisher markets.
\end{abstract}



==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/ack.tex <==
\begin{ack}
This work was supported by NSF Grant CMMI-1761546.
\end{ack}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/arrowdebreu.tex <==



\section{Arrow-Debreu Exchange Markets as Generalized Stackelberg Games}

In this section, we show that any competitive equilibrium of an Arrow-Debreu Markets are instances of Stackelberg games. An \mydef{Arrow-Debreu Exchange economy} $(\numbuyers, \numgoods, \util, \consendow)$ is a barter economy where a finite set of $\numbuyers$ traders, trade a finite set of $\numgoods$ goods. Every trader $\buyer \in \buyers$ is characterized by a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$, and an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$. For ease of notation, we denote $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and $\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. An instance of an Arrow-Debreu market is given by a tuple $(\numbuyers, \numgoods, \consumptions, \util, \consendow)$. When clear from context, we abbreviate $(\util, \consendow)$.

An \mydef{allocation} $\allocation \in \consumptions$ is a map from goods to buyers, represented as a matrix, s.t. $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$. We define a \mydef{price space} $\pricespace = \left\{ \price \ | \ \ \price[\good] \geq 0, \ \sum_{\good = 1}^{\numgoods} \price[\good] = 1 \right\}$.  Goods are assigned \mydef{prices} $\price \in \pricespace$. 
An outcome of the model is a tuple $\left( \allocation, \price \right) \in \consumptions \times \pricespace$.


A tuple $\left(\allocation^*, \price^* \right) \in \consumptions \times \pricespace$ consisting of allocations and prices respectively is a \mydef{competitive equilibrium} iff 1.~ traders maximize their utility over their \mydef{budget set}, i.e., for all $\buyer \in \buyers$  $\allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, and 2.~ the markets for each good clears and goods that are not entirely cleared are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ (\mydef{feasibility condition}) and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$ (\mydef{Walras' law}).

We formulate a Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ where:
%
\begin{align}\label{eq:stackelberg_arrow_debreu_game1}
    \util[\price](\price, \allocation) &= \sum_{\good \in \goods}  \min \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\
    \util[\allocation](\price, \allocation) &= \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
    \constr(\price, \allocation) &= \consendow \price - \allocation \price\label{eq:stackelberg_arrow_debreu_game3}
    % \\\pricespace = \pricespace \cap \{\sum_{\buyer \in \buyers} \bu \}
\end{align} 
%
\noindent
whose set of Stackelberg equilibria is equal to the set of Arrow-Debreu equilbria $(\util, \consendow)$ of a corresponding market. We note that for ease of exposition, we restrict ourselves to the Arrow-Debreu exchange market but the Stackelberg game we propose can easily be extended to Arrow-Debreu production economies by adding to the payoff function of the inner player, the profits of the firms, as well as the associated production constraints to the function $\constr$.

\begin{assumption}\label{assum:arrow_debreu}
Suppose that for all $\buyer \in \buyers$, 
1.~$\util[\buyer]$ is a continuous, and concave utility function representing locally non-satiated preferences,
2.~$\consumptions[\buyer]$ is non-empty, compact, and convex, 
3.~and that there exists an interior point for each consumer's utility maximization problem, i.e., $\exists \allocation \in \consumptions$ s.t. $\allocation[\buyer] \cdot \price < \consendow[\buyer] \cdot \price$
\end{assumption}

Before introducing the main theorems regarding this Stackelberg game, we introduce some important lemmas. First, we note that a Stackelberg equilibrium is guaranteed to exist in this game.

\begin{lemma}
Under \Cref{assum:arrow_debreu}, the set of Stackelberg equilibria of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ as defined in \Crefrange{eq:stackelberg_arrow_debreu_game1}{eq:stackelberg_arrow_debreu_game3} is non-empty and compact.\deni{Make sure the compactness theorem is correct}
\end{lemma}
\begin{proof}
    Since the $\min$ and $\max$ operators preserve continuity, $\util[\price]$ is also continuous. Additionally, under \Cref{assum:arrow_debreu}, $\util[\allocation]$ is also continuous since it is a sum of continuous functions and $\consumptions$ is non-empty and compact since it is a product of non-empty and compact sets. Finally, since $\constr$ is continuous, and $\pricespace$ is non-empty and compact, by \Cref{thm:exitence_stackelberg} a Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is guaranteed to exist.
\end{proof}

The following lemma states important properties of the inner player's Stackelberg equilibrium strategies.
\begin{lemma}\label{lemma:inner_arrow_debreu_optimality}
Consider the solution to the inner player's optimization problem $\allocation^* \in \argmax_{\allocation \in \consumptions: \allocation \price^* \leq \consendow \price^*} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])$ for the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ given an arbitrary strategy of the outer player $\price^*$. Suppose that \Cref{assum:arrow_debreu} holds, then $\allocation^*$ is optimal for the outer player iff we have that for all buyers $\buyer \in \buyers$:

1.~ $\allocation[\buyer]^*$ is a utility maximizing allocation over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, 
% i.e., $\allocation[\buyer]^* \in \argmax_{\allocation[ ]\in \consumptions[\buyer] : \allocation[ ] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \util[\buyer](\allocation[ ])$, and
2.~ $\allocation[\buyer]^*$ consumes the entire budget of consumer $\buyer$, i.e., $\allocation[\buyer]^* \cdot \price^* = \consendow[\buyer] \cdot \price^*$.
\end{lemma}
\begin{proof}

Consider the inner player's optimization problem for the Stackelberg equilibrium strategy of the outer player $\price^*$ $\max_{\allocation \in \consumptions: \allocation \price^* \leq \consendow \price^*} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])$. By the assumption of existence of an interior point in the budget set of all consumers, Slater's condition is satisfied for the inner player's problem, and there exists KKT multlipliers $\bm \lambda^* \in \R^\numbuyers_+$ which satisfy the necessary and sufficient KKT conditions. From the first order optimality conditions, we have:
\begin{align}
    \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \util[\allocation](\allocation) \right]_{\allocation = \allocation^*} + \sum_{\buyer \in \buyers} \lambda^*_\buyer \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \constr[\buyer](\price^*, \allocation[\buyer])\right]_{\allocation = \allocation^*} &\doteq 0 && \forall \buyer \in \buyers, \good \in \goods\\
    \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\right]_{\allocation = \allocation^*} + \sum_{\buyer \in \buyers} \lambda^*_\buyer \frac{\partial }{\partial \allocation[\buyer][\good]}  \left[ \consendow[\buyer] \cdot \price^* - \allocation[\buyer] \cdot \price^*\right]_{\allocation[\buyer] = \allocation[\buyer]^*} &= 0  && \forall \buyer \in \buyers, \good \in \goods\\
    \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]} \right]_{\allocation[\buyer] = \allocation[\buyer]^*}- \lambda^*_\buyer \price[\good]^* &= 0  && \forall \buyer \in \buyers, \good \in \goods\\
    \lambda^*_\buyer &= \frac{\left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer] = \allocation[\buyer]^*}}{\price[\good]^*} && \forall \buyer \in \buyers, \good \in \goods
\end{align}
where the last line is the equimarginal principle and implies that for all $\buyer \in \buyers$  $\allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$. 
% Hence, $(\price^*, \allocation^*)$ satisfies the first condition of being a competitive equilibrium.

Similarly, from the KKT necessary and sufficient complementarity conditions, we have that for all $\buyer \in \buyers$:
\begin{align}
    \lambda_\buyer^* \constr[\buyer](\price^*, \allocation[\buyer]^*) = 0\\
    \lambda_\buyer^* \left(\consendow[\buyer] \cdot \price^* - \allocation[\buyer]^* \cdot \price^* \right) = 0
\end{align}
It is well-known that for all traders $\buyer \in \buyers$, $\lambda^*$ corresponds to the marginal utility of money, i.e, the derivative of the indirect utility function of buyer $\buyer$ w.r.t. their budget. Since the utility function of each trader is locally non-satiated, we must have that $\lambda_\buyer^* > 0$, which gives us:
%
\begin{align}
    \left(\consendow[\buyer] \cdot \price^* - \allocation[\buyer]^* \cdot \price^* \right) = 0\\
    \price^* \cdot\left(\consendow[\buyer]  - \allocation[\buyer]^*  \right) = 0\label{eq:lower_level_walras_law}
\end{align}
% Summing over all the buyers, we obtain that $(\price^*, \allocation^*)$ satisfies the second part of the second condition to be a competitive equilibrium.
\end{proof}


\begin{lemma}\label{lemma:outer_player_max_utility_arrow_debreu}
The utility achieved by the outer player in the game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is upper bounded by 0 for any feasible strategy profile $(\price, \allocation)$, i.e.,  $\util[\price](\price, \allocation) \leq 0$ for all $(\price, \allocation) \in \pricespace \times \left\{ \allocation \ | \ \ \allocation \in \consumptions \ \ \allocation  \price^* \leq \consendow \price^*  \right\}$.
\end{lemma}
\begin{proof}
\begin{align}
    \util[\price](\price^*, \allocation^*) &= \sum_{\good \in \goods}  \min \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\
    &\leq 0 - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\ 
    &\leq - \sum_{\good \in \goods}  \price[\good] \cdot (0) \\
    &= 0
\end{align}
\deni{Make sure to add that $\price$ is feasible so  equation 16 holds.}
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_price_zero}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. Then, at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ if for any $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$.
\end{lemma}

\begin{proof}
For notational clarity, define the excess supply function associated with an optimistic best-response of the inner player $\s(\price) = \sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price)$ where: 
\begin{align}
\calD^*(\price) &= \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) &\in \argmax_{\allocation \in \calD^*(\price)} \left\{ \sum_{\good \in \goods}  \min \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) - \sum_{\good \in \goods}  \price[\good] \max \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) \right\}
\end{align}
% For the sake of contradiction, suppose that $\util[\price](\price^*, \allocation*) < 0$. Then, there must exist a set of good $\calG$ such that for all $k \in \calG$ either $s_k(\price^*) < 0$ or  $s_k(\price^*) > 0$ and $\price[k] > 0$.
By the necessary optimality conditions for the outer player's Stackelberg equilibrium strategy over the set $\pricespace$ \cite{} \deni{Cite Dempe theorem 5.6} we have:

\begin{align}
     \subdiff[{\price[\good]}] \util[\price](\price^*, \allocation^*(\price^*)) &\doteq 0\\
    \sum_{\good \in \goods} \subdiff[{\price[\good]}]\left( \min \left\{ s_\good(\price^*), 0 \right\}\right) - \max\left\{ s_\good(\price^*), 0\right\} - \sum_{\good \in \goods} \price[\good] \subdiff[{\price[\good]}] \max\left\{ s_\good(\price^*), 0\right\} &= 0
\end{align}\deni{note: above $\subdiff[{\price[\good]}]$ is the generalized Clark derivative, which is a generalization of subgradients.}
Suppose that $s_\good(\price^*) > 0$, the above condition then reduces to:
\begin{align}
    \sum_{\good \in \goods} \subdiff[{\price[\good]}] (0)  - s_\good(\price^*) - \sum_{\good \in \goods} \price[\good]  \subdiff[{\price[\good]}] s_\good(\price^*) = 0\\
    - s_\good(\price^*) - \sum_{\good \in \goods} \price[\good]  \subdiff[{\price[\good]}] s_\good(\price^*) = 0\\
    - s_\good(\price^*) + \sum_{\good \in \goods} \price[\good] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good](\price^*) = 0
\end{align}

\noindent
For the above equation to be true it must be that either $\price[\good] = 0$ or 
\begin{align}
    \price[\good] &> 0\\
      \sum_{\good \in \goods} \price[\good]  \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}]  \allocation[\buyer][\good](\price^*) &= s_\good(\price^*) \enspace .\label{eq:case2_price_zero_excess_supply}
\end{align} 

We will show that the later case occuring is a contradiction.

\noindent
Recall from \Cref{lemma:outer_player_max_utility_arrow_debreu} that for any $\price \in \pricespace$:
\begin{align}
    \sum_{k \in \goods} \allocation[\buyer][k]^*(\price) \price[k] = \sum_{k \in \goods} \consendow[\buyer][k] \price[k]
\end{align}
Taking the generalized Clarke derivative of both sides, we obtain:
\begin{align}
    \allocation[\buyer][\good]^*(\price) + \sum_{k \in \goods} \price[k] \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) = \consendow[\buyer][\good]
\end{align}
Re-organizing expressions and summing over all $\buyer \in \buyers$, we obtain:
\begin{align}
   \sum_{k \in \goods}\price[k] \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) =  \consendow[\buyer][\good] - \allocation[\buyer][\good]^*(\price) \\
    \sum_{k \in \goods} \price[k] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) =  \sum_{\buyer \in \buyers}\consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price)
\end{align}
Note that we have $\sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good]^*(\price)  = \subdiff[{\price[\good]}] s_\good(\price)$ by the definition of $\s$. Hence, we can re-write the above as:
\begin{align}
    \sum_{\good \in \goods} \price[\good] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good]^*(\price)  = s_\good(\price) 
\end{align}
which is in contradiction with \Cref{eq:case2_price_zero_excess_supply} and the assumption that $s_\good > 0$ implying that if $s_\good(\price^*) > 0$, we must have $\price[\good] = 0$.
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_feasible}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. Then, at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ then, for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$.
\end{lemma}

\begin{proof}
For notational clarity, let $\excessdemand(\price) = \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price)$ where: 
\begin{align}
\calD^*(\price) &= \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) &\in \argmax_{\allocation \in \calD^*(\price)} \left\{ \sum_{\good \in \goods}  \min \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) - \sum_{\good \in \goods}  \price[\good] \max \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) \right\}
\end{align}
Suppose for contradiction, that there exists a maximal set of goods $\calG \subset \goods$ such that for all $\good \in \calG$ $\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* = - \excessdemand[\good](\price^*) < 0$ or equivalently $\excessdemand[\good](\price^*) > 0$. Recall by \Cref{lemma:outer_player_max_utility_arrow_debreu} we have for any $\price \in \pricespace$:
\begin{align}
    \sum_{\good \in \goods} \price[\good]^* \left(\allocation[\buyer][\good]^* - \consendow[\buyer][\good] \right) = 0 && \forall \buyer \in \buyers
\end{align}
Summing up over all $\buyer \in \buyers$, we obtain Walras' law:
\begin{align}
    \sum_{\good \in \goods} \sum_{\buyer \in \buyers} \price[\good]^* \left(\allocation[\buyer][\good]^* - \consendow[\buyer][\good] \right) = 0 \\
    \sum_{\good \in \goods} \price[\good] \excessdemand[\good](\price^*) = 0 \\
    \sum_{\good \in \calG} \price[\good] \excessdemand[\good](\price^*) + \sum_{\good \in (\goods - \calG)} \price[\good] \excessdemand[\good](\price^*) = 0 \\
\end{align}
Note that by \Cref{lemma:stackelberg_arrow_debreu_price_zero}, we have that $\sum_{\good \in (\goods - \calG)} \price[\good] \excessdemand[\good](\price^*) = 0$ where $(\goods - \calG) \subset \goods$ is the set of good such that for all $\good \in (\goods - \calG), \excessdemand[\good](\price^*) \leq 0$.
\begin{align}
    \sum_{\good \in \calG} \price[\good] \excessdemand[\good](\price^*) = 0 
\end{align}
which is a contradiction. 
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_value}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. The payoff of the outer player at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is 0, i.e., $\util[\price](\price^*, \allocation^*) = 0$. Additionally, a strategy of the outer player $\price^*$ is Stackelberg equilibrium strategy for $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ iff 
1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$.
\end{lemma}

\begin{proof}
Combining \Cref{lemma:stackelberg_arrow_debreu_feasible} and \Cref{lemma:stackelberg_arrow_debreu_price_zero} we see that . For the other direction, we note that $\util[\price](\price^*, \allocation^*) = 0$. Additionally, this also means that if 1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then the utility of the outer player is $0$, which means that $\price^*$ is a Stackelberg equilibrium strategy.

To obtain the other direction, we simply note that $\util[\price](\allocation^*, \price^*)  = 0$, which is only possible if 1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, which
\end{proof}

\begin{theorem}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. 
Any competitive equilibrium $(\allocation^*, \price^*)$ of the Arrow-Debreu Market $(\util, \consendow)$ is also a Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$. 
% \deni{Need the outer player's action set to be the intersection of the prices space and prices that satisfy walras' law.}
\end{theorem}
% \deni{Need some Slater like condition \`a la Arrow-Debreu}

\begin{proof}

(Set of Arrow-Debreu Equilibria  $\subseteq$ Set of Stackelberg equilibria):

Let $(\allocation^*, \price^*)$ be an Arrow-Debreu equilibrium of  $(\consendow, \util)$, then the by the feasibility requirement of a competitive equilibrium, we have that for all $\good \in \goods$: $\sum_{\buyer \in \buyers} \allocation[\buyer][\good] - \sum_{\buyer \in \buyers}  \consendow[\buyer][\good] \leq 0$ or equivalently $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good] \geq 0$. Additionally, by Walras' law we know that $\price \cdot \left(\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer] \geq 0 \right) = 0$. Combining these two facts, we must have that $\util[\price](\allocation^*, \price^*) = 0$. Since the payoff of the outer player at s Stackelberg equilibrium is $0$ (\Cref{lemma:stackelberg_arrow_debreu_value}), we must have that $\price^*$ is a Stackelberg equilibrium strategy for the outer player. Additionally, since $\allocation^*$ is utility maximizing constrained by budget and Walras' law is satisfied by \Cref{lemma:inner_arrow_debreu_optimality} we have that $\allocation^*$ is a best-response of the inner player for $\price^*$. Hence, $(\price^*, \allocation^*)$ is a Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$.  
 
\noindent
(Set of Stackelberg equilibria  $\subseteq$ Set of Arrow-Debreu Equilibria):

Let $(\price^*, \allocation^*)$ be Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$, then by \Cref{lemma:stackelberg_arrow_debreu_value} the second condition of a competitive equilibrium is fullfilled. Additionally, by \Cref{lemma:inner_arrow_debreu_optimality} $\allocation^*$ is the budget constrained utility maximizing allocation associated with with $\price^*$, fulfilling the first condition of a competitive equilibrium. Hence, $(\price^*, \allocation^*)$ is a competitive equilibrium.






\if 0

Suppose the following:
\begin{align}
\calD^*(\price) = \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) \in \argmax_{\allocation \in \calD^*(\price)} - \sum_{\good \in \goods} (\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price))^2
\end{align}
 The necessary optimality condition for the outer player's Stackelberg equilibirium strategy, is given by the first order optimality condition for $\max_{\price \in \pricespace}- \frac{1}{2} \left\|\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer](\price)\right\|_2^2$. 
%  $\allocation[\buyer][\good]^*(\price) \in \argmax_{\allocation \in D(\price)} - \sum_{\good \in \goods} (\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price))^2$, that is:
\begin{align}
    \frac{\partial }{\partial \price[\good]} \left( - \frac{1}{2} \left\|\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer]\right\|_2^2\right) &\doteq 0 && \forall \good \in \goods\\
    \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) &= 0  && \forall \good \in \goods\\
    % \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) \price[\good] &= 0  && \forall \good \in \goods
    % \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]}\right) &= 0
\end{align}
% Summing the above for all goods $\good \in \goods$, we obtain:
% \begin{align}
%     \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \sum_{\good \in \goods}\left( \sum_{\buyer \in \buyers} \price[\good] \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) &= 0\\
% \end{align}
If $\sum_{\good \in \good} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*) = 0$ or if $ \sum_{\good \in \good} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*) = 0$ \emph{and} $\sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = 0$, then the first part of the second condition for a competitive equilibrium is satisfied. We are left to check that if we only have $\sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = 0$, the good must be not demanded.
Suppose that $\left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price)}{\partial \price[\good]}\right) > 0$,   the good is not demanded by any buyer, in which case 

\fi 
\end{proof}

\subsection{Recursive Arrow-Debreu Markets}


A \mydef{recursive Arrow-Debreu Exchange market} consists of:
\begin{enumerate}
    \item A set of states $\states$, describing the state in which the market is.
    \item A initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
    \item A transition function $\trans: \states \times \states \times \R_+^\numgoods \times \R_+^{\numgoods \times \numbuyers} \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when prices $\price \in  \R_+^{\numgoods} $ and allocations $\allocation \in  \R_+^{\numgoods \times \numbuyers} $ are determined by the supply and demand sides respectively, is denoted by $\trans(\state^\prime \mid \price, \allocation)$.
    \item A set of $\numgoods$ goods.
    \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
    \begin{enumerate}
        \item a continuous and concave utility function $\util[\buyer]: \states \times \R^\numgoods \to \R$
        \item an endowment at each state $\consendow[\buyer]: \states \to \R_+$
    \end{enumerate}
    \item a probability $\discount$ that the market will continue
\end{enumerate}

A recursive Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \states, \initstates, \util, \budget, \supply, \discount)$. When clear from context, we simply write $(\states, \initstates, \util, \budget, \discount)$.

An \mydef{allocation} $\allocation \in \R^{\numbuyers \times \numgoods}_+$ is a mapping from buyers to goods such that $\allocation[\buyer][\good] \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$.
%
An \mydef{allocation system} $\allocation: \states \to \R^{\numbuyers \times \numgoods}$ is a mapping from states to allocations of goods to buyers such that $\allocation[\buyer][\good](\state) \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$ in state $\state$. 
%
Goods are assigned anonymous \mydef{prices} $\price \in \R_+^\numgoods$ such that $\price[\good] \geq 0 $ denotes the cost of one unit of good $\good$ for any buyer.
%
A \mydef{price system} is a mapping $\price: \states \to \R^\numgoods_+$ from states to prices such that for all $\good \in \goods$ and $\state \in \states$, $\price[\good](\state) \geq 0$ denotes the price of good $\good$ in state $\state$.
A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \price^*)$. which consists of an allocation system and a price system such that:
\begin{enumerate}
    \item The buyers are expected utility maximizing: 
    \begin{align}
        \forall \buyer,\;\allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \R^{\numgoods \times \states} : \forall \state \in \states \allocation[\buyer](\state) \cdot \price(\state) \leq \consendow[\buyer](\state) \cdot \price(\state)} \E \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer](\staterv[\iter])) \right]
    \end{align}
    \item The market clears in each state and goods that are unallocated in each state are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\state \in \states$:
    \begin{align}
        \price[\good](\state) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good](\state) = \sum_{\buyer \in \buyers} \consendow[\buyer][\good]\\
        \price[\good](\state) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good](\state) \leq \sum_{\buyer \in \buyers} \consendow[\buyer][\good]
    \end{align}
\end{enumerate}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/checklist.tex <==
% \section{Submission of papers to NeurIPS 2022}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Appendix A}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, details are discussed in conclusion, and experiments sections.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Assumptions are summarized in \Cref{assum:main}}
        \item Did you include complete proofs of all theoretical results? 
    \answerYes{Yes, all proofs can be found in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, code repo can be found here: \coderepo.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details can be found in section 5 and Appendix E.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For experiments run multiple times, i.e., zero-sum convex constraints, exploitability always reached zero, and there was hence no error to report in all randomly initialized examples.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details can be found in Appendix E.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Details can be found in Appendix E.}
  \item Did you mention the license of the assets?
    \answerYes{Details can be found in Appendix E.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/conclusion.tex <==
\section{Conclusion}

In this paper, we proved the existence of recursive Stackelberg equilibria in zero-sum stochastic Stackelberg games, provided necessary and sufficient conditions for a policy profile to be a recursive Stackelberg equilibrium, and showed that a Stackelberg equilibrium can be computed in (weakly) polynomial time via value iteration.
%\sdeni{Further, we provided a characterization of recursive competitive equilibria in stochastic Fisher markets with savings, as they are an instance of zero-sum stochastic Stackelberg games.}{}
%recursive Stackelberg equilibria coincide with recursive competitive equilibria in stochastic Fisher markets
We then showed how these results can be applied to solve for the recursive competitive equilibria of a stochastic Fisher market with savings, by constructing a zero-sum stochastic Stackelberg game whose recursive Stackelberg equilibria are recursive competitive equilibria of the market.
Finally, we applied this methodology to solve several markets experimentally.
%used value iteration together with nested GDA to solve these markets.

Future work in this space could try using deep reinforcement learning methods to learn better (i.e., nonlinear) representations of the value functions.
%\amy{does this idea apply to both markets, with and without savings?}\deni{Yes, to both settings!}\amy{but the next sentence only applies with savings?}\deni{Yes}
It is also conceivable that deep reinforcement learning methods would be able to learn policies that scale up to larger markets than those considered here, as convergence of neural networks to globally optimal solutions has been observed empirically, even in highly non-convex problems \cite{li2018visualizing}, suggesting that they could potentially overcome the difficulties that first-order methods face in the presence of non-smoothness and non-concavity. 
Finally, our experimental results, in which our methods succeed at solving zero-sum \emph{convex-non-concave\/} stochastic Stackelberg games, suggest the need for and possibility of theoretical advances solving convex-non-concave min-max optimization problems, as little is understood beyond non-convex-concave domains.

%\deni{Add a few sentences on theoretical lack of explanation on convex-non-concave problems vs. non-convex-concave}

%\amy{i think we should rewrite this sentence saying something about Leontief markets specifically.} 

% \deni{Directions: Convex regression, and improve Leontief with deep learning, let transitions depend on allocations.}


==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/experiments.tex <==
\section{Experiments}
\label{sec:expts}

The zero-sum stochastic Stackelberg game associated with a stochastic Fisher market, can, in theory, be solved via value iteration (\Cref{alg:value_iter_fisher}), assuming one can perform a one-step backup operation of the corresponding Bellman equations (Equation~\ref{eq:fisher_bellman}), i.e., solve the min-max optimization problem given in Line 4 of \Cref{alg:value_iter_fisher}.
The $\sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer], \type[\buyer]))$ term renders the objective function in this min-max optimization problem convex-\emph{non}-concave.
As a result, known (first-order) methods, e.g., nested gradient descent ascent (GDA) \cite{goktas2021minmax}, are not guaranteed to find a globally optimal solution;
%to this min-max optimization problem, and instead may only converge to a locally optimal solution
and without a globally optimal solution to the inner optimization problem, our value iteration convergence guarantees (\Cref{thm:existence_stackelberg}) do not hold.
Still, gradient methods have been observed to escape local solutions in many non-convex optimization problems (e.g., \cite{jin2017escape, du2017gradient}), leading us to investigate the extent to which \Cref{alg:value_iter_fisher} can solve stochastic Fisher markets with savings using nested GDA \cite{goktas2021minmax} as a subroutine to solve the inner optimization problem.
%in other words, how effectively value iteration (\Cref{alg:value_iter_fisher}) using nested GDA \cite{goktas2021minmax} as a subroutine performs in this application.

\begin{algorithm}[H]
\caption{Value Iteration for Stochastic Fisher Market}
\label{alg:value_iter_fisher}
\begin{algorithmic}[1]
\State Initialize $\statevalue[0]$ arbitrarily, e.g. $\statevalue[0]=\zeros$
\For{$k = 1, \hdots, \numiters_{\statevalue}$}
        \State For all states $\state \in \states$, $\displaystyle
        \statevalue[k+1] (\type, \budget, \supply) = $ \\ $\min\limits_{\price \geq \zeros} \max\limits_{(\allocation, \saving) \geq \zeros: \allocation \price + \saving \leq \budget} \left\{
        \sum\limits_{\good \in \goods} \supply[\good] \price[\good] + \sum\limits_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer], \type[\buyer])) 
         + \discount \mathop{\E} \left[\statevalue[k][](\type^\prime, \budget^\prime + \saving, \supply^\prime) \right] \right\}$
\EndFor
\end{algorithmic}
\end{algorithm}

We attempted to compute the recursive competitive equilibria of three different classes of stochastic Fisher markets with savings.%
\footnote{Our code can be found \href{\rawcoderepo}{here}, and details of our experimental setup can be found in \Cref{sec_app:experiments}.}
%the zero-sum stochastic Stackelberg game associated with Fisher markets.
Specifically, we created markets with three classes of utility functions, each of which endowed the state-value function with different smoothness properties.
Let $\type[\buyer] \in \R^\numgoods$ be a vector of parameters, i.e., a \mydef{type}, that describes the utility function of buyer $\buyer \in \buyers$.
%, i.e., $\type[\buyer]$ is the type of player $\buyer$.
We considered the following (standard) utility function classes:
1.~\mydef{linear}: $\util[\buyer](\allocation[\buyer]) = \sum_{\good \in \goods} \type[\buyer][\good] \allocation[\buyer][\good]$; 2.~\mydef{Cobb-Douglas}:  $\util[\buyer](\allocation[\buyer]) = \prod_{\good \in \goods} \allocation[\buyer][\good]^{\type[\buyer][\good]}$; and 3.~\mydef{Leontief}:  $\util[\buyer](\allocation[\buyer]) = \min_{\good \in \goods} \left\{ \frac{\allocation[\buyer][\good]}{\type[\buyer][\good]}\right\}$. 
%\sadie{Maybe we should unite the language of ``class" here with the language of ``type".}\amy{type is okay.}

% We initialized a stochastic Fisher market with $\numbuyers = 2$ buyers and $\numgoods = 5$ goods. To simplify the analysis, we assumed deterministic transitions such that the buyers do not get new budgets at each time period, and their types/valuations as well as the supply of goods does not change at each state, i.e., the type/valuation space and supply space has cardinality 1. This reduced the market to a deterministic repeated market setting in which the amount of budget saved by the buyers differentiates different states of the market. To initialize the state space of the market, we first fixed a range of $[10,50]^\numgoods$ for the buyers' valuations and drew for all buyers $\buyer \in \buyers$ valuations $\type[\buyer]$ from that range uniformly at random at the beginning of the experiment. We have assumed the supply of goods is $\ones[\numgoods]$ and that the budget space was $[0,1]^\numbuyers$. This means that our state space for our experiments was $\states = \{ (\type[1], \type[2])\} \times \{ \ones[\numgoods] \} \times [0, 1]^\numbuyers$. We note that although the assumption that buyers valuations/type space has cardinality one does simplify the problem, the supply of the goods being $\ones$ at each state is wlog because goods are divisible and the allocation of goods to buyers at each state can then be interpreted as the percentage of a particular good allocated to a buyer. We assumed initial budgets of $\budget[][0] = \ones[\numbuyers]$ for both buyers. 

% In particular, we assumed that the value function had a linear form at each state such that $\statevalue(\type, \budget, \supply; \a, c) = \a^T\budget + c$ for some parameters $\a \in \R^\numbuyers, c \in \R$, and we tried to approximate the value function at the next step of value iteration by using linear regression. That is, at each value iteration step, we uniformly sampled 25 budget vectors from the range $[0,1]^\numbuyers$. Next, for each sampled budget $\budget$, we solved the min-max step given that budget as a state. This process gave us (budget, value) pairs on which we ran linear regression to approximate the value function at the next iterate. 

% We first modeled a stochastic Fisher market \emph{without\/} savings, where buyers' budgets are replenished
% %\amy{the state is the budget. in the without savings case, a new influx of money arrives at each state.}
% at each state.
% %\amy{add description of A-D market}
% To this end, we assumed that each buyer owned a good sold in the market, with their budget in the next time period proportional to the amount of money spent during the current time period on their good.
%\amy{Note that this model falls outside the scope of our theory, as transitions depend on allocations!} \amy{as per our meeting on 7/22, this turns out to be false. Sadie observed that there is really only one state in this model; since the market always clears, everyone spends all. upshot: these experiments were a useful sanity check, but we are going to delete them.} \sadie{Commented out the no saving case}
% In this case, we solve the min-max operator \amy{???} using \mydef{max-oracle gradient descent (GD)} with an exact max-oracle (\cite{goktas2021minmax}; \Cref{alg:max_oracle_on_qfunc_no_saving}).

%\deni{two setups: small markets+no interest rate as sanity check and big markets+probabilistic interest rate.}

We ran two different experiments.
First, we modeled a small stochastic Fisher market with savings \emph{without\/} interest rates.
In this setting, buyers' budgets, which are initialized at the start of the game, persist across states, and are replenished by a constant amount with each state transition.
Thus, the buyers' budgets from one state to the next are deterministic.
%\amy{is there any stochasticity at all? do buyer preferences change from one state to another, for example?} \deni{In this first experiment, there is no stochasticity at all!}

Second, we modeled a larger stochastic Fisher market with savings and probabilistic interest rates.
In this model, although buyers' savings persist across states, they are nondeterministic, as they increase or decrease based on the random movements of an interest rate with each state transition. 
More specifically, we chose five different equiprobable interest rates (0.9, 1.0, 1.1, 1.2, and 1.5) to provide buyers with more incentive to save as compared to the model without interest rates.

Since budgets are a part of the state space in stochastic Fisher markets, the state space is continuous; so we attempted to estimate the value function using linear regression, with a uniform sample of state and min-max value pairs (e.g., \cite{boyan1994generalization}).
% \amy{how was the sampling done? where did we get the particular set of pairs we used?}
To compute the min-max value at each sampled state, 
%i.e., the solution to the optimization problem in line 4 of \Cref{alg:value_iter_fisher}, 
we used nested GDA \cite{goktas2021minmax}, which, in this application, repeatedly takes a step of gradient descent on the prices followed by a loop of gradient ascent on the allocations and savings (\Cref{alg:nested_gda_on_qfunc}).
The requisite gradients were computing via auto-differentiation using JAX \cite{jax2018github}, for which we observed better numerical stability than analytically derived gradients, as can often be the case \cite{Griewank2012NumericalStability}.

%\amy{and why didn't simulated annealing work? you can add some anecdotal info about simulated annealing if you want, as well.}
%\sdeni{}{We also tried using 0th order heuristic methods, e.g., simulated annealing \cite{bertsimas1993simulated},  to compute min-max values, but they also proved numerically unstable.}
% \ssadie{}{As we states above, value iteration requires solving the min-max optimization problem in \Cref{eq:fisher_bellman} iteratively, and we attempted to do so through nested GDA at each iteration. In specific, }

% \amy{explain nested GDA in more detail here. explain that it requires taking the gradient of the value function wrt the demands-savings tuple (what is that?) in the inner loop.}
% \samy{}{We used JAX to compute these gradients, as it provides better numerical stability \cite{Griewank2012NumericalStability}.}\amy{better than what?}

%the value function is also continuous \amy{hmmm...i read a ``continuous state space'' as the opposite of a discrete one. but not all functions on continuous state spaces are continuous,}\sadie{I think we want to assert that the value function has continuous domain?}\amy{we already assert that. we say ``since the state space is continuous,''. my question is about the second part. why does that imply that the value function is also continuous?} in stochastic Fisher markets.

% For both methods, we have run value iteration for $30$ iterations. We ran nested GDA with learning rates $\learnrate[\allocation] = 0.5$, $\learnrate[\price] = 0.02$ for linear, $\learnrate[\allocation] = 0.5$, $\learnrate[\price] = 0.01$ for leontief, and $\learnrate[\allocation] = 0.5$, $\learnrate[\price] = 0.0005$ for Cobb-Douglas. We also ran max-oracle gradient descent with a learning rate of $\learnrate[\price] = 0.5$. The outer loop of nested GDA was run for $\numiters_{\price} = 30$ iterations, while its inner loop was run for $\numiters_{\allocation} = 100$ iterations, and the max-oracle gradient descent algorithm was run for $\numiters_{\price} = 30$ iterations. We depict the trajectory of the average value of the value function at each iteration of value iteration, under nested GDA in \Cref{fig:nested_gda_qfunc},  and under max-oracle gradient descent in \Cref{fig:maxoracle_qfunc}.

% We observe that even though nested GDA is not guaranteed to compute a global Stackelberg equilibrium at each iteration of value iteration, value iteration seems to converge. The same holds true for max-oracle gradient descent. However, since nested GDA might compute less optimal solution, we observe that value iteration under nested GDA converges to a value function with a lower average value, which makes sense due to the non-concavity of the optimization problem in $\saving$. 

In both experiments, to check whether the optimal value function was found, we measured the exploitability of the market, meaning the distance between the recCE computed and the actual recCE.
To do so, we checked two conditions:
1) whether each buyer's expected utility was maximized at the computed allocation and savings, at the prices outputted by the algorithm, and 2) whether the market always cleared.
In both settings, we extracted the greedy policy from the value function computed by value iteration, and unrolled it across time to obtain the greedy actions
% \sadie{Need to rephrase here}
$({\allocation}^{(\iter)}, {\saving}^{(\iter)},  {\price}^{(\iter)})$ at each state $\state[\iter]$.
% where the state is parameterized by  $\budget^{(\iter)}=\budget^{(\iter-1)}-{\saving}^{(\iter-1)}$ ($\budget^{(1)}=\ones[\numbuyers]$), $\supply^{(\iter)} = \ones[\numgoods]$, and $\type[]^{(\iter)}=\type[]$ is the fixed valuations we used to train our value function
We then computed the cumulative utility of these allocation and savings, i.e., for all $\buyer \in \buyers$, $\estutil[\buyer] \doteq \sum_{\iter=0}^{\numiters} \discount^\iter\util[\buyer](\allocation[\buyer]^{(\iter)})$.
% $(\util[1],\util[2])=\sum_{\iter=0}^{\numiters} \discount^\iter(\util[1](\allocation[1]^{(\iter)}),\util[2](\allocation[2]^{(\iter)}))$
We compared these values to the expected maximum utility $\util[i]^*$,
%for each buyer $i \in \buyers$,
given the prices and the other buyers' allocations 
%\amy{and savings? or do one buyer not care about the other buyers' savings? i guess not.} 
computed by our algorithm.
%We computed $\util[\buyer]^*$ by directly maximizing \sdeni{against other buyers in the without savings case and by solving the consumption/savings problem in the with savings case}{the cumulative utility of buyer $\buyer$, given the other buyers' policies.},\amy{isn't the direct solution just a special case of solving the consumption/savings problem? do we need to specify that we use a direct solution in the former case?}\sadie{They are slightly different as the direct solution involves action of other buyers but consumption/saving problem doesn't}\amy{that sounds very different. how can the consumption/savings problem not involve the actions of the other buyers? i would think you need to know the other buyers' demands in both cases. if not, i don't think i understand the consumption/saving problem. where is this problem defined in the paper?}\deni{What we have done is really the above. Would you agree Sadie? I think this covers both cases.}\amy{it does Deni, but it doesn't say anything more than the sentence before it. we were trying to give more detail about HOW we solved this problem, in each case.}
We report the normalized distance between these two values, $\estutil[\buyer]$ and $\util[i]^*$, which we call the \mydef{normalized distance to utility maximization (UM)}.
For example, in the case of two buyers, the normalized distance to UM $=\frac{||(\estutil[1],\estutil[2])-(\util[1]^\star,\util[2]^\star)||_2}{||(\util[1]^*,\util[2]^*)||_2}$.
Finally, we also measured excess demand, which we took as the \mydef{distance to market clearance (MC)}, i.e.,  $\frac{1}{\numiters}\sum_{\iter=1}^{ \numiters} ||\sum_{\buyer \in \buyers}\allocation[\buyer]^{(\iter)} - \supply[][\iter]||_2$.
% All norms are Euclidean.

In the experiment with smaller markets and without interest rates, \Cref{fig:avg_values_small} depicts the average value of the value function across a sample of states as it varies with time, and \Cref{table:exploitability_small} records the exploitability of the recCE found by \Cref{alg:value_iter_fisher}with nested GDA.
For all three class of utility functions, not only do the value functions converge, exploitability is also sufficiently minimized, as all the buyer utilities are maximized and the market always clears. 
% \samy{}{These results are exactly as our theory predicts, as these problems are convex-concave.}
% \amy{what about dependence in the transitions on allocations?}
% \amy{actually, why is Cobb Douglas still worse than the others?}

\begin{figure}[t]
\begin{subfigure}[h]{0.4\linewidth}
\vspace{0cm}
\centering
\includegraphics[width=50mm]{graphs/avg_values_small.png}
\captionof{figure}{Average values across budgets.}
%under Nested GDA.
\label{fig:avg_values_small}
\end{subfigure}\hfill
\begin{subfigure}[h]{0.55\linewidth}
\vspace{0cm}
\centering
\begin{tabular}{|c|c|c|} 
\hline
\begin{tabular}[c]{@{}c@{}}Utility \\Class\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distance to UM \end{tabular} & \begin{tabular}[c]{@{}c@{}}Distance to MC \end{tabular}  \\ 
\hline
% \hline
Linear & $0.011$   & $0.010$                                                             \\ 
\hline
Leontief &$0.056$  & $0.010$                                                                \\ 
\hline
Cobb-Douglas& $0.006$   & $0.010$                                                                \\
\hline
\end{tabular}
    \caption{Exploitability of recCE found by \Cref{alg:value_iter_fisher} with nested GDA in stochastic Fisher markets with savings but without interest rates.}
    \label{table:exploitability_small}
\end{subfigure}
\caption{Stochastic Fisher markets with savings but without interest rates.}
\end{figure}

%\amy{We observed that max-oracle GD with simulated annealing outperformed nested GDA, more often finding a global maximum for the inner player.}

In the experiment with larger markets and probabilistic interest rates (\Cref{fig:avg_values_big}, \Cref{table:exploitability_big}), in linear and Cobb-Douglas markets, the value functions converge, and exploitability is sufficiently minimized.
In Leontief markets, however, although the value function converges and the markets almost clear, the buyers' utilities are not fully maximized; instead, the cumulative utilities obtained are less than half of their expected maximum utilities.
The difficulty in this case likely arises from the fact that the Leontief utility function is not differentiable, so the min-max optimization problem for Leontief markets is neither smooth nor convex-concave, making it difficult, if not impossible, for nested GDA to find even a stationary point,
%of the Bellman equations in Line 4 of \Cref{alg:value_iter_fisher}, 
since gradient ascent is not guaranteed to converge to a stationary point of a function that is non-convex-non-smooth \cite{jordan2022complexity}.

% We can remedy this situation by computing allocations that maximize the buyers' utilities at the near-clearing prices output by the algorithm, which leads to perfect utility maximization (zero normalized distance to UM).
% These allocations, however, result in prices that are slightly farther from clearing (distance to MC of 0.11) than the aforementioned near-clearing prices (distance to MC of 0.08). 

\begin{figure}[t]
\begin{subfigure}[h]{0.4\linewidth}
\vspace{0cm}
\centering
\includegraphics[width=50mm]{graphs/avg_values_big_ir.png}
\captionof{figure}{Average values across budgets.}
%under Nested GDA.
\label{fig:avg_values_big}
\end{subfigure}\hfill
\begin{subfigure}[h]{0.55\linewidth}
\vspace{0cm}
\centering
\begin{tabular}{|c|c|c|} 
\hline
\begin{tabular}[c]{@{}c@{}}Utility \\Class\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distance to UM \end{tabular} & \begin{tabular}[c]{@{}c@{}}Distance to MC \end{tabular}  \\ 
\hline
Linear & $0.040$   & $0.009$                                                             \\ 
\hline
Leontief &$0.463$  & $0.009$                                                                \\ 
\hline
Cobb-Douglas& $0.017$   & $0.009$     \\
\hline
\end{tabular}
    \caption{Exploitability of recCE found by \Cref{alg:value_iter_fisher} with nested GDA in stochastic Fisher markets with savings and probabilistic interest rates.}
    \label{table:exploitability_big}
\end{subfigure}
\caption{Stochastic Fisher markets with savings and probabilistic interest rates.}
\end{figure}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/fisher.tex <==
\section{Recursive Market Equilibrium}
\label{sec:fisher}

We now introduce 
% move on to show 
an application of zero-sum stochastic Stackelberg games, which generalizes a well known market model, the Fisher market \cite{brainard2000compute}, to a dynamic setting in which buyers not only participate in markets across time, but their wealth persists. 
% We characterize market equilibrium in this model via a recursive min-max optimization problem (with dependent strategy sets) and hence provides a constructive proof of existence. We note that to the best of our knowledge, there do not even exists proofs of existence of market equilibria when saving is possible in markets with heterogeneous agents. 
A \mydef{(one-shot) Fisher market} consists of $\numbuyers$ buyers and $\numgoods$ divisible goods \cite{brainard2000compute}.
Each buyer $\buyer \in \buyers$ is endowed with a budget $\budget[\buyer] \in \budgetspace[\buyer] \subseteq \mathbb{R}_{+}$ and a utility function $\util[\buyer]: \mathbb{R}_{+}^{\numgoods} \times \typespace[\buyer] \to \mathbb{R}$, which is parameterized by a type $\type[\buyer] \in \typespace[\buyer]$ that defines a preference relation over the consumption space $\R^\numgoods_+$.
% \amy{you should introduce types here, if it is types that define utility functions!}
% \footnote{\sdeni{WLOG, we assume that all budgets are strictly positive; otherwise, we could remove a buyer with a zero budget without affecting the equilibrium.}{}} 
%As is standard in the literature, we assume that there is one divisible unit of each good in the market.
Each good is characterized by a supply $\supply[\good] \in \supplyspace[\good] \subset \R_+$.


An instance of a Fisher market is then a tuple $\calM \doteq (\numbuyers, \numgoods, \util, \type, \budget, \supply)$, where $\util = \left\{\util[1], \hdots, \util[\numbuyers] \right\}$ is a set of utility functions, one per buyer,
%\amy{why do you need utility functions in this market spec if you have types?}\deni{Type for me is the valuations that parameterize for instance linear utilities, utility functions are the actual form, i.e., they \amy{the utility functions?} describe whether if we have linear, CD, or Leontief utilities, then the type describes the utility function's parameters.} \sadie{I think in the static Fisher market model, we assumed that different buyers may have different class (linear, leontief, cd, or so) of utility, while type gives the specific valuations. That is, $u_i\in \{linear, leontief, cd\}$, while $t_i$ is some array of coefficients? But I thought the name ``type" is a little misleading, and maybe ``valuation" or ``coefficient" is more straight forward?}
$\budget \in \R_{+}^{\numbuyers}$ is the vector of buyer budgets, and $\supply \in \R_{+}^{\numgoods}$ is the vector of supplies.
When clear from context, we simply denote $\calM$
%$(\numbuyers, \numgoods, \util, \type, \budget, \supply)$ 
by $(\type, \budget, \supply)$.

Given a Fisher market $(\type, \budget, \supply)$, an \mydef{allocation} $\allocation = \left(\allocation[1], \hdots, \allocation[\numbuyers] \right)^T \in \R_+^{\numbuyers \times \numgoods}$ is a map from goods to buyers, represented as a matrix, s.t. $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$. Goods are assigned \mydef{prices} $\price = \left(\price[1], \hdots, \price[\numgoods] \right)^T \in \mathbb{R}_+^{\numgoods}$. A tuple $(\allocation^*, \price^*)$ is said to be a \mydef{competitive equilibrium (CE)} \cite{arrow-debreu, walras} if 
1.~buyers are utility maximizing, constrained by their budget, i.e., $\forall \buyer \in \buyers, \allocation[\buyer]^* \in \argmax_{\allocation[ ] : \allocation[ ] \cdot \price^* \leq \budget[\buyer]} \util[\buyer](\allocation[ ], \type[\buyer])$;
and 2.~the market clears, i.e., $\forall \good \in \goods,  \price[\good]^* > 0 \Rightarrow \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* = \supply[\good]$ and $\price[\good]^* = 0 \Rightarrow\sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* \leq \supply[\good]$.

% \amy{move to appendix!}
%\samy{We denote the type space of all buyers $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$, and the space of all possible budgets for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$. We denote the set of all goods' possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$.}{}\deni{This should not be removed, it is used in the appendix, and is also our state space, it's important!}\amy{if it is not used in the main body, just define it in the appendix. if you want to use it here, it goes above the previous paragraph so you can then say $(t,b,q) \in T \times B \times Q$.}

\if 0
A \mydef{stochastic Fisher market} is a dynamic market in which each state corresponds to a static Fisher market: i.e., each state $\state \in \states$ is \sdeni{characterized by}{defined as} a tuple $\state \doteq (\type, \budget, \supply)$.
% \sadie{this notation here means, in the Stochastic Fisher market model for each state, 1. utility function is not changing, but valuations may change (that is $\type$); 2. budgets may change; 3. supplies may change.  But how they will change exactly is describe by the specific transition function. In our experiments, for example, we only travel to states with the same type $\type$ and supplies $\supply$, and the budgets is changing. }
%%% SPACE
%$\in \typespace \times \budgetspace \times \supplyspace$.
%%% SPACE
%\footnote{We often refer to a tuple of types, budgets, and supplies $(\type, \budget, \supply)$ by a state variable $\state$ with the same superscripts, e.g., $(\type^\prime, \budget^\prime, \supply^\prime) = \state^\prime$.}
In each state, the buyers choose their allocations $\allocation = \left(\allocation[1], \hdots, \allocation[\numbuyers] \right)^T \in \R_+^{\numbuyers \times \numgoods}$ and the market determines prices, after which the market terminates with probability $(1-\discount)$, or it moves into a new state $\state^\prime$ with probability $\discount \trans(\state^\prime \mid \state, \allocation)$.
\fi

A \mydef{stochastic Fisher market with savings} is a dynamic market in which each state corresponds to a static Fisher market: i.e., each state $\state \in \states = \typespace \times \budgetspace \times \supplyspace$ is characterized by a tuple $\state \doteq (\type, \budget, \supply)$.
The market is initialized at state $\staterv[0] \sim \initstates$, and for each state $\staterv[\iter] \in \states$ encountered at time step $\iter \in \N_+$, the market determines the prices $\price[][\iter]$ of the goods, while the buyers choose their allocations $\allocation[][][\iter]$ and set aside some \mydef{savings} $\saving[\buyer][\iter] \in [0, \budget[\buyer]]$ to potentially spend at some future state.
Once allocations, savings, and prices have been determined, the market terminates with probability $1-\discount$, or it transitions to a new state $\staterv[\iter + 1] = \state^\prime$ with probability $\discount \trans(\state^\prime \mid \state, \saving)$, depending on the buyers' saving decisions.%
\footnote{In our model, which is consistent with the literature~\cite{romer2012advanced} 1.~prices do not determine the next state since market prices are set by a ``fictional auctioneer,'' not an actual market participant; 2.~allocations do not determine the next state.
Only savings, which are forward-looking decisions, affect future states---budgets, specifically.}
We denote a stochastic Fisher market by $\fishermkt[0] \doteq (\numbuyers, \numgoods, \util, \states, \initstates, \trans, \discount)$.

\if 0
A stochastic Fisher market with savings is denoted by 
%a tuple $(\numbuyers, \numgoods, \typespace, \budgetspace, \supplyspace, \util, \budget[][0],  \trans, \discount)$. When clear from context, we simply write 
$(\states, \util, \budget[][0], \trans, \discount)$.
\fi

% At each time step, each good $\good \in \goods$ is supplied in some amount $\supply[\good] \in \supplyspace[\good] \subset \R_+^\numgoods$. We denote the set of all goods' possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$. Each buyer $\buyer \in \buyers$, has some initial budget $\budget[\buyer][0] \in \budgetspace[\buyer] \subset \R_+$, a continuous utility function $\util[\buyer]: \R^\numgoods_+ \times \typespace[\buyer] \to \R_+ $ which is parametrized by a type $\type[\buyer] \in \typespace[\buyer]$ that defines a preference relation over the space of consumption $\R^\numgoods_+$. The buyer's type space $\typespace[\buyer]$ captures what the buyer's preferences might be at each time step and is an intrinsic parameter of the utility function.
% % , and an initial budget $\budget[\buyer][0] \in \budgetspace[\buyer]$ 
  % % coming from a budget space $\budgetspace[\buyer]$
% We denote the type space of all buyers $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$, and the space of all possible budgets for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$. At each time step, the market assumes a state $(\type, \budget, \supply) = \state \in \states = \typespace \times  \budgetspace \times \supplyspace$. 

\if 0
Given a stochastic Fisher market, a \mydef{recursive competitive equilibrium (recCE)} \cite{mehra1977recursive} is a per-state tuple $(\allocation^*, \price^*) \in \R_+^{\numbuyers \times \numgoods} \times  \R_+^{\numgoods}$, meaning allocation and pricing policies, i.e., mappings from states to allocations and prices, s.t.\ 1) the buyers are expected utility maximizing, constrained by their spending constraints, i.e., for all buyers $\buyer \in \buyers$, $\allocation[\buyer]^*$ is the optimal policy that, for all states $(\type, \budget, \supply) \in \states$, solves the Bellman equation $\budgetval[\buyer](\type, \budget, \supply) =$
$$
    %\budgetval[\buyer](\type, \budget, \supply) =
    \max_{\allocation[\buyer] \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\type, \budget, \supply) \leq \budget[\buyer]} \left\{ \util[\buyer]\left(\allocation[\buyer], \type[\buyer]\right) 
    % \\ \notag   & 
    + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply, (\allocation[\buyer], \allocation_{-\buyer}^*(\state))} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime, \supply^\prime) \right] \right\},
$$ 
%for all states $(\type, \budget, \supply) \in \states$ 
where $\allocation^*_{-\buyer}$, $\saving^*_{-\buyer}$ denote the competitive equilibrium allocation and saving policies excluding buyer $\buyer$,
and
2) the market clears in each state so that unallocated goods in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$,
$    
        \price[\good]^*(\type, \budget, \supply) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) = 1
$ and
$
        \price[\good]^*(\type, \budget, \supply) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) \leq 1
$.
\fi

% There exists two equivalent solution concepts for dynamic markets the sequential competitive equilibrium and the recursive competitive equilibrium. Suppose that $(\budget[][\iter], \type[][\iter], \supply[][\iter])_\iter$ is the sequence of states generated according to $\trans(\cdot \mid \state[\iter - 1], \allocation[][][\iter], \saving[][\iter])$ by  $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$. A \mydef{sequential competitive equilibrium} is a sequence of allocation, savings, and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that 1) all buyers are expected utility maximizing constrained by their saving and spending constraints, i.e., for all  $\buyer \in \buyers$, 
% $
%     ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)})_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  (\allocation[\buyer][\iter]), \saving[\buyer][\iter]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] + \saving[\buyer][\iter - 1] 
%     % \\ \budget[\buyer][\iter + 1] = \saving[\buyer][\iter]
%     }\right\}_{\iter = 1}^\infty } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer][][\iter], \type[\buyer][\iter])
% $ where $\type[\buyer][\iter]$, 
% and 2) The market clears in each time period 
% % \samy{and}{meaning}\deni{Not true, that would mean that goods unallocated are priced at zero only if Walras' law and feasibility holds.} 
% goods that are unallocated are priced at 0, i.e., for all $\good \in \goods$ and $\iter \in \N_+$,  if 
% $
%     {\price[\good]^*}^{(\iter)} > 0$ then $\sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = 1$, and if $
%     {\price[\good]^*}^{(\iter)} \geq 0$ then $\sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq 1
% $.

% % \mydef{sequential competitive equilibrium} which is sequence of allocation, saving and price tuples $({\allocation[][][\iter]}^*, {\saving[][\iter]}^* {\price[][\iter]}^*)_{\iter = 0}^\infty$ such that 1.~the buyers are expected utility maximizing constrained by the saving and spending constraint, i.e., for all $\buyer \in \buyers$, $ \{{\allocation[\buyer][][\iter]}^*, {\saving[][\iter]}^* \}_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  {\allocation[\buyer]^*}^{(\iter)} \in \R^{\numgoods}_+: \allocation[\buyer] \cdot {\price[][\iter]}^* + {\saving[][\iter]}^* \leq \budget[\buyer][\iter] }  \right\}_{\iter = 1}^\infty } \mathop{\E}_{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter])} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter])\right]$ 
% % % where $\state[\iter] = (\type[][\iter], \budget[][\iter], \supply[][\iter])$
% % 2.~the market clears in each time period and goods that are unallocated are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\iter \in \N_+$, ${\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = \supply[\good][\iter]$, or $ {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq \supply[\good][\iter]$. Unfortunately, although mathematically interesting, the sequential competitive equilibrium is untractable as it requires the computation of an infinite sequence.

% Note that the sequential competitive equilibrium allocations, savings, and prices at any time period are effectively a function of the state of the market, hence we could define a competitive equilibrium to be a mapping from states to a tuple of allocations, savings, and prices. Overloading notation, we define an \mydef{allocation policy}, $\allocation : \states \to \R_+^{\numbuyers \times \numgoods}$ as a mapping from states to allocations, a \mydef{saving policy} $\saving: \states \to \R_+^\numbuyers$ as a mapping from states to savings, and a \mydef{pricing policiy} $\price: \states \to \R_+^{\numgoods}$ as a mapping from states to prices.
% %




% Define $\budgetval[\buyer]: \states 
% % \times \R^{\states \times \numbuyers \times \numgoods} \times \R^{\states \times \numbuyers} \times \R^{\states \times \numgoods} 
% \to \R$ 
% % \deni{Add parameters to description}:
% \begin{align}
%     \budgetval[\buyer](\type, \budget, \supply
%     % ; \allocation, \saving, \price
%     ) &= 
%     % \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_\iter }
%     \mathop{\E}_{\substack{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter])\\ \state[0] = \state }} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter]\right)\right]\\
%     &= \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) + \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \allocation[][][](\state), \saving[][](\state)) } \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) \saving(\type, \budget, \supply), \supply^\prime; \allocation, \saving, \price) \right]
% \end{align}

% We can then re-express a sequential competitive equilibrium as a recursive competitive equilibrium.

Given a stochastic Fisher market with savings $\fishermkt[0]$
%$(\states, \util, \state[0], \trans, \discount)$, 
a \mydef{recursive competitive equilibrium (recCE)} \cite{mehra1977recursive} is a tuple $(\allocation^*, \saving^*, \price^*) \in \R_+^{\numbuyers \times \numgoods \times \states} \times \R_+^{\numbuyers \times \states} \times \R_+^{\numgoods \times \states}$, which consists of stationary \mydef{allocation}, \mydef{savings}, and \mydef{pricing policies} s.t.\ 1) the buyers are expected utility maximizers, constrained by their savings and spending constraints, i.e., for all buyers $\buyer \in \buyers$, $(\allocation[\buyer]^*, \saving[\buyer]^*)$ is an optimal policy that, for all states $\state \doteq (\type, \budget, \supply) \in \states$, solves the \mydef{consumption-savings problem}, defined by the following Bellman equations: for all $\state \in \states$, $\budgetval[\buyer](\state) =$
$$
    %\budgetval[\buyer](\type, \budget, \supply) =
    \max_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\state) + \saving[\buyer] \leq \budget[\buyer]} \left\{ \util[\buyer]\left(\allocation[\buyer], \type[\buyer]\right) 
    % \\ \notag   & 
    + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \state, (\allocation[\buyer], \allocation_{-\buyer}^*(\state)), (\saving[\buyer], \saving_{-\buyer}^*(\state)))} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + \saving[\buyer], \supply^\prime) \right] \right\},
$$ 
%for all states $(\type, \budget, \supply) \in \states$ 
where $\allocation^*_{-\buyer}$, $\saving^*_{-\buyer}$ denote the 
%competitive equilibrium 
allocation and saving policies excluding buyer $\buyer$; and
2) the market clears in each state so that unallocated goods in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$,
$    
        \price[\good]^*(\state) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\state) = \supply[\good]
$ and
$
        \price[\good]^*(\state) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\state) \leq \supply[\good]
$.
% \samy{By analogy with Markov perfect equilibrium, we can view a}
A recCE is Markov perfect, as it is a CE regardless of initial  state,%
\footnote{Just as any stochastic game can be (non-compactly) represented as a one-shot game, any stochastic Fisher market with savings can be represented as a one-shot Fisher market comprising the same buyers (with utility functions given by their discounted cumulative expected utility) 
% $\Ex_{\staterv[\iter]} \left[\discount^\iter \util[\buyer]\left(\allocation[\buyer][][\iter], \type[\buyer][][\iter]\right) \right]$
\samy{}{and the same goods\deni{saying the same goods is confusing because in the new market you think of the goods at each time step as being seperate good, I like the previous version better.}, enhanced with time-stamps.}
It has been shown that competitive equilibria exist in such markets\cite{prescott1972note}.
In particular, a recCE is a CE in this market; the time stamps ensure that the market clears at every time step, as required.}
%\amy{does whoever writes about the time-stamped construction prove that CE exist in these one-shot markets? also, would a recursive CE of the stochastic Fisher market also be a CE of this one-shot market?}
i.e., buyers are allocated expected discounted cumulative utility-maximizing goods regardless of initial state, and the aggregate demand for each good is equal to its aggregate supply \emph{at all states}.
\amy{why does the qualifier ``starting from any state'', or ``regardless of initial conditions'' apply only to the first half of this sentence and not the second?}\deni{Because the market clearance condition is more robust and holds in every time period. this is because the seller is myopic at recCE; only the buyers are long-term optimizers.}
%\amy{across all mkts encountered? or in expectation?}\deni{Across all markets encountered and demands/supplies are not discounted} \amy{why is it not an expectation? aren't some mkts more likely to be encountered than others?}\deni{Markets should clear independently of likelihood of realization of the market, market clearance is robust condition in this sense.}

% Define the following value function:
% \begin{align}
%     &\statevalue(\type, \budget, \supply; \allocation, \saving, \price) = \sum_{\good \in \goods} \supply[\good] \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](\type, \budget, \supply), \type[\buyer]) + \\ \notag &\discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \statevalue[][](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation, \saving, \price) \right]
% \end{align}

The following theorem establishes that we can build a zero-sum stochastic Stackelberg game whose \recSE{} correspond to the set of recCE of any stochastic Fisher market with savings.
Since \recSE{} are guaranteed to exist, recCE are also guaranteed to exist.
As \recSE, and hence recCE, are independent of the initial market state, we 
%\samy{}{henceforth} \amy{this is weird, since we barely use this notation!}
%\deni{"Note that as \recSE, and hence recCE, are independent of the initial market state, the recCE of stochastic Fisher markets with savings are independent of initial state distributions.} 
denote stochastic Fisher markets with savings by $\fishermkt \doteq (\numbuyers, \numgoods, \util, \states, \trans, \discount)$.

\begin{restatable}{theorem}{thmfishermarketrecursiveeqm}
\label{thm:fisher_market_recursive_eqm}
A stochastic Fisher market with savings $\fishermkt$
%$(\states, \util, \budget[][0], \trans, \discount)$
in which $\util$ is a set of continuous and homogeneous utility functions and the transition function is continuous in $\saving[\buyer]$ has at least one recCE.
Further, the \recSE{}
%$(\allocation^*, \saving^*, \price^*)$
% \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}
that solves the following Bellman equations corresponds to a recCE of $\fishermkt$: 
%\samy{}{for all states $\state \in \states$,}
%$(\states, \util, \budget[][0], \trans, \discount)$
\begin{align} \label{eq:fisher_bellman}
    \forall \state \in \states, \statevalue[][](\state) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times (\numgoods + 1)} : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \supply[\good] \price[\good] 
    + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer], \type[\buyer])) \notag\\ 
    + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \state, 
    % \allocation, 
    \saving)} \left[\statevalue[][](\type^\prime, \budget^\prime + \saving, \supply^\prime) \right]
\end{align} 
% \sadie{\budget^\prime - \saving?}\deni{ok wait, this is important cause I have seen this in your writing but this is not true! Can we get on a quick zoom call?}\sadie{sure!}
% Additionally, any Stackelberg equilibrium corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
\end{restatable}

\amy{the thm states that every recSE is a recCE. are you saying that there may be other recCEs that we do not model/cannot discover?}\deni{Yes, that is correct}

\amy{\begin{remark}
This theorem states that every recSE is a recCE.
But every recCE is not a recSE. \amy{add example!}\deni{The second part of this statement is not necesarrily true, I do not have an example. Happy to think about it another time but this is too time consuming for right now.}
\end{remark}}
 
\begin{remark}
This result cannot be obtained by modifying the Lagrangian formulation,
% \amy{is there an eq'n earlier in the paper to reference here?}\deni{Unfortunately no!}
i.e., the simultaneous-move game form, of the Eisenberg-Gale program, because the inner maximization problem is convex-non-concave, but recursive Nash equilibria 
% \samy{in deterministic \amy{why does deterministic matter here? why not just plain existence?}
are guaranteed to exist in zero-sum stochastic games only under the assumption of convex-concave payoffs \cite{jaskiewicz2018non}.
%%% SPACE, and did not understand 
%Another interesting property of the above stochastic Stackelberg game is that even though it is non-concave in $\saving$, if the optimal value function $\statevalue$ is known, any stationary (not necessarily globally optimal) $\hat{\saving}$ is sufficient to compute a recursive competitive equilibrium. However, it is not clear if value iteration is able to only compute value of $\hat{\saving}$ which are locally optimal. We provide some intuition on this with our experiments.
\end{remark}



% \deni{Integrate proof below to here}



% \if 0
% \subsection{Dynamic Fisher Markets}

% To warm-up, we first consider a repeated Fisher market in which buyers have only one budget to spend throughout time.
% A dynamic\amy{maybe this should be called a seq'l market, to match you notion of eqm?}\deni{Thing is the same mathematical construct can be analyzed both with a sequential equilibrium and a recursive equilibrium} Fisher market consists of:
% \begin{enumerate}
%     % \item A set of states $\states$, describing the state in which the market is.
%     % \item A initial budget  $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
%     \item A set of $\numgoods$ goods. Each good $\good \in \goods$ has wlog unit supply.
    
%     \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
%     \begin{enumerate}
%         \item a continuous and concave utility function $\util[\buyer]: \R^\numgoods \to \R$
%         \item an initial budget $\budget[\buyer][0] \in \R_+$ 
%         % \in \budgetspace$, where $\budgetspace$ is a compact-convex subset of $\R_+$
%     \end{enumerate}
%     % \item A transition function $\trans: \states \times \states \times \R_+^\numgoods \times \R_+^{\numgoods \times \numbuyers} \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when prices $\price \in  \R_+^{\numgoods} $ and $\allocation \in  \R_+^{\numgoods \times \numbuyers} $ are determined by the supply and demand sides respectively, is denoted by $\trans(\state^\prime \mid \price, \allocation)$.
    
    
%     \item a probability $\discount$ that the market will continue
%     \item an interest rate $\interest \in \R_+$ denoting the return on savings
% \end{enumerate}


% A dynamic Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \util, \budget[][0], \discount, \interest)$.\amy{what about $r$?}\deni{Added but I am guessing we should most likely remove it for final version} When clear from context, we simply write $(\util, \budget[][0], \discount, \interest)$.

% An \mydef{allocation} $\allocation \in \R^{\numbuyers \times \numgoods}_+$ is a mapping from buyers to goods such that $\allocation[\buyer][\good] \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$.
% %
% Goods are assigned anonymous \mydef{prices} $\price \in \R_+^\numgoods$ such that $\price[\good] \geq 0 $ denotes the cost of one unit of good $\good$ for any buyer.
% %
% Buyers can decide to spend some of their budget in the future by putting aside a \mydef{saving} $\saving \in \R_+^\numbuyers$ such that $\saving[\buyer] \geq 0$ denotes the amount of money saved by buyer $\buyer$.


% A \mydef{sequential competitive equilibrium} is sequence of allocation, \sdeni{}{savings}, and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraints at each time period such that for all  $\buyer \in \buyers$
%     \begin{align}
%         ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)})_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] \\ \budget[\buyer][\iter + 1] = (1+r) \saving[\buyer][\iter]} \right\}_{\iter = 1}^\infty } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)})
%     \end{align}
%     \item The market clears in each time period \samy{and}{meaning}\deni{Not true, that would mean that goods unallocated are priced at zero only if Walras' law and feasibility holds.} goods that are unallocated are priced at 0, i.e., for all $\good \in \goods$ and $\iter \in \N_+$:
%     \begin{align}
%         {\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = 1\\
%         {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq 1
%     \end{align}
% \end{enumerate}

% Define the \mydef{budget value function} $\budgetval[\buyer]: \R_+ \to \R$ for any buyer $\buyer$ as:

% \begin{align}
%     \budgetval[\buyer](\budget[\buyer]; \price[][*]) = \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] \\ \budget[\buyer][\iter + 1] = (1+r) \saving[\buyer][\iter]} \right\}_\iter } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}\right)
% \end{align}


% %
% We define an \mydef{allocation policy} $\allocation: \R^\numbuyers_+ \to \R^{\numbuyers \times \numgoods}$ as a mapping from budgets to allocations of goods to buyers such that $\allocation[\buyer][\good](\budget) \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$ in when buyers have budgets $\budget$. 
% %
% A \mydef{pricing policy} is a mapping $\price: \R_+ \to \R^\numgoods_+$ from budgets to prices such that for all $\good \in \goods$ and $\budget \in \R_+$, $\price[\good](\budget) \geq 0$ denotes the price of good when buyers have budgets $\budget$. 
% %
% A \mydef{saving policy} $\saving: \R_+^\numbuyers \to \R_+^\numbuyers$ isa mapping from budgets to savings such that $\saving[\buyer](\budget) \geq 0$ denotes the amount of money saved by buyer $\buyer$ at budgets $\budget$.

% We can then re-express the sequential competitive equilibrium in a more tractable equivalent form called a recursive competitive equilibrium using Bellman's optimality principle.  A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \saving^*, \price^*)$. which consists of an allocation policy and a pricing policy such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraint: \begin{align}
%         &\forall \buyer \in \buyers, \budget \in \R_+^\numbuyers &
%     (\allocation[\buyer]^*(\budget), \saving[\buyer]^*(\budget)) \in \argmax_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\budget) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer](1+ \interest))
%     \end{align}
%     \item The market clears in each state and goods that are unallocated in each state are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\state \in \states$:
%     \begin{align}
%         \price[\good]^*(\budget) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\budget) = 1\\
%         \price[\good]^*(\budget) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\budget) \leq 1
%     \end{align}
% \end{enumerate}


% \begin{lemma}\label{lemma:savings_foc}
% For any $\price \in \R_+^\numgoods$, a tuple $(\allocation[\buyer]^*, \saving[\buyer]^*)$ consisting of an allocation policy and saving policy for a buyer $\buyer$  is expected utility maximizing constrained by the saving and spending constrained iff there exists $\lambda^* > 0$ such that:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer])) - \lambda^*(\budget[\buyer]) \price[\good] \doteq 0 && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])  = \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest))   && \forall\buyer \in \buyers
% \end{align}
% \end{lemma}

% \begin{proof}
% Let $\calL(\allocation[\buyer], \saving[\buyer], \lambda; \price) = \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer]) + \lambda (\budget[\buyer] - \allocation[\buyer] \price)$ be the Lagrangian associated with $$\max_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\budget) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer])$$. Then, for any $\budget[\buyer] > 0$, Slater's condition holds \deni{Add more stuff on convexity + the necessary bureaucratic math} and the first order necessary and sufficient optimality conditions for an allocation $\allocation[\buyer]^* \in \R_+^{\numbuyers \times \numgoods}$, saving $\saving[\buyer]^* \in \R_+$ and associated Lagrangian multipliers $\lambda^* \in \R_+$ to be optimal for any prices $\price \in \R^\numgoods_+$ are given by the following pair of equations:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \lambda^*  \doteq \frac{\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer]))}{\price[\good]} && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \gamma (1+\interest)  \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(\budget[\buyer])(1+\interest)) -\lambda^*(\budget[\buyer]) \doteq 0 && \forall\buyer \in \buyers, \good \in \goods
% \end{align}
% Re-organizing expressions, yields:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \lambda^*  \doteq \frac{\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer]))}{\price[\good]} && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \lambda^*(\budget[\buyer]) \doteq \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest))  && \forall\buyer \in \buyers
% \end{align}
% This means that $\allocation[\buyer]^*$ and $\saving[\buyer]^*$ are optimal if there exists $\lambda \geq 0$ such that the above equations hold.

% Using the envelope theorem, we can also compute $\frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])$ as follows:
% \begin{align}
%     \frac{\partial \budgetval[\buyer]}{\partial \budget[\buyer]}(\budget[\buyer]) = \lambda^*(\budget[\buyer])
% \end{align}

% Combining the last two equations, we obtain, we can re-express the second optimality condition as follows:
% \begin{align}
%      \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])  = \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest)) 
% \end{align}
% \end{proof}

% Define the following optimal state value function:
% \begin{align}
%     \statevalue[][*][](\budget) = \min_{\{\price[][\iter] \in \R_+^{ \numgoods} \} }\max_{\left\{ \substack{  ({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)}) \in \R^{\numbuyers \times \numgoods}_+ \times \R_+^\numbuyers: \allocation[][][\iter] {\price^*}^{(\iter)} + \saving[][\iter] \leq \budget[][\iter] \\ \budget[][\iter + 1] = (1+\interest) \saving[][\iter]} \right\} } \sum_{\iter = 0}^\infty \discount^\iter\left(\sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer][\iter]\right) \log\left(\util[\buyer]\left(\allocation[\buyer][][\iter]\right)\right)\right)
% \end{align}
% We can re-express the above optimal state value function using Bellman's optimality principle:
% \begin{align}
%     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer])) + \discount \statevalue[][*](\saving)
% \end{align}

% \begin{theorem}
% The policy profile $(\price^*, \allocation^*, \saving^*) \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}$ that solves the following dynamic program:
% \begin{align}
%     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)
% \end{align}
% corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
% \end{theorem}

% \begin{proof}
% The first order necessary and sufficient optimality conditions for $\max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)$ are given by:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget)) - \langmult[\buyer]^*(\budget) \price[\good] \doteq 0 \label{eq:foc_rfm_2}\\
%     - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) +\discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) - \langmult[\buyer]^*(\budget) \doteq 0\label{eq:foc_rfm_2}
% \end{align}

% Using the envelope theorem, we can compute $\frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}$ as follows:
% \begin{align}
%     \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) = \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) + \langmult[\buyer]^*(\budget)
% \end{align}
% Re-organizing expressions, we get:
% \begin{align}
%     \langmult[\buyer]^*(\budget) = \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right)\label{eq:envelope_value_rfm}
% \end{align}

% Combining \Cref{eq:envelope_value_rfm} and \Cref{eq:foc_rfm_2}, we obtain:
% \begin{align}
%     - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) +\discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) &= \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right)\\
%     \discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) &= \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget)
% \end{align}
% which is exactly the optimality conditions for the savings of buyers by \Cref{lemma:savings_foc}.

% Going back to \Cref{eq:foc_rfm_2} and multiplying both sides by $\allocation[\buyer][\good]^*(\budget)$, we also have:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) - \langmult[\buyer]^*(\budget) \price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% Summing up across all $\good \in \goods$, we then have:
% \begin{align}
%     \sum_{\good \in \goods} \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) - \sum_{\good \in \goods} \langmult[\buyer]^*(\budget) \price[\good]\allocation[\buyer][\good]^*(\budget) = 0\\
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \sum_{\good \in \goods} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% By Euler's theorem for homogeneous functions, we have:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \util[\buyer](\allocation[\buyer]^*(\budget)) -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) = 0\\
%     \budget[\buyer] - \saving[\buyer]^* -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods}\price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% From the slack complementarity conditions, we have $ \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) =  \langmult[\buyer]^*(\budget)  \left(\budget[\buyer] - \saving[\buyer]^*(\budget)\right)$, giving us:
% \begin{align}
%     \budget[\buyer] - \saving[\buyer]^* - \langmult[\buyer]^*(\budget)  \left(\budget[\buyer] - \saving[\buyer]^*(\budget)\right) = 0\\
%     \langmult[\buyer]^*(\budget)  = 1
% \end{align}

% The first order necessary and sufficient conditions for $\min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)$ are given by:
% \begin{align}
%     1 - \sum_{\buyer \in \buyers} \langmult[\buyer]^*(\budget) \allocation[\buyer]^*(\budget) \in 0
% \end{align}
% Plugging back in the value of the optimal Lagrange multipliers, we obtain:

% \begin{align}
%     1 - \sum_{\buyer \in \buyers}  \allocation[\buyer]^*(\budget) \in 0\\
%     1 \in \sum_{\buyer \in \buyers}  \allocation[\buyer]^*(\budget) 
% \end{align}
% \end{proof}

% \subsection{Stochastic Fisher Markets}

% A stochastic Fisher market consists of:
% \begin{enumerate}
%     % \item A set of states $\states$, describing the state in which the market is.
%     % \item A initial budget  $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
%     \item A set of $\numgoods$ goods. Each good $\good \in \goods$ has:
%     \begin{itemize}
%         \item a supply space that denotes the possible supplies of goods $\supplyspace[\good] \subset \R_+^\numgoods$. We denote the set of all possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$
%     \end{itemize}
    
%     \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
%     \begin{enumerate}
%         \item a type space $\typespace[\buyer]$. We denote the type space of all buyers by $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$.
%         \item a continuous and concave utility function $\util[\buyer]: \R^\numgoods_+ \times \typespace[\buyer] \to \R_+ $. 
%         \item a space of possible budgets $\budgetspace$. We denote the space of all possible budget for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$
%         \item an initial budget $\budget[\buyer][0] \in \budgetspace[\buyer]$
%     \end{enumerate}
%     \item A transition function $\trans: \states \times \states \times  \R_+^{\numgoods \times \numbuyers} \times \R^\numbuyers \to [0,1]$ where for simplicity, we let $\states = \typespace \times \budgetspace  \times \supplyspace$ and the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when  allocations $\allocation \in  \R_+^{\numgoods \times \numbuyers}$ and saving $\saving \in \R^\numbuyers_+$ are determined by the consumers, is denoted by $\trans(\state^\prime \mid  \state, \allocation, \saving)$.
    
    
%     \item a probability $\discount$ that the market will continue
%     \item an interest rate $\interest \in \R_+$ denoting the return on savings
% \end{enumerate}

% A dynamic Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$. When clear from context, we simply write $(\util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$.

% A \mydef{sequential competitive equilibrium} is sequence of allocation and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)} {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraint, i.e., for all $\buyer \in \buyers$: \begin{align}
%         ({{\allocation[\buyer][][\iter]}^*}, {\saving[\buyer][\iter]}^*)_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  ({{\allocation[\buyer]}^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} +
%         \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_{\iter = 1}^\infty } \mathop{\E}_{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter]) }
%         \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]({\allocation[\buyer]}^{(\iter)}; \type[\buyer][\iter])\right] \enspace,
%     \end{align} 
%     where $\state[\iter] = (\type[][\iter], \budget[][\iter], \supply[][\iter])$.
%     \item The market clears in each time period and goods that are unallocated are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\iter \in \N_+$:
%     \begin{align}
%         {\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = \supply[\good][\iter]\\
%         {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq \supply[\good][\iter]
%     \end{align}
% \end{enumerate}

% Define $\budgetval[\buyer]: \states \times \R^{\states \times \numbuyers \times \numgoods} \times \R^{\states \times \numbuyers} \times \R^{\states \times \numgoods} \to \R$ \deni{Add parameters to description}:
% \begin{align}
%     \budgetval[\buyer](\type, \budget, \supply; \allocation, \saving, \price) &= \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_\iter } \mathop{\E}_{\substack{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter])\\ \state[0] = \state }} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter]\right)\right]\\
%     &= \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) + \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \allocation[][][](\state), \saving[][](\state)) } \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) \saving(\type, \budget, \supply), \supply^\prime; \allocation, \saving, \price) \right]
% \end{align}

% We can then re-express a sequential competitive equilibrium as a recursive competitive equilibrium. A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \saving^*, \price^*)$. which consists of an allocation policy and a pricing policy such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraint such that for all states $(\type, \budget, \supply) \in \states$:
%     \begin{align}
%     &
%     (\allocation[\buyer]^*(\type, \budget, \supply), \saving[\buyer]^*(\type, \budget, \supply)) \in \argmax_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\type, \budget, \supply) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) \\ \notag   & + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation^*, \saving^*, \price^*) \right]
%     \end{align}
%     \item The market clears in each state and goods that are unallocated in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$:
%     \begin{align}
%         \price[\good]^*(\type, \budget, \supply) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) = 1\\
%         \price[\good]^*(\type, \budget, \supply) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) \leq 1
%     \end{align}
% \end{enumerate}


% Define the following value function:
% \begin{align}
%     &\statevalue(\type, \budget, \supply; \allocation, \saving, \price) = \sum_{\good \in \goods} \supply[\good] \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](\type, \budget, \supply), \type[\buyer]) + \\ \notag &\discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \statevalue[][](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation, \saving, \price) \right]
% \end{align}


% \begin{theorem}
% There exists a recursive Stackelberg equilibrium $(\price^*, \allocation^*, \saving^*) \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}$ that solves the following dynamic program:
% \begin{align}
%     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest), \type[\buyer])) + \discount \statevalue[][*](\saving)
% \end{align}
% Additionally, any recursive Stackelberg equilibrium corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
% \end{theorem}

% \fi

% % We now move on to show an application of the computation of zero-sum stochastic Stackelberg game.
% % \subsection{Stochastic Fisher Markets}

% % To warm-up we start by considering a generalization of a well known market model, the Fisher market \cite{brainard2000compute}, to a dynamic setting. 
% % A \mydef{stochastic Fisher market} consists of a set of $\numgoods$ goods and set of $\numbuyers$ buyers. Each good $\good \in \goods$ has a supply space that denotes the possible supplies of goods $\supplyspace[\good] \subset \R_+^\numgoods$. We denote the set of all possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$. Each buyer $\buyer \in \buyers$ has a type space $\typespace[\buyer]$, a continuous  concave utility function $\util[\buyer]: \R^\numgoods_+ \times \typespace[\buyer] \to \R_+ $, and an initial budget $\budget[\buyer][0] \in \budgetspace[\buyer]$ coming from a budget space $\budgetspace[\buyer]$. We denote the type space of all buyers as $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$, and the space of all possible budget for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$. Buyers start their lives with budgets $\budget[][0]$, and are allocated different goods based on their budget and preferences in different markets drawn randomly from a \mydef{market state space} $\states = \typespace \times \budgetspace  \times \supplyspace$. More precisely, in each market buyers are given an \mydef{allocation} $\allocation \in \R^{\numbuyers \times \numgoods}_+$ which is a mapping from buyers to goods such that $\allocation[\buyer][\good] \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$. Additionally goods are assigned anonymous \mydef{prices} $\price \in \R_+^\numgoods$ such that $\price[\good] \geq 0 $ denotes the cost of one unit of good $\good$ for any buyer. At each discrete time step, buyers encounter a new market, and after some prices $\price$ and allocations $\allocation$ are decided by the market, either the market comes to an end with probability $(1-\discount)$ or it moves into a new state determined by a transition function $\trans: \states \times \states \times  \R_+^{\numgoods \times \numbuyers} \times \R^\numbuyers \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when allocations $\allocation \in  \R_+^{\numgoods \times \numbuyers}$ are determined by the market, is denoted by $\trans(\state^\prime \mid  \state, \allocation, \saving)$. A stochastic Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$. When clear from context, we simply write $(\util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$.

% % There exists two well-known solution concepts for dynamic markets which are equivalent. The first one is the \mydef{sequential competitive equilibrium} which is sequence of allocation and price tuples $({\allocation^*}^{(\iter)}, {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that 1.~the buyers are expected utility maximizing constrained by the saving and spending constraint, i.e., for all $\buyer \in \buyers$, $ \{{\allocation[\buyer][][\iter]}^*\}_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  {\allocation[\buyer]^*}^{(\iter)} \in \R^{\numgoods}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} \leq \budget[\buyer][\iter] }  \right\}_{\iter = 1}^\infty } \mathop{\E}_{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter])} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter])\right]$ 
% % % where $\state[\iter] = (\type[][\iter], \budget[][\iter], \supply[][\iter])$
% % 2.~the market clears in each time period and goods that are unallocated are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\iter \in \N_+$, ${\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = \supply[\good][\iter]$, or $ {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq \supply[\good][\iter]$. Unfortunately, although mathematically interesting, the sequential competitive equilibrium is untractable as it requires the computation of an infinite sequence!


% % Define $\budgetval[\buyer]: \states \times \R^{\statespace \times \numbuyers \times \numgood} \times \R^{\statespace \times \numbuyers} \times \R^{\statespace \times \numgood} \to \R$ \deni{Add parameters to description}:
% % \begin{align}
% %     \budgetval[\buyer](\type, \budget, \supply; \allocation, \saving, \price) &= 
% %     % \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_\iter }
% %     \mathop{\E}_{\substack{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter])\\ \state[0] = \state }} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter]\right)\right]\\
% %     &= \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) + \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \allocation[][][](\state), \saving[][](\state)) } \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) \saving(\type, \budget, \supply), \supply^\prime; \allocation, \saving, \price) \right]
% % \end{align}

% % We can then re-express a sequential competitive equilibrium as a recursive competitive equilibrium. A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \saving^*, \price^*)$. which consists of an allocation policy and a pricing policy such that:
% % \begin{enumerate}
% %     \item The buyers are expected utility maximizing constrained by the saving and spending constraint such that for all states $(\type, \budget, \supply) \in \statespace$:
% %     \begin{align}
% %     &
% %     (\allocation[\buyer]^*(\type, \budget, \supply), \saving[\buyer]^*(\type, \budget, \supply)) \in \argmax_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\type, \budget, \supply) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) \\ \notag   & + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation^*, \saving^*, \price^*) \right]
% %     \end{align}
% %     \item The market clears in each state and goods that are unallocated in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$:
% %     \begin{align}
% %         \price[\good]^*(\type, \budget, \supply) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) = 1\\
% %         \price[\good]^*(\type, \budget, \supply) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) \leq 1
% %     \end{align}
% % \end{enumerate}


% % Define the following value function:
% % \begin{align}
% %     &\statevalue(\type, \budget, \supply; \allocation, \saving, \price) = \sum_{\good \in \goods} \supply[\good] \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](\type, \budget, \supply), \type[\buyer]) + \\ \notag &\discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \statevalue[][](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation, \saving, \price) \right]
% % \end{align}


% % \begin{theorem}
% % There exists a Stackelberg equilibrium $(\price^*, \allocation^*, \saving^*) \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}$ that solves the following dynamic program:
% % \begin{align}
% %     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest), \type[\buyer])) + \discount \statevalue[][*](\saving)
% % \end{align}
% % Additionally, any Stackelberg equilibrium corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
% % \end{theorem}

% \subsection{Dynamic Fisher Markets}

% To warm-up, we first consider a repeated Fisher market in which buyers have only one budget to spend throughout time.
% A dynamic\amy{maybe this should be called a seq'l market, to match you notion of eqm?}\deni{Thing is the same mathematical construct can be analyzed both with a sequential equilibrium and a recursive equilibrium} Fisher market consists of:
% \begin{enumerate}
%     % \item A set of states $\states$, describing the state in which the market is.
%     % \item A initial budget  $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
%     \item A set of $\numgoods$ goods. Each good $\good \in \goods$ has wlog unit supply.
    
%     \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
%     \begin{enumerate}
%         \item a continuous and concave utility function $\util[\buyer]: \R^\numgoods \to \R$
%         \item an initial budget $\budget[\buyer][0] \in \R_+$ 
%         % \in \budgetspace$, where $\budgetspace$ is a compact-convex subset of $\R_+$
%     \end{enumerate}
%     % \item A transition function $\trans: \states \times \states \times \R_+^\numgoods \times \R_+^{\numgoods \times \numbuyers} \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when prices $\price \in  \R_+^{\numgoods} $ and $\allocation \in  \R_+^{\numgoods \times \numbuyers} $ are determined by the supply and demand sides respectively, is denoted by $\trans(\state^\prime \mid \price, \allocation)$.
    
    
%     \item a probability $\discount$ that the market will continue
%     \item an interest rate $\interest \in \R_+$ denoting the return on savings
% \end{enumerate}


% A dynamic Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \util, \budget[][0], \discount, \interest)$.\amy{what about $r$?}\deni{Added but I am guessing we should most likely remove it for final version} When clear from context, we simply write $(\util, \budget[][0], \discount, \interest)$.

% An \mydef{allocation} $\allocation \in \R^{\numbuyers \times \numgoods}_+$ is a mapping from buyers to goods such that $\allocation[\buyer][\good] \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$.
% %
% Goods are assigned anonymous \mydef{prices} $\price \in \R_+^\numgoods$ such that $\price[\good] \geq 0 $ denotes the cost of one unit of good $\good$ for any buyer.
% %
% Buyers can decide to spend some of their budget in the future by putting aside a \mydef{saving} $\saving \in \R_+^\numbuyers$ such that $\saving[\buyer] \geq 0$ denotes the amount of money saved by buyer $\buyer$.


% A \mydef{sequential competitive equilibrium} is sequence of allocation, savings, and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraints at each time period such that for all  $\buyer \in \buyers$
%     \begin{align}
%         ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)})_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] \\ \budget[\buyer][\iter + 1] = (1+r) \saving[\buyer][\iter]} \right\}_{\iter = 1}^\infty } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)})
%     \end{align}
%     \item The market clears in each time period \samy{and}{meaning}\deni{Not true, that would mean that goods unallocated are priced at zero only if Walras' law and feasibility holds.} goods that are unallocated are priced at 0, i.e., for all $\good \in \goods$ and $\iter \in \N_+$:
%     \begin{align}
%         {\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = 1\\
%         {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq 1
%     \end{align}
% \end{enumerate}

% Define the \mydef{budget value function} $\budgetval[\buyer]: \R_+ \to \R$ for any buyer $\buyer$ as:

% \begin{align}
%     \budgetval[\buyer](\budget[\buyer]; \price[][*]) = \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] \\ \budget[\buyer][\iter + 1] = (1+r) \saving[\buyer][\iter]} \right\}_\iter } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}\right)
% \end{align}


% %
% We define an \mydef{allocation policy} $\allocation: \R^\numbuyers_+ \to \R^{\numbuyers \times \numgoods}$ as a mapping from budgets to allocations of goods to buyers such that $\allocation[\buyer][\good](\budget) \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$ in when buyers have budgets $\budget$. 
% %
% A \mydef{pricing policy} is a mapping $\price: \R_+ \to \R^\numgoods_+$ from budgets to prices such that for all $\good \in \goods$ and $\budget \in \R_+$, $\price[\good](\budget) \geq 0$ denotes the price of good when buyers have budgets $\budget$. 
% %
% A \mydef{saving policy} $\saving: \R_+^\numbuyers \to \R_+^\numbuyers$ isa mapping from budgets to savings such that $\saving[\buyer](\budget) \geq 0$ denotes the amount of money saved by buyer $\buyer$ at budgets $\budget$.\deni{Add saving policy}

% We can then re-express the sequential competitive equilibrium in a more tractable equivalent form called a recursive competitive equilibrium using Bellman's optimality principle.  A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \saving^*, \price^*)$. which consists of an allocation policy and a pricing policy such that:
% \begin{enumerate}
%     \item The buyers are expected utility maximizing constrained by the saving and spending constraint: \begin{align}
%         &\forall \buyer \in \buyers, \budget \in \R_+^\numbuyers &
%     (\allocation[\buyer]^*(\budget), \saving[\buyer]^*(\budget)) \in \argmax_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\budget) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer](1+ \interest))
%     \end{align}
%     \item The market clears in each state and goods that are unallocated in each state are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\state \in \states$:
%     \begin{align}
%         \price[\good]^*(\budget) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\budget) = 1\\
%         \price[\good]^*(\budget) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\budget) \leq 1
%     \end{align}
% \end{enumerate}


% \begin{lemma}\label{lemma:savings_foc}
% For any $\price \in \R_+^\numgoods$, a tuple $(\allocation[\buyer]^*, \saving[\buyer]^*)$ consisting of an allocation policy and saving policy for a buyer $\buyer$  is expected utility maximizing constrained by the saving and spending constrained iff there exists $\lambda^* > 0$ such that:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer])) - \lambda^*(\budget[\buyer]) \price[\good] \doteq 0 && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])  = \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest))   && \forall\buyer \in \buyers
% \end{align}
% \end{lemma}

% \begin{proof}
% Let $\calL(\allocation[\buyer], \saving[\buyer], \lambda; \price) = \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer]) + \lambda (\budget[\buyer] - \allocation[\buyer] \price)$ be the Lagrangian associated with $$\max_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\budget) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer](\allocation[\buyer]) + \discount \budgetval[\buyer](\saving[\buyer])$$. Then, for any $\budget[\buyer] > 0$, Slater's condition holds \deni{Add more stuff on convexity + the necessary bureaucratic math} and the first order necessary and sufficient optimality conditions for an allocation $\allocation[\buyer]^* \in \R_+^{\numbuyers \times \numgoods}$, saving $\saving[\buyer]^* \in \R_+$ and associated Lagrangian multipliers $\lambda^* \in \R_+$ to be optimal for any prices $\price \in \R^\numgoods_+$ are given by the following pair of equations:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \lambda^*  \doteq \frac{\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer]))}{\price[\good]} && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \gamma (1+\interest)  \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(\budget[\buyer])(1+\interest)) -\lambda^*(\budget[\buyer]) \doteq 0 && \forall\buyer \in \buyers, \good \in \goods
% \end{align}
% Re-organizing expressions, yields:
% \begin{align}
%     \allocation[\buyer][\good]^*(\budget[\buyer]) > 0 \implies  \lambda^*  \doteq \frac{\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}(\allocation[\buyer]^*(\budget[\buyer]))}{\price[\good]} && \forall\buyer \in \buyers, \good \in \goods\\
%     \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \lambda^*(\budget[\buyer]) \doteq \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest))  && \forall\buyer \in \buyers
% \end{align}
% This means that $\allocation[\buyer]^*$ and $\saving[\buyer]^*$ are optimal if there exists $\lambda \geq 0$ such that the above equations hold.

% Using the envelope theorem, we can also compute $\frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])$ as follows:
% \begin{align}
%     \frac{\partial \budgetval[\buyer]}{\partial \budget[\buyer]}(\budget[\buyer]) = \lambda^*(\budget[\buyer])
% \end{align}

% Combining the last two equations, we obtain, we can re-express the second optimality condition as follows:
% \begin{align}
%      \saving[\buyer]^*(\budget[\buyer]) > 0 \implies \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\budget[\buyer])  = \gamma (1+\interest) \frac{\partial \budgetval[\buyer]}{\partial \saving[\buyer]}(\saving[\buyer]^*(1+\interest)) 
% \end{align}
% \end{proof}

% Define the following optimal state value function:
% \begin{align}
%     \statevalue[][*][](\budget) = \min_{\{\price[][\iter] \in \R_+^{ \numgoods} \} }\max_{\left\{ \substack{  ({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)}) \in \R^{\numbuyers \times \numgoods}_+ \times \R_+^\numbuyers: \allocation[][][\iter] {\price^*}^{(\iter)} + \saving[][\iter] \leq \budget[][\iter] \\ \budget[][\iter + 1] = (1+\interest) \saving[][\iter]} \right\} } \sum_{\iter = 0}^\infty \discount^\iter\left(\sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer][\iter]\right) \log\left(\util[\buyer]\left(\allocation[\buyer][][\iter]\right)\right)\right)
% \end{align}
% We can re-express the above optimal state value function using Bellman's optimality principle:
% \begin{align}
%     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer])) + \discount \statevalue[][*](\saving)
% \end{align}


% \begin{theorem}
% The policy profile $(\price^*, \allocation^*, \saving^*) \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}$ that solves the following dynamic program:
% \begin{align}
%     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)
% \end{align}
% corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
% \end{theorem}

% \begin{proof}
% The first order necessary and sufficient optimality conditions for $\max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)$ are given by:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget)) - \langmult[\buyer]^*(\budget) \price[\good] \doteq 0 \label{eq:foc_rfm_2}\\
%     - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) +\discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) - \langmult[\buyer]^*(\budget) \doteq 0\label{eq:foc_rfm_2}
% \end{align}

% Using the envelope theorem, we can compute $\frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}$ as follows:
% \begin{align}
%     \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) = \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) + \langmult[\buyer]^*(\budget)
% \end{align}
% Re-organizing expressions, we get:
% \begin{align}
%     \langmult[\buyer]^*(\budget) = \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right)\label{eq:envelope_value_rfm}
% \end{align}

% Combining \Cref{eq:envelope_value_rfm} and \Cref{eq:foc_rfm_2}, we obtain:
% \begin{align}
%     - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right) +\discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) &= \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget) - \log\left(\util[\buyer](\allocation[\buyer]^*(\budget)) \right)\\
%     \discount (1+ \interest) \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}\left(\saving[\buyer]^* (1+ \interest) \right) &= \frac{\partial \statevalue[][*]}{\partial \budget[\buyer]}(\budget)
% \end{align}
% which is exactly the optimality conditions for the savings of buyers by \Cref{lemma:savings_foc}.

% Going back to \Cref{eq:foc_rfm_2} and multiplying both sides by $\allocation[\buyer][\good]^*(\budget)$, we also have:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) - \langmult[\buyer]^*(\budget) \price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% Summing up across all $\good \in \goods$, we then have:
% \begin{align}
%     \sum_{\good \in \goods} \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) - \sum_{\good \in \goods} \langmult[\buyer]^*(\budget) \price[\good]\allocation[\buyer][\good]^*(\budget) = 0\\
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \sum_{\good \in \goods} \frac{\partial\util[\buyer]}{\partial \allocation[\buyer][\good]} (\allocation[\buyer]^*(\budget))\allocation[\buyer][\good]^*(\budget) -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% By Euler's theorem for homogeneous functions, we have:
% \begin{align}
%     \frac{\budget[\buyer] - \saving[\buyer]^*}{\util[\buyer](\allocation[\buyer]^*(\budget))} \util[\buyer](\allocation[\buyer]^*(\budget)) -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) = 0\\
%     \budget[\buyer] - \saving[\buyer]^* -  \langmult[\buyer]^*(\budget) \sum_{\good \in \goods}\price[\good]\allocation[\buyer][\good]^*(\budget) = 0
% \end{align}
% From the slack complementarity conditions, we have $ \langmult[\buyer]^*(\budget) \sum_{\good \in \goods} \price[\good]\allocation[\buyer][\good]^*(\budget) =  \langmult[\buyer]^*(\budget)  \left(\budget[\buyer] - \saving[\buyer]^*(\budget)\right)$, giving us:
% \begin{align}
%     \budget[\buyer] - \saving[\buyer]^* - \langmult[\buyer]^*(\budget)  \left(\budget[\buyer] - \saving[\buyer]^*(\budget)\right) = 0\\
%     \langmult[\buyer]^*(\budget)  = 1
% \end{align}

% The first order necessary and sufficient conditions for $\min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest))) + \discount \statevalue[][*](\saving)$ are given by:
% \begin{align}
%     1 - \sum_{\buyer \in \buyers} \langmult[\buyer]^*(\budget) \allocation[\buyer]^*(\budget) \in 0
% \end{align}
% Plugging back in the value of the optimal Lagrange multipliers, we obtain:

% \begin{align}
%     1 - \sum_{\buyer \in \buyers}  \allocation[\buyer]^*(\budget) \in 0\\
%     1 \in \sum_{\buyer \in \buyers}  \allocation[\buyer]^*(\budget) 
% \end{align}
% \end{proof}

% % \subsection{Stochastic Fisher Markets}

% % A stochastic Fisher market consists of:
% % \begin{enumerate}
% %     % \item A set of states $\states$, describing the state in which the market is.
% %     % \item A initial budget  $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
% %     \item A set of $\numgoods$ goods. Each good $\good \in \goods$ has:
% %     \begin{itemize}
% %         \item a supply space that denotes the possible supplies of goods $\supplyspace[\good] \subset \R_+^\numgoods$. We denote the set of all possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$
% %     \end{itemize}
    
% %     \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
% %     \begin{enumerate}
% %         \item a type space $\typespace[\buyer]$. We denote the type space of all buyers by $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$.
% %         \item a continuous and concave utility function $\util[\buyer]: \R^\numgoods_+ \times \typespace[\buyer] \to \R_+ $. 
% %         \item a space of possible budgets $\budgetspace$. We denote the space of all possible budget for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$
% %         \item an initial budget $\budget[\buyer][0] \in \budgetspace[\buyer]$
% %     \end{enumerate}
% %     \item A transition function $\trans: \states \times \states \times  \R_+^{\numgoods \times \numbuyers} \times \R^\numbuyers \to [0,1]$ where for simplicity, we let $\states = \typespace \times \budgetspace  \times \supplyspace$ and the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when  allocations $\allocation \in  \R_+^{\numgoods \times \numbuyers}$ and saving $\saving \in \R^\numbuyers_+$ are determined by the consumers, is denoted by $\trans(\state^\prime \mid  \state, \allocation, \saving)$.
    
    
% %     \item a probability $\discount$ that the market will continue
% %     \item an interest rate $\interest \in \R_+$ denoting the return on savings
% % \end{enumerate}

% % A dynamic Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$. When clear from context, we simply write $(\util, \budget[][0], \typespace, \budgetspace, \supplyspace,  \trans, \discount)$.

% % A \mydef{sequential competitive equilibrium} is sequence of allocation and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)} {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that:
% % \begin{enumerate}
% %     \item The buyers are expected utility maximizing constrained by the saving and spending constraint, i.e., for all $\buyer \in \buyers$: \begin{align}
% %         ({\allocation[\buyer][][\iter]^*}, {\saving[\buyer][\iter]^*})_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_{\iter = 1}^\infty } \mathop{\E}_{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter]) } \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter])\right] \enspace,
% %     \end{align} 
% %     where $\state[\iter] = (\type[][\iter], \budget[][\iter], \supply[][\iter])$.
% %     \item The market clears in each time period and goods that are unallocated are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\iter \in \N_+$:
% %     \begin{align}
% %         {\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = \supply[\good][\iter]\\
% %         {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq \supply[\good][\iter]
% %     \end{align}
% % \end{enumerate}

% % Define $\budgetval[\buyer]: \statespace \times \R^{\statespace \times \numbuyers \times \numgood} \times \R^{\statespace \times \numbuyers} \times \R^{\statespace \times \numgood} \to \R$ \deni{Add parameters to description}:
% % \begin{align}
% %     \budgetval[\buyer](\type, \budget, \supply; \allocation, \saving, \price) &= \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_\iter } \mathop{\E}_{\substack{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter])\\ \state[0] = \state }} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter]\right)\right]\\
% %     &= \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) + \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \allocation[][][](\state), \saving[][](\state)) } \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) \saving(\type, \budget, \supply), \supply^\prime; \allocation, \saving, \price) \right]
% % \end{align}

% % We can then re-express a sequential competitive equilibrium as a recursive competitive equilibrium. A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \saving^*, \price^*)$. which consists of an allocation policy and a pricing policy such that:
% % \begin{enumerate}
% %     \item The buyers are expected utility maximizing constrained by the saving and spending constraint such that for all states $(\type, \budget, \supply) \in \statespace$:
% %     \begin{align}
% %     &
% %     (\allocation[\buyer]^*(\type, \budget, \supply), \saving[\buyer]^*(\type, \budget, \supply)) \in \argmax_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\type, \budget, \supply) + \saving[\buyer] \leq \budget[\buyer]}  \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) \\ \notag   & + \discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation^*, \saving^*, \price^*) \right]
% %     \end{align}
% %     \item The market clears in each state and goods that are unallocated in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$:
% %     \begin{align}
% %         \price[\good]^*(\type, \budget, \supply) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) = 1\\
% %         \price[\good]^*(\type, \budget, \supply) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\type, \budget, \supply) \leq 1
% %     \end{align}
% % \end{enumerate}


% % Define the following value function:
% % \begin{align}
% %     &\statevalue(\type, \budget, \supply; \allocation, \saving, \price) = \sum_{\good \in \goods} \supply[\good] \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](\type, \budget, \supply), \type[\buyer]) + \\ \notag &\discount \mathop{\E}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \type, \budget, \supply)} \left[ \statevalue[][](\type^\prime, \budget^\prime + (1+\interest) (\saving[\buyer], \saving_{-\buyer}^*(\type, \budget, \supply)), \supply^\prime; \allocation, \saving, \price) \right]
% % \end{align}


% % \begin{theorem}
% % There exists a Stackelberg equilibrium $(\price^*, \allocation^*, \saving^*) \in \R^{\R_+ \times \numgoods} \times \R_+^{\R_+ \times \numbuyers \times \numgoods} \times \R_+^{\R_+ \times \numbuyers}$ that solves the following dynamic program:
% % \begin{align}
% %     \statevalue[][*](\budget) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times \numgoods } \times \R_+^\numbuyers : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer](1 + \interest), \type[\buyer])) + \discount \statevalue[][*](\saving)
% % \end{align}
% % Additionally, any Stackelberg equilibrium corresponds to the recursive competitive equilibrium of the CCH Fisher market $(\util, \budget[][0], \discount)$
% % \end{theorem}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/generalsum.tex <==
A \mydef{(generalized) Stackelberg game}, $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$, is a two-player, general-sum game, where one player, who we call the outer, or $\outer$-, player (resp.\ the inner, or $\inner$-, player)\deni{Might want to replace outer and inner with follower and leader}, is trying to maximize their payoff, defined by a \emph{continuous} \mydef{payoff function} $\util[\outer]: X \times Y \rightarrow \mathbb{R}$ (resp. $\util[\inner]: X \times Y \rightarrow \mathbb{R}$), by taking an action from their non-empty and compact \mydef{\sdeni{strategy}{action} set}\deni{first player's action set is equal to their strategy set but this is not the case for the second player. For the second player, the action set is $\innerset$, while the strategy set is $\outerset \times \innerset$, i.e., it is the set of all possible contingent plans.} $\outerset \subset \R^\outerdim$, and (resp. $\innerset \subset \R^\innerdim$) s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1](\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$ continuous. A \mydef{strategy profile} $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff for all $\numconstr \in [\numconstrs]$, $\constr[\numconstr](\outer, \inner) \geq 0$. A Stackelberg game is said to be convex if the actions sets $\outerset, \innerset$ are convex, and for all $(\outer, \inner) \in \outerset \times \innerset$ the payoff functions $\util[\outer](\ \cdot \, \inner), \util[\inner](\outer, \ \cdot \ )$ as well as the constraints $\constr[1](\outer, \ \cdot \ ), \hdots, \constr[\numconstrs](\outer, \ \cdot \ )$, are concave.\deni{Maybe switch from payoff functions to loss functions so that this is more consistent?}
For each outer player's action $\outer \in \outerset$, we define the best-response set of the inner player as $\br(\outer) = \argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)$.
In Stackelberg games, the outer player seeks to maximize their payoff assuming the inner player chooses a feasible best response that maximizes the outer player's payoff, i.e., the outer player maximizes their \mydef{marginal function} \cite{berge1997topological}, is defined as $\marginal[\outer](\outer) = \max_{\inner \in \br(\outer) }  \util[\outer](\outer, \inner)$. Note that for the purposes of our expositions to ensure that $\marginal[\outer]$ is a well-defined function, we assumed in this definition that the follower breaks ties amongst their best-responses in the leader’s favor. This is known as \mydef{optimistic tie breaking} and provides a best-case guarantee for the leader. 
% The inner player's value function, $\val[\innerset]: \outerset \to \R$, which they seek to maximize, is simply the objective function given the outer player's action $\hat{\outer}$: i.e., $\val[\innerset](\inner; \hat{\outer}) = \obj(\hat{\outer}, \inner)$.

A strategy profile $\left(\outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ s.t.\ $\constr(\outer^{*}, \inner^{*}) \geq \zeros$ is an $(\epsilon, \delta)$-\mydef{Stackelberg equilibrium} if
\begin{align}
    \util[\outer](\outer^*, \inner^*) \geq \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner) - \varepsilon && \forall \outer \in \outerset\\
    \util[\inner](\outer^*, \inner^*) \geq \util[\inner](\outer^*, \inner) - \delta 
    && \forall  \inner \in \innerset  \text{ s.t. } \constr(\outer^*, \inner) \geq \zeros
\end{align}

Intuitively, a $(\varepsilon, \delta)$-Stackelberg equilibrium is a point at which the $\outer$-player's (resp.\ $\inner$-player's) payoff is no more than $\varepsilon$ (resp.\ $\delta$) away from its optimum.
A $(0,0)$-Stackelberg equilibrium is guaranteed to exist in Stackelberg games by the following theorem.

\begin{remark}
Note that, to guarantee existence of a Stackelberg equilibrium we assumed \mydef{optimistic tie breaking}. An alternative but as valid way of defining a Stackelberg equilibrium would have been to assume that the follower breaks ties against the leader's favor, i.e., \mydef{pessimistic tie breaking}, in such a case one can similarly show the existence of a Stackelberg equilibrium \cite{}. Historically, the literature on bi-level optimization has focused on the optimistic tie breaking rule as it allows for easier tractability
% However, while pessimistic  tie-breaking guarantees that the set of Stackelberg equilibria is non-empty and compact, optimistic tie-breaking guarantees that the set of Stackelberg equilibria is non-empty, compact, and \emph{convex}, as shown by the following theorem. 
\end{remark}

% The convexity of the set of Stackelberg equilibria allows 
% \subsection{Prperties of Stackelberg Equilibrium in Generalized Stackelberg Games}

% \deni{This assumption is not needed for static setting}

In general, a Nash equilibrium is not guaranteed to exist in convex Stackelberg games but a Stackelberg equilibrium always exists as shown by the following theorem. The following theorem is a slight variant of pre-existing results in the literature as it also shows that the set of Stackelberg equilbiria is compact. 

\begin{theorem}\label{thm:exitence_stackelberg}
% Suppose that parts 2 and 3 of \Cref{assum:stackelberg_general_sum} hold, then t
The set of Stackelberg equilibria of any Stackelberg game $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$ is non-empty and compact.
\end{theorem}

\begin{proof}
First, we note that since for all $\outer \in \outerset$, $\util[\inner](\outer, \inner ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer,\inner )$ are continuous in $\inner$, for all $\outer \in \outerset$, the correspondence $ \calC(\outer) = \{\inner \in  \innerset  \mid \constr(\outer, \inner) \geq \zeros\}$ is compact-valued and continuous. As a result, by the maximum theorem \cite{berge1997topological}, the best-response correspondence $\br$ is non-empty, upper hemicontinuous, compact-valued. Additionally, by Weierstrass's theorem, the set of optimistic best-responses of the inner player for any strategy of the outer player $\outer \in \outerset$, i.e., $\argmax_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ , is compact since $\util[\outer](\outer, \inner)$ is continuous and $\br(\outer)$ is compact. 

Now, we note that since $\br$ is non-empty, upper hemicontinuous, and compact-valued in $\outer$, and $\util[\outer](\outer, \inner)$ is continuous, by Theorem 2 of \citeauthor{berge1997topological} \cite{berge1997topological} the marginal function $\util[\outer]^*(\outer) = \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is upper semi continuous in $\outer$. Since for all $\outer \in \outerset$, $\br(\outer)$ is compact and  $\util[\outer](\outer, \inner)$  is continuous in $\inner$, $\util[\outer]^*(\outer)$ is well-defined for all $\outer \in \outerset$ such that for all $\outer \in \outerset, \left| \util[\outer]^*(\outer) \right| < \infty$, i.e., it is
%  a proper function. and 
level-bounded. By Theorem 1.9 of \citeauthor{rockafellar2009variational} \cite{rockafellar2009variational}, since $\util[\outer]^*$ is upper semicontinuous,
% proper, 
and level-bounded, the set $\argmax_{\outer \in \outerset}  \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is non-empty and compact.
% %
% \noindent
% Since we have shown that $\argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)$ is compact and non-empty, and $\util[\outer]( \ \cdot \, \inner)$ is concave, we have that $\max_{\inner \in \argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)} \util[\outer](\outer, \inner)$ is concave in $\outer$.
\end{proof}

\if 0

Next, we prove that the set of Stackelberg equilibria of a Stackelberg game are also convex. Our result depends on the following technical lemma which is a slight more general variant of known results.

\begin{lemma}\label{lemma:max_thm_var}
Consider a parametric optimization problem $\obj^*(\outer) = \max_{\inner \in \calC(\outer)} \obj(\outer, \inner)$. Suppose that $\calC: \outerset \rightrightarrows  \innerset$ is upper hemicontinuous, compact-convex valued, $\outerset \subset \R^\outerdim$ is convex, and $\obj$ is continuous and concave, then 1) $\obj^*(\outer)$ is upper semicontinuous and concave, and 2) $\calC^*(\outer) = \argmax_{\inner \in \calC(\outer)} \obj(\outer, \inner)$ is non-empty-, convex-, and compact-valued.
\end{lemma}

\begin{proof}
By Theorem 2 of \citeauthor{berge1997topological} \cite{berge1997topological} $\obj^*(\outer) = \max_{\inner \in \calC(\outer)} \obj(\outer, \inner)$ is upper semicontinuous in $\outer$ since $\calC$ is upper hemi-continuous and $\obj$ is continuous.

Since for all $\outer \in \R^\outerdim$, $\calC(\outer)$ is compact and  $\obj(\outer, \inner)$  is continuous in $\inner$, $\obj^*(\outer)$ is well-defined for all $\outer \in \R^\outerdim$ such that for all $\outer \in \R^\outerdim, \left| \obj^*(\outer) \right| < \infty$, i.e., $\obj^*$ is a proper function and level-bounded. By Theorem 1.9 of \citeauthor{rockafellar2009variational} \cite{rockafellar2009variational}, since $\obj^*$ is upper semicontinuous, proper, and level-bounded, for all $\outer \in \outerset$, $\calC^*(\outer)$ is non-empty and compact. 

We now prove that $\calC^*(\outer)$ is convex for all $\outer \in \outerset$. Pick $\bar{\inner}, \tilde{\inner} \in \calC^*(\outer^\prime)$, and let $\inner^\prime = \lambda \bar{\inner} + (1-\lambda) \tilde{\inner}$ for $\lambda \in [0,1]$. Note that we have $\inner^\prime \in \calC(\outer^\prime)$ since $\calC(\outer)$ is convex for all $\outer \in \outerset$. We then have by the concavity of $\obj$: 
\begin{align}
    \obj(\outer^\prime, \inner^\prime) &= \obj(\outer^\prime, \lambda \bar{\inner} + (1-\lambda) \tilde{\inner})\\
    &\geq  \lambda \obj(\outer^\prime,\bar{\inner} ) + (1-\lambda) \obj(\outer^\prime,   \tilde{\inner})\\ 
    &= \lambda \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner ) + (1-\lambda) \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner)\\
    &= \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner)
\end{align}
%
\noindent
which means that $\inner^\prime \in \calC^*(\outer^\prime)$, i.e., $\calC^*$ is convex-valued.


Pick any $\bar{\outer}, \tilde{\outer} \in \outerset$ and let $\outer^\prime = \lambda \bar{\outer} + (1-\lambda)\tilde{\outer}$ for $\lambda \in [0,1]$. By the convexity of $\outerset$, we then have $\outer^\prime \in \outerset$.  Let $\bar{\inner} \in \calC^*(\bar{\outer}) =  \argmax_{\inner \in \calC(\bar{\outer})} \obj(\bar{\outer}, \inner)$,  $\tilde{\inner} \in \calC^*(\tilde{\outer}) = \argmax_{\inner \in \calC(\tilde{\outer})} \obj( \tilde{\outer}, \inner)$, and $\inner^\prime = \lambda \bar{\inner} + (1-\lambda)\tilde{\inner}$. Since $\calC$ is convex-valued and $\outerset$ is convex, $\calC$ has a convex graph and we have $\inner^\prime \in \calC(\outer^\prime)$, which gives us:
\begin{align}
    \obj^*(\outer^\prime) &\geq \obj(\outer^\prime, \inner^\prime) && \text{(By definition of $\obj^*$)} \\
    &= \obj\left(\lambda \bar{\outer} + (1-\lambda)\tilde{\outer},  \lambda \bar{\inner} + (1-\lambda)\tilde{\inner}\right)\\
    &\geq \lambda \obj\left( \bar{\outer}, \bar{\inner} \right) + (1-\lambda) \obj(\tilde{\outer}, \tilde{\inner}) && \text{(Convexity of $\obj$)}\\
    &= \lambda \obj^*(\bar{\outer}) + (1-\lambda) \obj^*(\tilde{\outer})
\end{align}
%
which establishes that $\obj^*$ is concave.
\end{proof}


\deni{Seperate existence and convexity proofs. Existence requires continuous concave in each player's variable + convex constraints, while convex set of solutions requires outer player's payoff to be entire concave. This means that we get existence for both pessimistic and optimistic tie breaking, but we get convexity only for optimisitc tie breaking.}
\begin{theorem}
Suppose that \Cref{assum:stackelberg_general_sum} holds, then the set of Stackelberg equilibria of any convex Stackelberg game $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$ is non-empty, compact and convex.
\end{theorem}

\begin{proof}
First, we note that since for all $\outer \in \outerset$, $\util[\inner](\outer, \inner ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer,\inner )$ are continuous and concave in $\inner$, 
% for all $\outer \in \outerset$, we have that the set $\{\inner \in  \innerset  \mid \constr(\outer, \inner) \geq \zeros\}$ is compact and convex, and 
by the maximum theorem \cite{berge1997topological}, the best-response correspondence $\br$ is non-empty, upper hemicontinuous, compact-, and convex-valued. Hence, by \Cref{lemma:max_thm_var} the set of optimistic best-responses of the inner player for any strategy of the outer player $\outer \in \outerset$, i.e., $\argmax_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$, is non-empty, convex, and compact since $\util[\outer](\outer, \inner)$ is continuous and concave, and $\br(\outer)$ is compact. Similarly, by \Cref{lemma:max_thm_var} $\util[\outer]^*(\outer) = \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is upper semicontinuous and concave.

By \Cref{thm:exitence_stackelberg}, we know that the set of Stackelberg equilibrium strategies of the outer player, \\ i.e. $\argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, is non-empty, and compact, we will show it also is convex.
Pick $\bar{\outer}, \tilde{\outer} \in \argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, and let $\outer^\prime = \lambda \bar{\outer} + (1-\lambda) \tilde{\outer}$ for $\lambda \in [0,1]$. Note that we have $\outer^\prime \in \outerset$ since $\outerset$ is convex for all $\outer \in \outerset$. We then have by the concavity of $\util[\outer]^*$: 
\begin{align}
    \util[\outer]^*(\outer^\prime) &= \util[\outer]^*(\lambda \bar{\outer} + (1-\lambda) \tilde{\outer})\\
    &\geq  \lambda \util[\outer]^*(\bar{\outer} ) + (1-\lambda) \util[\outer]^*(\tilde{\outer})\\ 
    &= \lambda \max_{\outer \in \outerset} \util[\outer]^*(\outer) + (1-\lambda) \max_{\outer \in \outerset} \util[\outer]^*(\outer)\\
    &= \max_{\outer \in \outerset} \util[\outer]^*(\outer)
\end{align}
which means that $\outer^\prime \in \argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, i.e., the set of Stackelberg equilibrium strategies of the outer player is convex. 
\end{proof}

\fi


In general Stackelberg equilibria are not convex, and the broadest conditions known for the set of Stackelberg equilibria to be additionally is that $\util[\outer], \util[\inner], \constr[1], \hdots, \constr[\numconstrs]$ are all affine. \cite{} \deni{Corollary of thm 3.1 of Dempe + convex optimization's solutions being convex property}



\section{Stochastic Stackelberg Games}


\if 0
\begin{itemize}
    \item A discrete set of states $\states$, such that each $\state \in \states$ describes the state in which the game is.
    \item A continuous set of actions $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ for the $\outer$- and $\inner$- players respectively, which denote the actions the players can take throughout the game.
    \item An initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
    \item A reward function $\reward[\outer]: \states \times \outerset \times \innerset \to \R$ (resp. $\reward[\inner]: \states \times \outerset \times \innerset \to \R$) which takes as input the state of the game, the actions of the players, and outputs a reward for the outer (inner) player.
    \item A constraint function $\constr: \states \times \outerset \times \innerset \to \R^\numconstrs$ which denotes the constraints the players' actions have to satisfy in each state. In particular, for each state $\state \in \states$, we require that $(\outer, \inner) \in \outerset \times \innerset$ be picked such that $\constr(\state, \outer, \inner) \geq \zeros$.
    \item A transition function $\trans: \states \times \states \times \outerset \times \innerset \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when actions $\outer \in \outerset$ and $\inner \in \innerset$ are played by the inner and outer player respectively, is denoted by $\trans(\state^\prime \mid \state, \outer, \inner)$.
    \item A discount rate $\discount \in [0,1)$, which can be understood as the probability that the game will continue after an action is played by any player
\end{itemize}
\fi
% We denote a stochastic min-max Stackelberg game by a tuple .



A \mydef{stochastic Stackelberg game} $(\states, \outerset, \innerset, \initstates, \reward[\outer], \reward[\inner], \constr, \trans, \discount)$ is a dynamic two-player sequential, i.e., Stackelberg, game where one player we call the outer- or $\outer$-player  (resp. inner- or $\inner$-player) (or outer and inner players respectively) moves through a set of states $\states$ picking an action to play from their continuous set of actions $\outerset \subset \R^\outerdim$ ($\innerset \subset \R^\innerdim$). Players start the game at an initial state determined by an initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$. At each state the action $\outer \in \outerset$ picked by outer player determines the set of \mydef{feasible} actions $\inner \in \innerset$ such that $\constrs(\outer, \inner)$ that the inner player can in turn play. Once the outer and inner players made their moves they receive rewards $\reward[\outer]: \outerset \times \innerset \to \R$ and $\reward[\inner]: \outerset \times \innerset \to \R$ respectively, then the game either ends with probability $(1-\discount)$, where $\discount \in (0,1)$ is called the \mydef{discount rate}, or transitions to a new state $\state^\prime \in \states$ according to a \mydef{transition} probability function $\trans: \states \times \states \times \outerset \times \innerset \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when actions $\outer \in \outerset$ and $\inner \in \innerset$ are played by the inner and outer player respectively, is denoted by $\trans(\state^\prime \mid \state, \outer, \inner)$.  

The goal of the outer (resp. inner) player is to pick an action at each state given by a \mydef{policy}, i.e., a mapping from states to pobability distributions over actions $\policy[\outer]: \states \to \Delta(\outerset)$ (resp. $\policy[\inner]: \states \to \simplex(\innerset)$) which maximizes their cumulative expected reward.\footnote{We focus on deterministic policies over continuous action spaces which maximizes their cumulative expected reward. A special case of our setting is stochastic policies over discrete action spaces for Stackelberg games with bilinear payoffs.} 
The cumulative reward function for any player $\player \in \players$, $\cumul[\player]: \outerset^\states \times \innerset^\states \to \R$ denotes the total expected reward of the player for given policies of the players and is given by:
\begin{align}
    \cumul[\player](\policy[\outer], \policy[\inner]) = \mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\outer]( \staterv[\iter]), \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]) \right]
\end{align}
For simplicity, we will denote the expected reward for at a particular state under a policy profile $(\policy[\outer], \policy[\inner])$: $$\int_{(\outer,\inner) \in \outerset \times \innerset}  \reward[\player]\left(\state, \outer, \inner\right) d\policy[\outer](\state) d\policy[\inner](\state)$$ simply by $\reward[\player](\state, \policy[\outer](\state), \policy[\inner](\state))$. 
% An \mydef{outcome} of a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ is a policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ consisting of policies for the outer and inner players respectively. 
We require any policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ to be \mydef{feasible}, i.e.,  for all states $\state \in  \states$, and for all actions $(\outer, \inner) \in \outerset \times \innerset$ such that $(\policy[\outer](\state))(\outer) (\policy[\inner](\state))(\inner) > 0$, we require $\constr(\state, \outer, \inner) \geq 0$. For simplicity, we define $\constrs : \simplex(\outerset)^\states \times \simplex(\innerset)^\states \to \R^{\states \times \outerset \times \innerset \times \numconstrs}$ such that $\constrs(\policy[\outer], \policy[\inner]) = ((\policy[\outer](\state))(\outer) (\policy[\inner](\state))(\inner) \constr(\state, \outer, \inner))_{\state, \outer, \inner}$, and define feasible outcomes as those $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ such that $\constrs(\policy[\outer], \policy[\inner]) \geq \zeros$\deni{To improve.}. We define the best response \emph{policy} correspondence of the inner player as $\br(\policy[\outer]) = \argmax_{\policy[\inner] \in \simplex(\innerset)^\states : \constrs(\policy[\outer], \policy[\inner]) \geq \zeros} \cumul[\inner](\policy[\outer], \policy[\inner])$.\footnote{Although the notation for the best-response action  and best-response policy correspondences coincide, the reader can distinguish the two from context and input types to the correspondences.} The relevant solution concept for stochastic Stackelberg games is the \mydef{Stackelberg equilibrium}.

\begin{definition}
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a Stackelberg equilibrium of a stochastic Stackelberg game iff 
\begin{align}
    \cumul[\outer](\policy[\outer]^*, \policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer])} \cumul[\outer](\policy[\outer], \policy[\inner]) && \forall \policy[\outer] \in \simplex(\outerset)^\states\\
    \cumul[\inner](\policy[\outer]^*, \policy[\inner]^*) \geq \cumul[\outer](\policy[\outer]^*, \policy[\inner]) 
    && \forall  \policy[\inner] \in \simplex(\innerset)^\states  \text{ s.t. } \constrs(\policy[\outer]^*, \policy[\inner]) \geq \zeros
\end{align}
\end{definition}
%
\noindent
% \sadie{Should this be $\policy[\outer]^*\in \argmin \max$ and $\policy[\inner]^* \in \argmax$? And why we use $g$ instead of $G$ here?}
\begin{remark}
We note that this is a stronger definition of a Stackelberg equilibrium then is required since we require the constraints $\constr(\state, \policy[\outer], \policy[\inner]) \geq \zeros$ to be satisfied for all states $\state \in \states$. Technically, at a Stackelberg equilibrium it would be enough for the constraints to be satisfied only for states which have a strictly positive probability of being reached by the strategy profile. 
% However, since the game is Markovian, i.e., the transition probabilities and reward function only depend on the current state and action, the actions outputted for states reached by the Stackelberg equilibrium policies with a strictly positive probability are the same under both definitions.
\amy{writing unclear to me}\deni{Fixed!}
\end{remark}

The results we derive in the rest of this paper rely on the two set of assumptions which apply to general-sum and zero-sum settings respectively.
\begin{assumption}\label{assum:stackelberg_general_sum}
1.~$\outerset$ and $\innerset$ are convex 
2.~for all $\outer \in \outerset$, $\util[\inner](\outer, \ \cdot \ ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer, \ \cdot \ )$ are concave, and 
3.~for all $\inner \in \innerset$ $\util[\outer]$ is concave in $\inner$,
4.~with $\reward$ bounded, i.e., $\left\|\reward\right\|_{\infty} \leq \rewardbound < \infty$.
\end{assumption}

\begin{assumption}\label{assum:main}
1.~$\outerset$ and $\innerset$ are convex
2.~For all states $\state \in \states$, $\reward(\state, \cdot, \cdot), \constr[1](\state, \cdot, \cdot), \ldots, \constr[\numconstrs](\state, \cdot, \cdot)$ are continuous and convex-concave;
3.~(Slater's condition) $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\state, \outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$, and
4.~with $\reward$ bounded, i.e., $\left\|\reward\right\|_{\infty} \leq \rewardbound < \infty$.
\end{assumption}


We now define the state-value and action-value functions and analyze their properties. These results will then be used to prove existence of Stackelberg equilibria and the convergence of algorithms to Stackelberg equilibria.

The \mydef{action value function} for each player $\player \in \players$, $\actionvalue[][][][\player]: \states \times \outerset \times \innerset \to \R$, is defined as:
\begin{align}\label{eq:action_value}
    \actionvalue[][][][\player](\state, \outer, \inner; \policy[\outer], \policy[\inner]) = \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty (1- \discount) \discount^\iter \reward[\inner](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\player]( \staterv[\iter]),  \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]), \right. \notag \\ \left. \staterv[0] = \state, \outerrv[0] = \outer, \innerrv[0] = \inner \right]
\end{align}

The \mydef{state-value function} for each player $\player \in \players$, $\statevalue[][][][\player]: \states \times \outerset^\states \times \innerset^\states \to \R$, is given by:
\begin{align}\label{eq:state_value}
    \statevalue[][][][\player](\state; \policy[\outer], \policy[\inner] ) &= \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty (1- \discount)\discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\outer]( \staterv[\iter]), \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]), \staterv[0] = \state \right]\\
    &= \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state); \policy[\outer], \policy[\inner])
\end{align}
\sadie{Do you think we can adopt the notation  $\E^{\policy[]}$ in the note to indicate the expected value given we act according to $\policy[]$. For example, $\statevalue(\state; \policy[\outer], \policy[\inner] ) = \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter])} ^{\policy[\outer]\policy[\inner]}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \staterv[0] = \state \right]$? Will this make the notations more concise?}
% \sadie{For the part under $\E$, should that be $\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])$?}
For clarity, we will often denote the state value and action value function by $\statevalue[][{\policy[\outer]}][{ \policy[\inner]}](\state)$ and $\actionvalue[][{\policy[\outer]}][{ \policy[\inner]}](\state, \outer, \inner)$ respectively. Additionally, we denote $\statevalfuncs  = [-\rewardbound, \rewardbound]^{2 \times \states}$ as the the space of all state value functions of the form $\statevalue: \states \to [-\rewardbound, \rewardbound]^2$, and $\actionvalfuncs = [-\rewardbound, \rewardbound]^{2 \times \times \states \times \outerset \times \innerset}$ as the space of all action value functions $\actionvalue: \states \times \outerset \times \innerset \to [-\rewardbound, \rewardbound]^2$. Note that by \Cref{assum:main} the range of the state and action value functions are $[-\rewardbound, \rewardbound]$.

\if 0
The cumulative reward function for any player $\player \in \players$, $\cumul[\player]: \outerset^\states \times \innerset^\states \to \R$ denotes the total expected reward of the player for given policies of the players and is given by:
\begin{align}
    \cumul[\player](\policy[\outer], \policy[\inner]) = \mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] = \policy[\outer]( \staterv[\iter]), \innerrv[\iter] = \policy[\inner](\staterv[\iter]) \right]
\end{align}
\fi
% For any policy of the outer player $\policy[\outer] \in \outerset$, we define the best-response set of the inner player as $\br(\policy[\outer]) = \argmax_{\policy[\inner] \in \innerset^\states : \constrs(\policy[\outer], \policy[\inner]) \geq \zeros} \cumul[\inner](\policy[\outer], \policy[\inner])$.

We first note the following fundamental relationship between the state-value and action-value functions which is an analog of Bellman’s Theorem \cite{} and which follows from the definitions of \crefrange{eq:state_value}{eq:action_value}:
\begin{theorem}
Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, for all $\player \in \players$, $\statevalue \in \statevalfuncs$, $\actionvalue \in \actionvalfuncs$, $\policy[\outer] \in \outerset^\states$, and $\policy[\inner] \in \innerset^\states$, $\statevalue[][][][\player] = \statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$ 
% \amy{$\statevalue(\state) = \statevalue(\state ;  \policy[\outer], \policy[\inner]) $}
and $\actionvalue[][][][\player] = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$ iff:
\begin{align}
    &\statevalue[][][][\player](\state) = \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state))\label{eq:belman_q_to_v}\\
    &\actionvalue[][][][\player](\state, \outer, \inner) = (1 - \discount) \reward[\player](\state, \outer, \inner) + \discount \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[    \statevalue[][][][\player](\staterv^\prime)  \right] \label{eq:belman_v_to_q}
\end{align}
\end{theorem}

\begin{proof}
By the definition of the state value function we have $\statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player] = \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state))$, hence by \Cref{eq:belman_q_to_v} we must have that $\statevalue[][][][\player] = \statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$. Additionally, by \Cref{eq:belman_v_to_q} and the definition of the action-value functions this also implies that $\actionvalue[][][][\player](\state, \outer, \inner) = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\player](\state, \outer, \inner)$
\end{proof}
% \amy{add proof}
A stronger equilibrium concept for stochastic min-max Stackelberg games would be one that would require that the strategy profile be a Stackelberg equilibrium of each subgame of the stochastic min-max Stackelberg game, aptly called subgame perfect Stackelberg equilibrium. a feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a \mydef{Markov perfect Stackelberg equilibrium} of a stochastic Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward[\outer], \reward[\inner], \constr, \trans, \discount)$ if for all $\state \in \states, \iter \in \N, \statedist[\iter+1](\state) = \sum_{\state^\prime \in \states} \trans(\state \mid \state^\prime, \policy[\outer]^*(\state^\prime), \policy[\inner]^*(\state^\prime)) \statedist[\iter ](\state^\prime)$, $(\policy[\outer]^*, \policy[\inner]^*)$ is a Stackelberg equilibrium of $(\states, \outerset, \innerset, \statedist[\iter], \reward[\outer], \reward[\inner], \constr, \trans, \discount)$. By definition, the set of Markov perfect Stackelberg equilibria of a stochastic min-max Stackelberg game is a subset of the set of Stackelberg equilibria of the game. However, it is not directly clear whether if the inclusion holds the other way round as well. 


\begin{theorem}\label{thm:equiv_def_stackelberg}
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a Stackelberg equilibrium of a stochastic Stackelberg game  $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ iff for all $\state \in \states$ :
\begin{align}
    \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\state) \geq \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner) && \forall \outer \in \outerset \\
    \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\inner](\state) \geq \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\inner](\policy[\outer]^*(\state), \inner)
    && \forall  \inner \in \innerset  \text{ s.t. } \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros
\end{align}
\end{theorem}
% \sadie{for the constraint, should we do $\constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros$ and $\constr(\state, \outer, \inner) \geq \zeros?$}\deni{Fixed, does it look good now?}\sadie{It looks good to me!}
\begin{proof}
($\leftarrow$):
We prove the first inequality, the right hand side follow similarly. For all states $\state \in \states$, we have:
\begin{align}
    \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner) && \forall \outer \in \outerset\\
    \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \sum_{\state \in \states} \initstates[  ](\state) \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner)  && \forall \outer \in \outerset \\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\sum_{\state \in \states} \initstates[  ](\state)  \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]}][\outer](\outer, \policy[\inner](\state))  && \forall \outer \in \outerset\\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\sum_{\state \in \states} \initstates[  ](\state)  \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\outer](\policy[\outer](\state), \policy[\inner](\state))  && \forall \policy[\outer] \in \outerset^\states \\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\cumul(\policy[\outer], \policy[\inner]) && \forall \policy[\outer] \in \outerset^\states 
\end{align}

% \begin{align}
%     \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner)  \\
%     % \max_{\policy[\inner] \in \states^\innerset : \constr(\state, \policy[\outer]^*(\state), \policy[\inner](\state)) \geq 0}
%     \sum_{\state \in \states} \initstates[  ](\state) \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \sum_{\state \in \states} \initstates[  ](\state) \max_{\policy[\inner] \in \states^\innerset : \constr(\state, \policy[\outer]^*(\state), \policy[\inner](\state)) \geq 0} \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]}] \left(\state\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \max_{\policy[\inner] \in \states^\innerset : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros} \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]}] \left(\state\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \max_{\policy[\inner] \in \states^\innerset : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right) 
%     \leq \cumul \left( \policy[\outer]^*, \policy[\inner]^* \right)  
% \end{align}
% Similarly, for the right hand side inequality, for all states $\state \in \states$ we have:
% \begin{align}
%     \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)  \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)
% \end{align}
($\rightarrow$): We prove the first inequality, the right-hand side follows similarly.
\begin{align}
    \policy[\outer]^* &\in \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \cumul[\outer](\policy[\outer], \policy[\inner]) \\
    &\in  \sum_{\state \in \states} \initstates[  ](\state) \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \statevalue[][{\policy[\outer]}][{ \policy[\inner]}] \left(\state\right) \\
    &\in  \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \statevalue[][{\policy[\outer]}][{ \policy[\inner]}] \left(\state\right)
\end{align}
where the second line follows from the Markovian property of the game which ensures that the optimal action in a particular state is independent of the actions taken in other states.
Re-stating the above in terms of action-value function, we get for all states $\state \in \states$:
\begin{align}
    \policy[\inner]^*(\state) &\in \argmax_{\outer \in \outerset} \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) 
\end{align}
% \sadie{I'm a little confused about this step. How did we transfer from $\statevalue[][][]$ to $\actionvalue[][][][]$? When we should use $\constr$ and when we should use $\constrs$?} \deni{add proposition 2.3 for us.} 
% Hence, by the definition of the maximum, we have for all states $\state \in \state$:
% \begin{align}
%     \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) \leq \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state) \right) \leq  \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) 
% \end{align}
\end{proof}


Since the condition given in the above theorem is independent of the initial state distribution of the game, that Stackelberg equilibria are independent of the initial state distribution. As a result, for all $\initstates, {\initstates}^\prime \in [0,1]^\states$, we have that the Stackelberg equilibria of $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ and $(\states, \outerset, \innerset, {\initstates}^\prime, \reward, \constr, \trans, \discount)$ are the same. Hence, a corollary of the above theorem is that in stochastic min-max Stackelberg games, the set of Stackelberg equilibria coincides with the set of subgame perfect Stackelberg equilibria.

\begin{corollary}
The set of Stackelberg equilibria and subgame perfect Stackelberg equilibria coincide in stochastic min-max Stackelberg games.
\end{corollary}

We now move on to investigate the existence properties of Stackelberg equilibria. To this end, we first define the following operators: $\statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states]: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to \statevalfuncs$, $\actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states]: \statevalfuncs \times \outerset^\states \times \innerset^\states \to \actionvalfuncs$, and $\argval[\actionvalfuncs] : \actionvalfuncs \to \outerset^\states \times \innerset^\states$: 
\begin{align}
    \left(\statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states](\actionvalue, \policy[\outer], \policy[\inner])\right)(\state) = \actionvalue(\state, \policy[\outer](\state), \policy[\inner](\state))\label{eq:v_operator}
\end{align}

\begin{align}
    \left(\actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states](\statevalue, \policy[\outer], \policy[\inner])\right)(\state, \outer, \inner) = \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) + \discount \statevalue(\staterv^\prime) \right]\label{eq:q_operator}
\end{align}

\begin{align}
    \argval[\actionvalfuncs](\actionvalue) = \left\{(\policy[\outer]^*, \policy[\inner]^*) 
    % \in \outerset^\states \times \innerset^\states
    \mid  \forall \state,  \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner) \leq \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)  \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)\right\}
\end{align}


% \begin{theorem}
% Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, if there exists $\actionvalue \in \actionvalfuncs$, $\policy[\outer] \in \outerset^\states$, and $\policy[\inner] \in \innerset^\states$ such that
% %
% $\statevalue = \statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states](\actionvalue, \policy[\outer], \policy[\inner])$, 
% %
% $\actionvalue = \actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states](\statevalue, \policy[\outer], \policy[\inner])$,
% %
% and
% $(\policy[\outer],  \policy[\inner]) \in \argval[\actionvalfuncs](\actionvalue)$, then $(\policy[\outer]^*, \policy[\inner]^*)$ is a Stackelberg equilibrium of $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ and we have
% $\statevalue = \statevalue[][{\policy[\outer]}][{\policy[\inner]}]$, $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$.
% %  
% \end{theorem}

% \begin{proof}
% By \Crefrange{eq:v_operator}{eq:q_operator} we have for all states $\state \in \states$:
% \begin{align}
%     &\statevalue[](\state) = \actionvalue[](\state, \policy[\outer](\state), \policy[\inner](\state))\\
%     &\actionvalue[](\state, \outer, \inner) = \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right]
% \end{align}
% Therefore, by \Cref{thm:bellman}, we have that $\statevalue = \statevalue[][{\policy[\outer]}][{\policy[\inner]}]$, $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$. Additionally, by 
%  \Cref{thm:equiv_def_stackelberg} and the definition of $\argval[\actionvalfuncs](\actionvalue)$, we know that $(\policy[\outer],  \policy[\inner])$ is a Stackelberg equilibrium.
% \end{proof}

% Using the above, we construct a function $\policyfp: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to  \actionvalfuncs \times \outerset^\states \times \innerset^\states$ such that $\policyfp = \left(I \times \argval[\actionvalfuncs]\right) \circ \actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states] \circ \statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states]$ where $I$ is the identity operator. The following corollary of \Cref{thm:bellman} applies to to $\policyfp$:

% \begin{corollary}\label{corr:fp_stackelberg}
% Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, if there exists a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$, then $(\policy[\outer], \policy[\inner])$ is a Stackelberg equilibrium, and $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$.
% \end{corollary}



% \begin{lemma}
% The set of Stackelberg equilibria of any min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$ is non-empty, compact, and convex.
% \end{lemma}
% \begin{proof}
% By proposition B.2 from \cite{goktas2021minmax}, the set of Stackelberg equilibria of any min-max Stackelberg game is non-empty. Additionally, under \Cref{assum:main}, we have that for all $\outer \in \outers$, $\obj(\outer, \cdot)$ is concave, and $\{\inner \innerset \mid \constr(\outer, \inner) \geq \zeros\}$ is convex. Hence, by \cite{} the set of solutions $\outerset^*(\outer) = \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is compact- and convex- valued.
% %
% Similarly, under \Cref{assum:main}, by proposition B.1 from \cite{goktas2021minmax}, $\max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is continuous and convex. Hence, the set of solutions $\innerset^* = \argmin_{\outer \in \outerset} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is compact- and convex-valued. Since the carthesian product of two compact-convex-valued correspondences is compact-convex-valued, we have that the set of Stackelberg equilbiria $\outerset^*\left(\innerset^*\right)$ is also compact-convex-valued.
% \end{proof}

% \begin{corollary}
% The correspondence $\argval[\actionvalfuncs]$ is non-empty-, compact-, convex-valued.
% \end{corollary}

% \begin{proof}
% For any $\actionvalue \in \actionvalfuncs$ and for all states $\state \in \states$, we have that $\left( \argval[\actionvalfuncs](\actionvalue) \right)(\state)$ is the set of Stackelberg equilibria of the min-max Stackelberg game $(\outerset, \innerset, \actionvalfuncs, \constr(\state, \cdot, \cdot))$ which is non-empty-compact-convex-valued. Hence, $\argval[\actionvalfuncs](\actionvalue)$ must be non-empty-compact-convex valued as well since it is the product of multiple non-empty-compact-convex sets.
% \end{proof}

% \begin{lemma}\label{lemma:fp_existence}
% The correspondence $\policyfp$ has a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$.
% \end{lemma}
% \begin{proof}
% $\policyfp: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to \actionvalfuncs \times \outerset^\states \times \innerset^\states$ is non-empty-, and convex-valued. It is also compact-valued, i.e., its graph is closed. Hence, by Kakutani's fixed point a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$ exists.
% \end{proof}

% \amy{Deni's conjecture: we don't need to assume boundedness in zero-sum games, only in non-zero-sum games}

% Combining \Cref{lemma:fp_existence} and \Cref{corr:fp_stackelberg}, we obtain:
\begin{theorem}\label{thm:stackelberg_existence}
Any stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ has at least one Stackelberg equilibrium 
\end{theorem}

\begin{proof}
Let $\calK = \statevalfuncs \times \simplex(\outerset)^\states \times \simplex(\innerset)^\states$.  Note that since $\calK$ is a carthesian product of compact convex sets, it is also compact convex set (of a locally convex space).
Consider a correspondence $\fp: \left(\v, \policy[\outer], \policy[\inner] \right) \in \left(\calK \right) \rightrightarrows (\w(\v, \policy[\outer], \policy[\inner]), \phi(\v, \policy[\outer], \policy[\inner])))$ where $\w, \phi$ are defined respectively as:

\begin{align}
    w_\outer\left(\v, \policy[\outer], \policy[\inner] \right)(\state) = \max_{\policy \in \simplex(\outerset)^\states} \left[  \reward[\outer](\state, \policy(\state), \policy[\inner](\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy(\state) d\policy[\inner](\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states\\
    w_\inner\left(\v, \policy[\outer], \policy[\inner] \right)(\state) = \max_{\policy \in \simplex(\innerset)^\states : \constrs(\policy[\outer], \policy) \geq \zeros} \left[  \reward[\inner](\state, \policy[\outer](\state), \policy(\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy[\outer](\state) d\policy[](\state)  \statevalue[][][][\inner](\state^\prime)\right] && \forall \state \in \states\\\
    \phi_\outer(\v, \policy[\outer], \policy[\inner])(\state) = \argmax_{\policy \in \simplex(\outerset)^\states} \left[  \reward[\outer](\state, \policy(\state), \policy[\inner](\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy(\state) d\policy[\inner](\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states\\
    \phi_\inner(\v, \policy[\outer], \policy[\inner])(\state) = \argmax_{\policy \in \br(\policy[\outer])} \left[  \reward[\outer](\state, \policy[\outer](\state), \policy(\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy[\outer](\state) d\policy(\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states
\end{align}

Note that the objective of all of the optimization problems above are linear in their inputs since they are the sum of two expectations. Hence, by \Cref{assum:stackelberg_general_sum} since $\constr(\state, \outer, \inner)$ is convex in $\inner$ for all $\state \in \states$, Berge's maximum theorem  \cite{berge1997topological} applies and we have that $\w\left(\v, \policy[\outer], \policy[\inner] \right)$ is continuous. Similarly, since $\simplex(\outerset)^\states$ is compact, by Berge's maximum theorem $\phi_\outer$ is upper hemicontinuous and convex-valued.

Note that by Berge's maximum theorem under \Cref{assum:stackelberg_general_sum}, $\br$ is upper hemicontinuous, and nonempty-compact valued.
Hence, by theorem 4.2.1 of \citeauthor{bank1983non} \cite{bank1983non} since the best-response correspondence is upper hemicontinuous and the marginal function of the outer player is upper semicontinuous, $\phi_\outer$ must be upper hemicontinuous.

Hence, by Kakutani's fixed point theorem a fixed point of $\fp$ exists.
% \begin{align}
% \fp
% \begin{pmatrix}
%     \statevalue[][][][\outer]\\
%     \statevalue[][][][\inner]\\
%     \policy[\outer]\\
%     \policy[\inner]
% \end{pmatrix}
% =
% \begin{pmatrix}
%     \max_{\policy \in \simplex(\outerset)^\states} \left\{ \reward(\state) \right\}\\
%     \statevalue[][][][\inner]\\
%     \policy[\outer]\\
%     \policy[\inner]
% \end{pmatrix}
% \end{align}
\end{proof}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/intro.tex <==
Min-max optimization has paved the way for recent progress in a variety of fields, from machine learning to economics.
In a \mydef{constrained min-max optimization problem},
% \samy{(with independent constraint sets)}{}\amy{i think this clause only makes sense to us!},
%\amy{are we sure we want to say that we ``solve an operator,'' as opposed to a problem?}\deni{With the new phrasing of this paragraph, I think I agree this change makes sense!}
%\deni{I feel like we should already call it a game in some way so that it is clear without the abstract. Also, I prefer the term zero-sum game, because they're not called min-max stochastic games but zero-sum stochastic games, so that everything connects nicely.}
$\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner)$, the objective function $\obj: \outerset \times \innerset \to \R$ is continuous, and the constraint sets $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ are nonempty and compact.
When $\obj$ is convex-concave, and the constraint sets $\outerset$ and $\innerset$ are convex, the seminal minimax theorem \cite{neumann1928theorie, sion1958general} holds, i.e., $\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner) = \max_{\inner \in \innerset} \min_{\outer \in \outerset} \obj(\outer, \inner)$, and such problems can be interpreted as solving a \mydef{min-max} (or \mydef{zero-sum}) one-shot \emph{simultaneous-move\/} \mydef{game} 
%\sdeni{(with independent action sets)}{}
%\deni{A simultaneous-move game always has independent strategy sets, as otherwise it would be a pseudo-game!}
between an \mydef{outer player} $\outer$ and an \mydef{inner player} $\inner$ with respective payoff functions $-\obj$, $\obj$ and respective action sets $\outerset$, $\innerset$, where the solutions $(\outer^*, \inner^*) \in \outerset \times \innerset$ 
% \samy{of the min-max operator}{}\amy{we are no longer solving an operator} \samy{correspond to a Nash equilibrium, i.e., strategies which}{}
are \mydef{Nash equilibria}: i.e., \mydef{best responses} to one another with $\outer^* \in \argmin_{\outer \in \outerset} \obj(\outer, \inner^*)$ and $\inner^* \in \argmax_{\inner \in \innerset} \obj(\outer^*, \inner)$.

More generally, one can consider \mydef{zero-sum stochastic games} played over an infinite discrete time horizon $\N_+$.
%\deni{I saw this term in \url{https://link.springer.com/content/pdf/10.1007\%2F978-3-319-27335-8\_8-1.pdf} and I really like it because essentially what we are solving is still an MDP, but with a different operator instead. Like we call them min-max optimization problems, but idk, if you prefer that it makes sense!} ok!ok!
%\amy{i don't disagree, but it is not Shapley's terminology. i think it is better to stick with Shapley's terminology, which was stochastic game, since Shapley is the one whose results you are citing here.}
%\amy{you could introduce this new min-max MDP terminology, and add a footnote that Shapley called these stochastic games. but no -- b/c we want to say "stochastic Stackelberg game" later, not Stackelberg MDP.}\deni{but to be fair, I call it min-max MDP with dependent strategy set!}
%fine...but redundant...
%in which two players play state-dependent min-max games as they traverse a set of states $\state[1], \state[2], \ldots, \in \states$.
The game starts at some initial state $\staterv[0] \sim \initstates$. 
%\amy{$\state[0] \sim \initstates$?}\deni{I think here the state is clearly a random variable so I want it to be a capital letter to be consistent with the rest of the paper. For the next few sentences, the state was encountered, i.e., realized hence why it is lower case. Happy to explain this more in person but this is what I converged to after some self-debate.}
At each subsequent time-step $\iter \in \N_+$, players encounter a new state $\state[\iter] \in \states$.
After taking their respective actions $(\outer[\iter], \inner[\iter])$ from their respective action spaces $\outerset(\state[\iter]) \subseteq \R^\outerdim$ and $\innerset(\state[\iter]) \subseteq \R^\innerdim$,
% \deni{I want to now remove this dependence from here too because we are saying the actions of each player depends on the state which is a random variable but the writing down the actions of the players as random variables complicates presentation!!! We should just remove it and add a footnote, does that work?}
they receive payoffs $\reward (\state[\iter], \outer[\iter], \inner[\iter])$, and then either transition to a new state $\staterv[\iter+1] \sim \trans (\cdot \mid \state[\iter], \outer[\iter], \inner[\iter])$ with probability $\discount$, or the game ends with the remaining probability.
The goal of the outer (resp.{} inner) player is to play  
%\sdeni{policy $\policy[\outer]: \states \to \outerset$ (resp.{} $\policy[\inner]: \states \times \innerset$)}
a (\mydef{non-stationary}) \mydef{policy}, i.e., a sequence of history-dependent actions $\{\outer[\iter]\}_{\iter = 0}^\infty$ (resp.{} $\{\inner[\iter]\}_{\iter = 0}^\infty$),
%\deni{Technically the goal of the players is to play a non-stationary policy, but I am afraid that writing it that way will complicate things, what are you thoughts?} \amy{just write it in English, not math. define a policy as a function from game histories to actions. and don't write $\policy[\outer] (\staterv)$ or $\policy[\inner] (\staterv)$ yet} \deni{Made some edits, I think I was able to do this without discussing any notion of a policy?} 
that maximizes (resp.{} minimizes) their expected cumulative discounted payoff (resp. loss) $\mathop{\Ex} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outer[\iter], \inner[\iter]) \right]$, fixing their opponent's policy. 

Note that any zero-sum stochastic game can be (non-compactly) represented as a zero-sum one-shot game with objective function $\mathop{\Ex} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outer[\iter], \inner[\iter]) \right]$ and action sets comprising sequences $ \prod_{t=0}^\infty \outerset$ and $ \prod_{t=0}^\infty \innerset$ for the outer and inner players, respectively.
Although the traditional minimax theorem \cite{neumann1928theorie, sion1958general} does not hold in these games, because this objective function is not convex-concave in these actions, \citeauthor{shapley1953stochastic} nonetheless establishes the existence of Nash equilibria \cite{shapley1953stochastic},
by deriving a more general minimax theorem.

% .i.e., Bellman equations $\statevalue (\staterv) = \min_{\outer \in \outerset} \max_{\inner \in \innerset} \left\{ \obj (\staterv, \outer, \inner) + \gamma \E_{\staterv^\prime \sim \trans(\cdot \mid \staterv, \outer, \inner)} \statevalue (\staterv^\prime) \right\}$ with unknown $\statevalue$
% i.e., $\min_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states} \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \policy[\outer](\staterv[\iter]), \policy[\inner](\staterv[\iter]))} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \policy[\outer](\staterv[\iter]), \policy[\inner](\staterv[\iter])) \right] $ where $\reward (\staterv, \outer, \inner)$ is a state-dependent function, for all states $\staterv \in \states$, $\discount \in (0, 1)$ is a discount factor, and $\trans(\staterv^\prime \mid \staterv, \outer, \inner)$ is a transition function.
% A solution to a zero-sum stochastic game is a \mydef{policy profile} $\policy = (\policy[\outer], \policy[\inner])$ which consists of \mydef{policies} $\policy[\outer]: \states \to \outerset$ and $\policy[\inner]: \states \to \innerset$ for the outer and inner players respectively such that $\min_{\policy[\outer] \in \outerset^\states} \max_{\policy[\outer] \in \outerset^\states} \mathop{\E^{\policy[\outer], \policy[\inner]}}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \right]$ }
% \deni{I see you removed the Bellman equation math but to me that is very important. On its own, your description does not tell us that in stochastic games we are trying to maximize the cumulative utility across all states. Also this does not even define what a state is, it is quite unclear. I feel like the previous formalism was shorter and clearer. I feel strongly about this bc right now the description does not tell us what is the objective is stochastic games at all!! Also, I state our Fisher market SSG as a Bellman equation, so I would love that understanding to be conveyed from the get-go. The way this is stated right now, it makes no sense why call it recursive NE/SE, where is the recursiveness?}

%\amy{i dropped the parens around stationary, and added non-stationary above. so now there are two defined types of policies, meaning the word policy is no longer reserved only for mappings from states to actions. that is specifcally a \emph{stationary} policy.} 

A \mydef{stationary} (or \mydef{Markovian~\cite{maskin2001markov}}) \mydef{policy} is a mapping from states to actions.
%We denote a stationary policy for the outer (resp.{} inner) player by $\policy[\outer]: \states \to \outerset$ ($\policy[\inner]: \states \to \innerset$).
When $\reward (\state, \outer, \inner)$ is bounded, continuous, and concave-convex in $(\outer, \inner)$, for all $\state \in \states$, 
we are guaranteed the existence of a stationary policy profile, i.e., a pair of stationary policies $\policy[\outer]: \states \to \outerset$, $\policy[\inner]: \states \to \innerset$ for the outer and inner players, respectively, specifying the actions taken at each state, with a unique value such that both players maximize their expected payoffs, as a generalization of the minimax theorem holds \cite{shapley1953stochastic}:%
\footnote{Shapley's original results, which concern state-dependent payoff functions that are bilinear in the outer and inner players' actions, extend directly to payoffs which are convex-concave in the players' actions.}
\vspace{-5mm}

{\small
\begin{align*}
\min_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states} \mathop{\E} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \policy[\outer](\staterv[\iter]), \policy[\inner](\staterv[\iter])) \right]
&= \max_{\policy[\inner] \in \innerset^\states} \min_{\policy[\outer] \in \outerset^\states}  \mathop{\E} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \policy[\outer](\staterv[\iter]), \policy[\inner](\staterv[\iter])) \right]
\end{align*}}

\vspace{-2mm}
In other words, under the aforementioned assumptions, we are guaranteed the existence of a \mydef{recursive Nash equilibrium} (sometimes called Markov perfect equilibrium \cite{maskin2001markov}, a refinement of extensive-form game subgame perfect equilibrium for Markov games), namely a stationary policy profile in which players not only play Nash equilibria: i.e., best responses to one another, but do so regardless of initial state.
%\amy{i think i like ``regardless of initial conditions'' better, b/c it suggests ``in a history-independent way''.}
%%% MPE: best responses at any state of the game, i.e., best-responses independent of the original distribution 
%\sdeni{}{, a consequence of Bellman's principle of optimality \cite{bellman1952theory} applied to both sides of the above equality}.
% , in which two players travel through a set of states $\states$, and at each state $\state \in \states$ the outer and inner players take respectively actions $(\policy[\outer](\state), \policy[\inner](\state))$ which are long term best-responses to one another, receive rewards $\reward(\state, \policy[\outer](\state), \policy[\inner](\state))$, and either transition to a new state $\state^\prime \sim \trans(\cdot \mid \state, \policy[\outer](\state), \policy[\inner](\state))$, or the game ends with a probability of $(1-\discount)$. Note that at a recursive Nash equilibrium, both players maximize their expected cumulative rewards.
Additionally, when the rewards at each state are convex-concave, a recursive Nash equilibrium can be computed in polynomial time by iterative application of the min-max operator  \cite{shapley1953stochastic}.
Zero-sum \emph{stochastic\/} games generalize zero-sum games from a single state to multiple states, and have found even more applications in a variety of fields \cite{jaskiewicz2018non}. 

When the objective function in a min-max optimization problem is not convex-concave, a minimax theorem is not guaranteed to hold, precluding the interpretation of the game as simultaneous-move, and the guaranteed existence of Nash equilibrium.
Nonetheless, the optimization problem can still be viewed as a min-max (or zero-sum) one-shot \emph{Stackelberg\/} game, in which the outer player moves before the inner one.
The canonical solution concept in such games is \mydef{Stackelberg equilibrium (SE)}.
%Such optimization problems are better seen as two-player sequential, i.e., \mydef{Stackelberg \cite{stackelberg1934marktform} games}, and their solutions, as \mydef{Stackelberg equilibria (SE)}, since the order in which the players move affects the optimal value of the problem.
Interestingly, in Stackelberg games, the inner player's actions can be constrained by the outer player's choice, without impacting existence~\cite{goktas2021minmax}.
The result is a \mydef{min-max one-shot Stackelberg game}: i.e., $\min_{\outer \in \outerset} \max_{\inner \in \innerset: h(\outer, \inner) \geq \zeros} \obj (\outer, \inner)$, where $\obj, h: \outerset \times \innerset \to \R$ are continuous, and $\outerset, \innerset$ are non-empty and compact.
Even more problems of interest are captured by this model \cite{bertsimas2011theory,  fisac2015reach, bansal2017hamilton, leung2022learning}.
%\sdeni{However, a minimax theorem is not guaranteed to hold in this setting; as a result, these problems are best interpreted as zero-sum sequential, i.e., Stackelberg \cite{stackelberg1934marktform}, games, and their solutions, as Stackelberg equilibria.}{}
%Similar to the \samy{independent strategy set}{stochastic game} setting,

One can likewise consider \mydef{zero-sum stochastic Stackelberg games}, which generalize both zero-sum one-shot Stackelberg games and zero-sum stochastic (simultaneous-move) games.
Similar to zero-sum stochastic games, 
%\samy{}{though not necessarily simultaneous-move,} 
these games are played over an infinite discrete time horizon $\N_+$, start at some state $\staterv[0] \sim \initstates$ and consist of nonempty and compact actions spaces $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$% 
%state-dependent actions spaces $\outerset\sdeni{}{(\state)} \subset \R^\outerdim$ and $\innerset\sdeni{}{(\state)} \subset \R^\innerdim$%
\footnote{To simplify notation, we drop the dependency of action spaces on states going forward, but our theory applies in this more general setting.},
%to this setting in a straightforward fashion
%i.e., Bellman equations $\statevalue(\state) = \min_{\outer \in \outerset} \max_{\inner \in \innerset: \constr(\state, \outer, \inner) \geq \zeros} \left\{ \obj(\outer, \inner) + \gamma \E_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)}\statevalue(\staterv^\prime) \right\}$ with unknown $\statevalue$. 
a state-dependent payoff function
$\reward (\state, \outer, \inner)$, a transition probability $\trans(\state^\prime \mid \state, \outer, \inner)$, and a discount rate $\discount$.
In addition, they are augmented with a state-dependent (joint action) constraint function $\constr(\state, \outer, \inner)$,
% \sadie{why we are using $h$ and $g$ both for constraints?}\deni{$h$ is for the static constraints with not state $g$ is for the dynamic constraints which take as input a state!}\sadie{Oh I see! Thank you!}
with two players that seek to optimize their cumulative discounted payoffs, in expectation, while satisfying the constraint $\constr(\state, \outer, \inner) \geq \zeros$ at each state $\state \in \states$.
Applications of this model include autonomous driving \cite{fisac2015reach, leung2022learning}, reach-avoid problems in human-robot interaction \cite{bansal2017hamilton}, and robust optimization in stochastic environments \cite{bertsimas2011theory}, 
\deni{Double check if there are more papers to add!.}
and, as we show, economic markets.

%\amy{wait a sec! how is this the canonical solution concept if we are making it up?!}\deni{Okay thanks for noticing this, this has clarified my thinking.}
\deni{Here is the new story: at a high level, while in a stochastic game, players pick policies *before the start of the game* simultaneously, in stochastic Stackelberg games, a leader picks a policy first, and then the follower pick a best response policy *before the start of the game*. Our goal then becomes to investigate if playing stochastic Stackelberg game, can be seen as equivalent to playing a Stackelberg game at each state of the game, i.e., does \recSE{} or Markov perfect Stackelberg equilibrium exist.}

While in stochastic games, players announce their policies simultaneously before play commences, in stochastic Stackelberg games, the outer player, 
%hereafter the leader\deni{If you agree with this change, I will make the leader/follower change everywhere!},\amy{we can make this change another time. before the official posting after the conference, if we decide we want to}
announces their policy first, after which the inner player announces theirs.
% \deni{Once again, with now the Bellman equation removed, it is not clear what is the difference between SSG and Stochastic games.}
The canonical solution concept for such games is the \mydef{Stackelberg equilibrium}, which is guaranteed to exist in non-stationary policies under mild assumptions \cite{goktas2021minmax,vorobeychik2012computing}.
The computational complexity of such policies, however, can be prohibitive, since even representing such policies in an infinite horizon setting is intractable.
A natural question to ask, then, is whether \emph{stationary\/} equilibria exist in zero-sum Stackelberg games, i.e., stationary policy profiles in which, starting at any state of the game, the outer player maximizes their expected discounted cumulative payoff while the inner player best responds.
Following the analogous Nash nomenclature, we call such policies \mydef{recursive Stackelberg equilibria (\recSE{})} (or Markov perfect Stackelberg equilibria).

In this paper, we define and prove the existence of \recSE{} in zero-sum stochastic Stackelberg games, provide necessary and sufficient conditions for a policy profile to be a \recSE, and show that a \recSE{} can be computed in (weakly) polynomial time via value iteration.
We further show that zero-sum stochastic Stackelberg games can be used to solve problems of pricing and allocating goods across agents and time.
In particular, we introduce \mydef{stochastic Fisher markets}, a stochastic generalization of the Fisher market \cite{brainard2000compute}, and a special case of \citeauthor{Friesen1979stochastic}'s \cite{Friesen1979stochastic} financial market model, which itself is a stochastic generalization of the \citeauthor{arrow-debreu} model of a competitive economy \cite{arrow-debreu}.
We then prove the existence of recursive competitive equilibrium (recCE) \cite{mehra1977recursive} in this model, under the assumption that consumers have continuous and homogeneous utility functions, by characterizing the recCE of any stochastic Fisher market as the recSE of a corresponding zero-sum stochastic Stackelberg game.
Finally, we use value iteration to solve various stochastic Fisher markets, highlighting the issues that value iteration can encounter, depending on the smoothness properties of the
%%% SPACE
%utility functions. 
utilities.
%\deni{We have not defined reward function, how to refer to this?}\amy{we used utility function in the previous sentence. can't you say utility here as well?}\deni{I think for clarity let's say that but really it is that every utility function defines some reward function whose smoothness properties in return define the properties of the problem.}
% 
\if 0
%%% SPACE
We summarize our contributions as follows:
%
\begin{itemize}

    \item We prove the existence of recursive Stackelberg equilibrium in min-max stochastic Stackelberg games with dependent strategy sets under the assumptions that the payoff function is continuous and bounded at each state. (\Cref{thm:existence_stackelberg}). 
    
    \item We prove a subdifferential generalization of the Benveniste-Scheinkman theorem \cite{Benveniste1979value}, which allows us to subdifferentiate parametrized Bellman equations (\Cref{thm:subdiff_bellman}).
    
    \item Using our subdifferential version of the Benveniste-Scheinkman theorem (\Cref{thm:subdiff_bellman}), we provide necessary conditions for a policy profile to be a Stackelberg equilibrium of a stochastic Stackelberg game, assuming the payoff function is concave in the outer player's action at each state (\Cref{thm:necessary_conditions}).
    These conditions become sufficient when, in addition, the payoff function is concave in the inner player's action (\Cref{thm:necessary_sufficient_conditions}).
    
    \item We introduce stochastic Fisher markets, and provide a constructive proof of existence of recursive competitive equilibria assuming buyers with continuous and homogeneous utility functions by showing that such stochastic Fisher markets are an instance of a stochastic Stackelberg game (\Cref{thm:fisher_market_recursive_eqm}).
    
    \item We solve for a recursive competitive equilibrium in various stochastic Fisher markets using value iteration, highlighting the issues that value iteration might face as a consequence of the smoothness properties of the utility functions.
\end{itemize}
\fi
% 

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

\paragraph{Notation} 
We use caligraphic uppercase letters to denote sets (e.g., $\calX$);
% calligraphic uppercase letters to denote correspondences (e.g., $\calX$),
%\amy{what about correspondences? see commented out bit just here} \deni{I use caligraphic letters! Essentially mappings' letters are defined by the type of their outputs'}
bold lowercase letters to denote vectors (e.g., $\price, \bm \pi$);
bold uppercase letters to denote matrices and vector-valued random variables (e.g., $\allocation$, $\bm \Gamma$)---which one should be clear from context;
lowercase letters to denote scalar quantities (e.g., $x, \gamma$);
and uppercase letters to denote scalar-valued random variables (e.g., $X, \Gamma$).
%
We denote the $i$th row vector of a matrix (e.g., $\allocation$) by the corresponding bold lowercase letter with subscript $i$ (e.g., $\allocation[\buyer])$. 
Similarly, we denote the $j$th entry of a vector (e.g., $\price$ or $\allocation[\buyer]$) by the corresponding Roman lowercase letter with subscript $j$ (e.g., $\price[\good]$ or $\allocation[\buyer][\good]$).
We denote functions by a letter:
%with the type determined by the value of the functions
e.g., $f$ if the function is scalar valued, and $\f$ if the function is vector valued.
We denote the vector of ones of size $\numbuyers$ by $\ones[\numbuyers]$.
We denote the set of integers $\left\{1, \hdots, n\right\}$ by $[n]$, the set of natural numbers by $\N$, the set of real numbers by $\R$. We denote the postive and strictly positive elements of a set by a $+$ and $++$ subscript respectively, e.g., $\R_+$ and $\R_{++}$. 
% the set of positive natural numbers by $\N_+$ , the set of non-negative real numbers by $\R_+$, and the set of strictly positive real numbers by $\R_{++}$.
We denote the orthogonal projection operator onto a set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|^2$. We denote by $\simplex[n] = \{\x \in \R_+^n \mid \sum_{i = 1}^n x_i = 1\}$, and by $\simplex(A)$, the set of probability measures on the set $A$.

\deni{Should we stick to the outer, inner player language or should we instead embrace the leader-follower language since in the stochastic setting the problem "looks less" inner-outer?}
\amy{leader follower, but another time!}

A \mydef{stochastic Stackelberg game} $(\states, \outerset, \innerset, \initstates, \reward[\outer], \reward[\inner], \constr, \trans, \discount)$ is a two-player game played over an infinite discrete time horizon $\N_+$.
%\deni{I saw this term in \url{https://link.springer.com/content/pdf/10.1007\%2F978-3-319-27335-8\_8-1.pdf} and I really like it because essentially what we are solving is still an MDP, but with a different operator instead. Like we call them min-max optimization problems, but idk, if you prefer that it makes sense!} ok!ok!
%\amy{i don't disagree, but it is not Shapley's terminology. i think it is better to stick with Shapley's terminology, which was stochastic game, since Shapley is the one whose results you are citing here.}
%\amy{you could introduce this new min-max MDP terminology, and add a footnote that Shapley called these stochastic games. but no -- b/c we want to say "stochastic Stackelberg game" later, not Stackelberg MDP.}\deni{but to be fair, I call it min-max MDP with dependent strategy set!}
%fine...but redundant...
%in which two players play state-dependent min-max games as they traverse a set of states $\state[1], \state[2], \ldots, \in \states$.
At each time-step $\iter \in \N_+$, the players, who we call the outer- (resp.{} inner-) players, encounter a new state $\state \in \states$, and choose an action to play from their continuous set of actions $\outerset \subset \R^\outerdim$ (resp.\ $\innerset \subset \R^\innerdim$).
Play initiates at a start state $\staterv[0]$ drawn from a distribution $\initstates: \states \to [0, 1]$.
At each state $\state \in \states$ the action $\outer \in \outerset$ chosen by the outer player determines the set of \mydef{feasible} actions $\{\inner \in \innerset \mid \constr(\state, \outer, \inner) \geq \zeros \}$ available to the inner player, where $\constr: \states \times \outerset \times \innerset \to \R^\numconstrs$.
After the outer and inner players both make their moves, they receive payoffs 
%\amy{isn't payoff a better term than rewards, since one player is maximizing and the other minimizing?}\deni{Incredible point!!!}
$\reward[\outer]: \states \times \outerset \times \innerset \to \R$ and $\reward[\inner]: \states \times \outerset \times \innerset \to \R$, respectively, and the game either ends with probability $1-\discount$, where $\discount \in (0,1)$ is called the \mydef{discount factor}, or transitions to a new state $\state^\prime \in \states$, according to a \mydef{transition} probability function $\trans: \states \times \states \times \outerset \times \innerset \to [0,1]$ s.t.\ $\trans(\state^\prime \mid \state, \outer, \inner) \in [0,1]$ denotes the probability of transitioning to state $\state^\prime \in \states$ from state $\state \in \states$ when action profile $(\outer, \inner) \in  \outerset \times \innerset$ is chosen by the players.

% The goal of the outer (resp. inner) player is to pick an action at each state given by a \mydef{policy}, i.e., a mapping from states to probability distributions over actions $\policy[\outer]: \states \to \Delta(\outerset)$ (resp. $\policy[\inner]: \states \to \simplex(\innerset)$) which maximizes for $\player \in \{\outer, \inner\}$ the cumulative expected reward 
% $
%      \mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \state[\iter],\outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\outer]( \staterv[\iter]), \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]) \right]
% $

In this paper, we focus on \mydef{zero-sum} stochastic Stackelberg games 
% \amy{introduce some shorthand for a stochastic Stackelberg game, like $G$ or $\Gamma$, so you don't have to list the entire tuple every time you want to say, ``Given a game $G$,''}
$\initgame \doteq (\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, 
%a specialization of the more general setting
in which the outer player's loss is the inner player's gain, i.e., $\reward[\outer] = -\reward[\inner]$. 
% \deni{Later on I drop the initial state distribution because Stackelberg equilibria of games with different initial state distributions are the same, have to make sure to mention it.} 
%\sdeni{We say that a zero-sum stochastic Stackelberg game is \mydef{convex-concave} if, for all $\state \in \states$, $\reward(\state, \outer, \inner), \constr[1](\state, \outer, \inner), \hdots, \constr[\numconstrs](\state, \outer, \inner)$ are convex-concave in $(\outer, \inner)$.}{} 
% As we will show, in the zero-sum case, as opposed to the general-sum setting, 
A zero-sum stochastic Stackelberg game reduces to zero-sum (simultaneous-move) stochastic game \cite{shapley1953stochastic} in the special case where $\constr(\state, \outer, \inner) \geq 0$, for all state-action tuples $(\state, \outer, \inner) \in \states \times \outerset \times \innerset$.
%\samy{As we will show, it suffices to focus on stationary
%\deni{Not deterministic, b/c: If we take the action space to be the probability simplex these policies are not deterministic in a discrete action stochastic Stackelberg game.}
%policies in which a \mydef{policy} for the outer (resp.\ inner) player is a mapping from states to actions $\policy[\outer]: \states \to \outerset$ (resp.\ $\policy[\inner]: \states \to \innerset$).}{}
% \footnote{We focus on deterministic policies over continuous action spaces. A special case of our setting is stochastic policies over discrete action spaces for Stackelberg games with bilinear payoffs.} 
%The \mydef{outcome} of a zero-sum stochastic Stackelberg game $\initgame$
%$(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ is a policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ consisting of policies for the outer and inner players, respectively.
%\deni{I think an outcome of the model is actually a non-stationary policy, and I do not want to define that so I think we are better off not definining an outcome, it is not used anywhere anyways}
More generally, a policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ is said to be \mydef{feasible} if $\constr(\state, \policy[\outer](\state), \policy[\inner](\state)) \geq 0$, for all states $\state \in \states$.
To simplify notation, we introduce a function $\constrs : \outerset^\states \times \innerset^\states \to \R^{\numstates \times \numconstrs}$ such that $\constrs(\policy[\outer], \policy[\inner]) = (\constr(\state, \policy[\outer](\state), \policy[\inner](\state)))_{\state \in \states}$, and define feasible policy profiles as those $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ s.t.\ $\constrs(\policy[\outer], \policy[\inner]) \geq \zeros$.
From now on, we assume:

\begin{assumption}
\label{assum:main}
1.~For all states $\state \in \states$, the functions $\reward (\state, \cdot, \cdot), \constr(\state, \cdot, \cdot)$ are continuous in $(\outer, \inner) \in \outerset \times \innerset$,
and payoffs are bounded, i.e., $\left\| \reward \right\|_{\infty} \leq \rewardbound < \infty$, for some $\rewardbound \in \R_{+}$,
2.~$\outerset, \innerset$ are non-empty and compact, and for all $\state \in \states$ and $\outer \in \outerset$ there exists $\inner \in \innerset$ s.t.\ $\constr(\state, \outer, \inner) \geq \zeros$.%
\footnote{Note that this condition is weaker than Slater's condition; it simply ensures the feasible action sets are non-empty for the inner player at each state.}
%\deni{range is $\R_+$ which is implied because the norm is always greater than zero and alpha is less than $\infty$}

% 3.~(Slater's condition) $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\state, \outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$,\deni{Remove Slater's condition bc I added it to thms that need it bc not all of them need it?}
% and 
% 3.~$\outerset, \innerset$ are convex sets.\deni{Add differentiability maybe here to make things shorter?}
\end{assumption} 
% \deni{Need irreducibility assumption or a communication class type of definition.}
% \sadie{I think maybe we still need all states in *feasible* definition since we have no information about the starting state, and it can be every state. But if we know the starting state (in some sense), we can use $\state\in \reachstates{\state}$.}\deni{I've come to the conclusion that this will complicate things too much, check out my new addition under the definition of Stackelberg equilibrium.}

Given a zero-sum stochastic Stackelberg game $\initgame$, the \mydef{state-value function}, $\statevalue: \states \times \outerset^\states \times \innerset^\states \to \R$, and the \mydef{action-value function}, $\actionvalue: \states \times \outerset \times \innerset \times \outerset^\states \times \innerset^\states \to \R$, respectively, are defined as: \\
{\small\begin{align}
% $
    \statevalue(\state; \policy[\outer], \policy[\inner] ) &= \mathop{\E^{\policy[\outer], \policy[\inner]}}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty 
    % (1-\discount)
    \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid
    % \outerrv[\iter] = \policy[\outer]( \staterv[\iter]), \innerrv[\iter]  = \policy[\inner](\staterv[\iter]),
    \staterv[0] = \state \right] \\ %\label{eq:state_value}
% $
% \end{align}
% \begin{align}\label{eq:state_value}
% \end{align}
% and,
% \sadie{For the part under $\E$, should that be $\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])$?}
% \sadie{Do you think we can adopt the notation  $\E^{\policy[]}$ in the note to indicate the expected value given we act according to $\policy[]$. For example, $\statevalue(\state; \policy[\outer], \policy[\inner] ) = \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter])} ^{\policy[\outer]\policy[\inner]}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \staterv[0] = \state \right]$? Will this make the notations more concise?}
% \begin{align}\label{eq:action_value}
% \begin{align}
% \tiny
% $$
    \actionvalue(\state, \outer, \inner; \policy[\outer], \policy[\inner]) &= \mathop{\E^{\policy[\outer], \policy[\inner]}}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty 
    % (1-\discount)
    \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid
    % \outerrv[\iter] =  \policy[\outer]( \staterv[\iter]),  \innerrv[\iter] = \policy[\inner](\staterv[\iter]),
    \staterv[0] = \state, \outerrv[0] = \outer, \innerrv[0] = \inner \right] 
    % \label{eq:action_value} 
    %\enspace .
\end{align}}
% $$.
% \deni{Fix the $(1-\discount)$, I do not think the factors are propagating though algo or proofs correctly}

Again, to simplify notation, we write expectations conditional on $\outerrv[\iter] = \policy[\outer]( \staterv[\iter])$ and $\innerrv[\iter] = \policy[\inner](\staterv[\iter])$ as $\E^{\policy[\outer], \policy[\inner]}$, and denote the state- and action-value functions by $\statevalue[][{\policy[\outer]}][{ \policy[\inner]}](\state)$, and $\actionvalue[][{\policy[\outer]}][{ \policy[\inner]}](\state, \outer, \inner)$, respectively.
Additionally, we let $\statevalfuncs  = [-\nicefrac{\rewardbound}{1- \discount}, \nicefrac{\rewardbound}{1- \discount}]^{\states}$ be the space of all state-value functions of the form $\statevalue: \states \to [-\nicefrac{\rewardbound}{1- \discount}, \nicefrac{\rewardbound}{1- \discount}]$, and we let $\actionvalfuncs = [-\nicefrac{\rewardbound}{1- \discount}, \nicefrac{\rewardbound}{1- \discount}]^{\states \times \outerset \times \innerset}$ be the space of all action-value functions of the form $\actionvalue: \states \times \outerset \times \innerset \to [-\nicefrac{\rewardbound}{1- \discount}, \nicefrac{\rewardbound}{1- \discount}]$.
Note that by \Cref{assum:main} the range of the state- and action-value functions is $[-\nicefrac{\rewardbound}{1- \discount}, \nicefrac{\rewardbound}{1- \discount}]$.
The cumulative payoff function of the game $\cumul: \outerset^\states \times \innerset^\states \to \R$ is the total expected loss (resp.\ gain) of the outer (resp.\ inner) player, given by $\cumul (\policy[\outer], \policy[\inner]) = \mathop{\E}_{\state \sim \initstates (\state)} \left[ \statevalue[][{\policy[\outer]}][{\policy[\inner]}] (\state) \right]$.
    % \\
    % &=\mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \state[\iter], \outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] = \policy[\outer]( \staterv[\iter]), \innerrv[\iter] = \policy[\inner](\staterv[\iter]) \right]\\

% \begin{definition}[Stacklberg Equilibrium]
The canonical solution concept for stochastic Stackelberg games is the \mydef{Stackelberg equilibrium (SE)}.
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is said to be a Stackelberg equilibrium (SE) of a zero-sum stochastic Stackelberg game $\initgame$ iff \\
%\begin{align}
    $$\max_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right) \leq \cumul \left( \policy[\outer]^*, \policy[\inner]^* \right)  \leq \min_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer], \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer], \policy[\inner] \right) \enspace .$$
%    \enspace .
%\end{align}
% \end{definition}
Note the strength of this definition, as it requires the constraints $\constr(\state, \policy[\outer], \policy[\inner]) \geq \zeros$ to be satisfied at all states $\state \in \states$, not only states which are reached with strictly positive probability.
A SE is guaranteed to exist in zero-sum stochastic Stackelberg games, under \Cref{assum:main}, as a corollary of \citeauthor{goktas2021minmax}'s \cite{goktas2021minmax} Proposition B.2.; however, this existence result is non-constructive.%
\footnote{We note SE should technically be defined in terms of non-stationary policies; however, as we will show, stationary policies suffice, since SE exist in stationary policies.}

In this paper, we study a Markov perfect refinement of SE, which we call \mydef{recursive Stackelberg equilibrium} (\recSE{}).

\begin{definition}[Recursive Stackelberg Equilibrium (\recSE{})]\label{lemma:stackelberg_action_value}
Given $\initgame$, a policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a \mydef{recursive Stackelberg equilibrium} (\recSE{}) iff, for all $\state \in \states$, it holds that:
{\small
$$
 \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner) \leq 
\actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \policy[\outer]^*(\outer), \policy[\inner]^*(\inner))
\leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner).
$$
}
\end{definition}

Equivalently, a policy profile $(\policy[\outer]^*, \policy[\inner]^*)$ is a \recSE{} if $(\policy[\outer]^*(\state), \policy[\inner]^*(\state))$ is a SE with value $\statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)$ at each state $\state \in \states$:
i.e., $\statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) = \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)$, for all %states 
$\state \in \states$.
% In other words, a feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a Stackelberg equilibrium if $\policy[\outer]^* \in \argmin_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states : \constrs(\policy[\outer], \policy[\inner]) \geq 0}  \cumul \left( \policy[\outer], \policy[\inner] \right)$ and $\policy[\inner]^* \in \argmax_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer]^*, \policy[\inner]) \geq 0}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right)$.
% \sadie{Should this be $\policy[\outer]^*\in \argmin \max$ and $\policy[\inner]^* \in \argmax$? And why we use $g$ instead of $G$ here?}

% \begin{remark}
% This is a strong definition of a \recSE, since we require the constraints $\constr(\state, \policy[\outer], \policy[\inner]) \geq \zeros$ to be satisfied at all states $\state \in \states$, not only states which are reached with strictly positive probability. 
% % Technically, at a Stackelberg equilibrium it would be enough for the constraints to be satisfied only for states which have a strictly positive probability of being reached by the policy profile. 
% % However, since the game is Markovian, i.e., the transition probabilities and reward function only depend on the current state and action, the actions outputted for states reached by the Stackelberg equilibrium policies with a strictly positive probability are the same under both definitions.
% % \amy{writing unclear to me}\deni{Fixed!}
% \end{remark}
% \amy{why not write u as the expected value of v, where s is drawn from $\mu^{(0)}$?}
% \begin{definition}
% A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a \recSE of a stochastic min-max Stackelberg game iff 
% \begin{align}
%     \max_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right) \leq \cumul \left( \policy[\outer]^*, \policy[\inner]^* \right)  \leq \min_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer], \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer], \policy[\inner] \right) 
%     \enspace .
% \end{align}
% \end{definition}
%
% In other words, a feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a recursive Stackelberg equilibrium if  $\policy[\outer]^* \in \argmin_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \innerset^\states : \constrs(\policy[\outer], \policy[\inner]) \geq 0}  \cumul \left( \policy[\outer], \policy[\inner] \right)$ and $\policy[\inner]^* \in \argmax_{\policy[\inner] \in \innerset^\states : \constrs( \policy[\outer]^*, \policy[\inner]) \geq 0}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right)$.
% \sadie{Should this be $\policy[\outer]^*\in \argmin \max$ and $\policy[\inner]^* \in \argmax$? And why we use $g$ instead of $G$ here?}
% \begin{remark}
% We note that this is a stronger definition of a \recSE than is required since we require the constraints $\constr(\state, \policy[\outer], \policy[\inner]) \geq \zeros$ to be satisfied for all states $\state \in \states$. Technically, at a \recSE it would be enough for the constraints to be satisfied only for states which have a strictly positive probability of being reached by the policy profile. 
% % However, since the game is Markovian, i.e., the transition probabilities and reward function only depend on the current state and action, the actions outputted for states reached by the Stackelberg equilibrium policies with a strictly positive probability are the same under both definitions.
% \end{remark}

\paragraph{Mathematical Preliminaries}
%
A probability measure $q_1 \in \simplex(\states)$ \mydef{convex stochastically dominates (CSD)} $q_2 \in \simplex(\states)$ if $\int_\states \statevalue(s) q_1(s) ds \geq \int_\states \statevalue(s) q_2(s) ds$ for all continuous, bounded, and convex functions $\statevalue$ on $S$.
A transition function $\trans$ is termed \mydef{CSD convex} in $\outer$ if, for all $\lambda \in (0,1)$, $\inner \in \innerset$ and any $(\state^\prime, \outer^\prime), (\state^\dagger, \outer^\dagger) \in \states \times \outerset$, with $(\state, \outer) = \lambda (\state^\prime, \outer^\prime) + (1-\lambda) (\state^\dagger, \outer^\dagger)$, it holds that $\lambda \trans(\cdot \mid \state^\prime, \outer^\prime, \inner) + (1-\lambda) \trans(\cdot \mid \state^\dagger, \outer^\dagger, \inner)$ CSD $\trans(\cdot \mid \state, \outer, \inner)$.
A transition function $\trans$ is termed \mydef{CSD concave} in $\inner$ if, for all $\lambda \in (0,1)$ and any $(\state^\prime, \inner^\prime), (\state^\dagger, \inner^\dagger) \in  \states \times \outerset \times \innerset$, with $(\state, \inner) = \lambda (\state^\prime,  \inner^\prime) + (1-\lambda) (\state^\dagger, \inner^\dagger)$, it holds that $\trans(\cdot \mid \state, \outer, \inner)$ CSD $\lambda \trans(\cdot \mid \state^\prime, \outer, \inner^\prime) + (1-\lambda) \trans(\cdot \mid \state^\dagger, \outer, \inner^\dagger)$.
A mapping $L : \calA \to \calB$ is said to be a \mydef{contraction mapping} (resp.{} \mydef{non-expansion}) w.r.t.\ norm $\left\| \cdot \right\|$ iff for all $\x, \y \in \calA$, and for $k \in [0,1)$ (resp.{} $k = 1$) such that $\left\| L(\x) - L(\y) \right\| \leq k \left\| \x - \y \right\|$.
The \mydef{min-max operator} $\min_{\outer \in \outerset} \max_{\inner \in \innerset}: \R^{\outerset \times \innerset} \to \R$ w.r.t. to sets $\outerset, \innerset$ takes as input a function $\obj: \outerset \times \innerset \to \R$ and outputs $\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner)$.
The \mydef{generalized min-max operator} $\min_{\outer \in \outerset} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros}: \R^{\outerset \times \innerset} \to \R$ w.r.t. to sets $\outerset, \innerset$ and the function $\constr: \outerset \times \innerset \to \R$ takes as input a function $\obj: \outerset \times \innerset \to \R$ and outputs $\min_{\outer \in \outerset} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$.


==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/properties.tex <==
\section{Properties of Recursive Stackelberg equilibrium}
\label{sec:properties}

% \begin{proposition}
% Suppose that $(\policy[\outer]^*, \policy[\inner]^*)$ is a Stackelberg equilibrium, with associated action value function $\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$. Then, the greedy policy $\left({\policy[\outer]}^{\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]}, {\policy[\inner]}^{\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]} \right)$ with respect to $\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$ is also a Stackelberg equilibrium.
% \end{proposition}
% \begin{proof}
% Suppose that the greedy policy  $\left({\policy[\outer]}^{\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]}, {\policy[\inner]}^{\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]} \right)$ with respect to $\actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$ is not a Stackelberg equilibrium. 
% \end{proof}

% \section{Properties of Stackelberg Equilibrium}
% \sdeni{
% We first state a \sdeni{necessary}{sufficient} condition that the state-value function induced by a policy profile needs to satisfy in order for that policy profile to be a \recSE. It is not directly clear if there exists a policy for any zero-sum stochastic Stackelberg game which satisfies this \sdeni{necessary}{sufficient} condition since there is no way to guarantee that such an inequality will hold at all states.\footnote{All omitted results and proofs can be found in the appendix.}
% }{}
% \begin{restatable}{lemma}{lemmastackelbergactionvalue}
% % \label{lemma:stackelberg_action_value}
% \sdeni{Consider a zero-sum stochastic Stackelberg game $\initgame$.
% A policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a \recSE{} if, for all $\state \in \states$, we have that:
% %
% %\begin{align}
%     $\max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner) \leq 
%     \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \policy[\outer]^*(\outer), \policy[\inner]^*(\inner))
%     \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)$.
% %\enspace .
% %\end{align}
% Equivalently, a policy profile $(\policy[\outer]^*, \policy[\inner]^*)$ is a \recSE{} if for all $\state \in \states$, $(\policy[\outer]^*(\state), \policy[\inner]^*(\state))$ is a Stackelberg equilibrium with value $\statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)$:
% %\deni{Either add definition of Stackelberg equilibrium or cite paper}\amy{i think the ``i.e.'' i added is enough}:
% i.e., $\statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) = \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)$ at each $\state \in  \states$.}{}
% \end{restatable}

% \sadie{for the constraint, should we do $\constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros$ and $\constr(\state, \outer, \inner) \geq \zeros?$}\deni{Fixed, does it look good now?}\sadie{It looks good to me!}

In this section, we show that a \recSE{} exists in all zero-sum stochastic Stackelberg games.%
\footnote{All omitted results and proofs can be found in the appendix.}
To do so, we first associate an operator $\bellopt: \statevalfuncs \to \statevalfuncs$ with any zero-sum stochastic Stackelberg game $\initgame$, the fixed points of which we show satisfy \Cref{lemma:stackelberg_action_value}, and hence are necessary and sufficient to
characterize \deni{Is necessary and sufficient redundant here? I don't feel it is?}\amy{i do think it is redundant. i think that is exactly what characterization means. but i am also fine with saying this twice}
the value function associated with a \recSE{} of $\initgame$.
We then show that this operator is a contraction mapping, thereby establishing the existence of such a fixed point.
Together these results generalize \citeauthor{shapley1953stochastic}'s theorem on the existence of Markov perfect Nash equilibria in zero-sum stochastic games \cite{shapley1953stochastic}.
%, i.e., zero-sum stochastic Stackelberg games in which $\constrs(\policy[\outer], \policy[\inner]) \geq \zeros$, for all $(\policy[\outer], \policy[\inner]) \in \outerset^\states \times \innerset^\states$.

Given a zero-sum stochastic Stackelberg game $\initgame$, define $\bellopt: \statevalfuncs \to \statevalfuncs$ as the operator $\left(\bellopt \statevalue[] \right) (\state) = \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner)\geq \zeros} \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right]$. 
We call the set of $\numstates$ equations $\left(\bellopt \statevalue[] \right) (\state) =  \statevalue[](\state)$ with $\statevalue[]$ unknown the \mydef{Bellman equations} for $\initgame$.
The next theorem shows that these Bellman equations
% \samy{are necessary and sufficient to}{}\amy{i think this is what characterize means!}\deni{Conditions can characterize something (sufficiency) or something satisfies, i.e., characterizes, certain mathematical conditions. I think it is better precise but up to you.}
characterize the state-value function associated with a \recSE.
Consequently, the solution to a zero-sum stochastic Stackelberg game can be described by its Bellman equations.

%uniqueness
 
%We first show that the fixed points of $\bellopt$ correspond to the $\recSE$ of the associated game.

\begin{restatable}{theorem}{thmfpbelloptisstackelberg}
\label{thm:fp_bellopt_is_stackelberg}
Given $\initgame$, the policy profile $(\policy[\outer]^*, \policy[\inner]^*)$ is a \recSE{} iff it induces a value function which is a fixed point of $\bellopt$: i.e., $(\policy[\outer]^*, \policy[\inner]^*)$ is a \recSE{} iff, for all $\state \in \states,$ $\left(\bellopt \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}] \right) (\state) = \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}](\state)$.
\end{restatable}
The following technical lemma is crucial to proving that $\bellopt$ is a contraction mapping.
It tells us that the generalized min-max operator is non-expansive; in other words, the generalized min-max operator is 1-Lipschitz w.r.t.\ the sup-norm.

\begin{restatable}{lemma}{lemmaminmaxlipschitz}
\label{lemma:minmax_lipschitz}
Suppose that $f, h: \outerset \times \innerset \to \R$, $\constr: \outerset \times \innerset \to \R^\numconstrs$ are continuous functions, and $\outerset, \innerset$ are compact sets.
Then
%\begin{align}
$\left| \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} f(\outer, \inner) - \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} h(\outer, \inner) \right|$ \\
$\leq \max_{(\outer, \inner) \in \outerset \times \innerset } \left| f(\outer, \inner) -  h(\outer, \inner) \right|$.
%\enspace .
%\end{align}
\end{restatable}

%With the above lemma in hand, we can now prove that $\bellopt$ is a contraction mapping.

\begin{restatable}{theorem}{thmcontractionmapping}\label{thm:contraction_mapping}
Consider the operator $\bellopt$ associated with a zero-sum stochastic Stackelberg game $\initgame$. Under \Cref{assum:main}, $\bellopt$ is a contraction mapping w.r.t.\ to the sup norm $\left\| . \right\|_{\infty}$ with 
%contraction
constant $\gamma$.
\end{restatable}

\begin{proof}
%[Proof of \Cref{thm:contraction_mapping}]
We will show that $\bellopt$ is a contraction mapping.
The result then follows by Banach's fixed point theorem \cite{banach1922operations}.
Let $\statevalue[], {\statevalue[]}^\prime \in \statevalfuncs$ be any two state value functions, and let $\actionvalue, {\actionvalue}^\prime \in \actionvalfuncs$ be the associated action-value functions, respectively.
Then, it holds that
\begin{align}
    &\left\| \bellopt \statevalue[] - \bellopt {\statevalue[]}^\prime \right\|_{\infty} \nonumber \\
    &= \max_{\state \in \states} \left|\min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq  \zeros} \actionvalue(\state, \outer, \inner) - \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq  \zeros} {\actionvalue}^{\prime}(\state, \outer, \inner) \right| \nonumber \\
    &\leq \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \left| \actionvalue(\state, \outer, \inner) - {\actionvalue}^{\prime}(\state, \outer, \inner) \right| \label{eq:dist_min_maxes} \\
    &= \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \left|\mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right] - \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount {\statevalue[]}^\prime(\staterv^\prime)  \right] \right| \nonumber \\
    %&\leq \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \left|\mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[\discount \statevalue[](\staterv^\prime)  - \discount {\statevalue[]}^\prime(\staterv^\prime)  \right] \right| \\
    &=\discount \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \left|\mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \statevalue[](\staterv^\prime)  -  {\statevalue[]}^\prime(\staterv^\prime)  \right] \right| \nonumber \\
    &\leq\discount \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \max_{\state^\prime \in \states} \left| \statevalue[](\state^\prime)  -  {\statevalue[]}^\prime(\state^\prime) \right| \label{eq:exp_less_than_max} \\
    &= \discount \max_{\state \in \states} \max_{(\outer, \inner) \in \outerset \times \innerset} \left| \statevalue[](\state)  -  {\statevalue[]}^\prime(\state) \right| \nonumber \\
    &= \discount \left\|\statevalue[] - {\statevalue[]}^\prime \right\|_\infty \enspace , \nonumber
\end{align}

\noindent
where \Cref{eq:dist_min_maxes} follows by \Cref{lemma:minmax_lipschitz} and \Cref{eq:exp_less_than_max} follows from the fact that the expectation of a random variable is less than or equal to its maximum value.
\end{proof}

Given an initial state-value function $\statevalue[0] \in \statevalfuncs$, we define the \mydef{value iteration} process  as $\statevalue[\iter+1] = \bellopt \statevalue[\iter]$, for all $\iter \in \N_+$ (\Cref{alg:value_iter}).
One way to interpret $\statevalue[\iter]$ is as the function that returns the value $\statevalue[\iter](\state)$ of each state $\state \in \states$ in the $\iter$-stage zero-sum stochastic Stackelberg game starting at the last stage $\iter$ and proceeding backwards to stage $0$, with terminal payoffs given by $\statevalue[0]$.
The following theorem, which is a consequence of Theorems~\ref{thm:fp_bellopt_is_stackelberg} and~\ref{thm:contraction_mapping}, and the Banach fixed point theorem \cite{banach1922operations}, not only proves the existence of a \recSE{}, but further provides us with a means of computing a \recSE{} via value iteration. 

\begin{restatable}{theorem}{thmexistencestackelberg}
\label{thm:existence_stackelberg}
Consider a zero-sum stochastic Stackelberg game $\initgame$.
Under \Cref{assum:main}, $\initgame$ has
% \samy{at least one \recSE{} $(\policy[\outer]^*, \policy[\inner]^*)$ with unique\amy{what does unique mean here?}\deni{For all equilibria, the payoffs that the players get are the same.}}{
a unique
value function $\statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$ associated with all \recSE{} $(\policy[\outer]^*, \policy[\inner]^*)$,
which can be computed by iteratively applying $\bellopt$ to
any initial state-value function $\statevalue[0] \in \statevalfuncs$: i.e., $\lim_{\iter \to \infty} \statevalue[\iter] = \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$.
\end{restatable}

\begin{remark}
Unlike Shapley's existence theorem for recursive Nash equilibria in zero-sum stochastic games, \Cref{thm:existence_stackelberg} does not require the payoff function to be convex-concave.
The only conditions needed are continuity of the payoffs and constraints, and bounded payoffs.
This makes the \recSE{} a potentially useful solution concept, even for non-convex-non-concave stochastic games. 
\end{remark}

%\sdeni{Note that the proof of \Cref{thm:existence_stackelberg} shows that there exists a policy profile which satisfies the conditions of \Cref{lemma:stackelberg_action_value}.}{}

Since a \recSE{} is guaranteed to exist, and is by definition independent of the initial state distribution, we can infer that the \recSE{} of any zero-sum stochastic Stackelberg game $\initgame = (\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ is independent of the initial state distribution $\initstates$.
%As a result, for all $\initstates, {\initstates}^\prime \in [0,1]^\states$, we have that the \recSE{} of $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ and $(\states, \outerset, \innerset, {\initstates}^\prime, \reward, \constr, \trans, \discount)$ are the same. 
Hence,
% obtain the following corollary of the above theorem, and  
in the remainder of the paper, we denote zero-sum stochastic Stackelberg games by $\game \doteq (\states, \outerset, \innerset, \reward, \constr, \trans, \discount)$. 

\if 0
\sdeni{It seems that a stronger equilibrium concept for zero-sum stochastic Stackelberg games would be one that requires the strategy profile be a \recSE{} of each subgame,
%of the zero-sum stochastic Stackelberg game,
aptly called \mydef{subgame perfect Stackelberg equilibrium}.
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a subgame perfect Stackelberg equilibrium of a zero-sum stochastic Stackelberg game $\game$ if, for all $\state \in \states, \iter \in \N, \statedist[\iter+1](\state) = \sum_{\state^\prime \in \states} \trans(\state \mid \state^\prime, \policy[\outer]^*(\state^\prime), \policy[\inner]^*(\state^\prime)) \statedist[\iter ](\state^\prime)$, $(\policy[\outer]^*, \policy[\inner]^*)$ is a \recSE{} of $(\states, \outerset, \innerset, \statedist[\iter], \reward, \constr, \trans, \discount)$.
By definition, the set of subgame perfect Stackelberg equilibria of a zero-sum stochastic Stackelberg game is a subset of the set of \recSE{} of the game.
Since the set of \recSE{} is independent of the initial state distribution $\initstates$, the reverse inclusion also holds.
We thus have the following corollary:
}{}
\begin{corollary}
\sdeni{The set of \recSE{} and subgame perfect Stackelberg equilibria coincide in zero-sum stochastic Stackelberg games.}{}
\end{corollary}
\fi

\Cref{thm:existence_stackelberg} tells us that value iteration %\samy{}{(\Cref{alg:value_iter})}
converges to the value function associated with a \recSE.
Additionally, under \Cref{assum:main}, \recSE{} is computable in (weakly) polynomial time.%
\footnote{This convergence is only weakly polynomial time, because the computation of the generalized min-max operator applied to an arbitrary continuous function is an NP-hard problem; it is at least as hard as non-convex optimization.
If, however, we restrict attention to convex-concave stochastic Stackelberg games, then Stackelberg equilibria are computable in polynomial time.}

\begin{restatable}[Convergence of Value Iteration]{theorem}{thmvalueiter}\label{thm:value_iter}
% Denote $\policy[\outer]^{(k)}=\policy[\outer]^{\actionvalue[k]}$, $\policy[\inner]^{(k)}=\policy[\inner]^{\actionvalue[k]}$ be greedy policies with respect to $\actionvalue[k]$. 
% Then, let $\statevalue[k]=\statevalue[][{\policy[\outer]^{(k)}}][{\policy[\inner]^{(k)}}]$. Let $\epsilon>0$. 
Suppose value iteration is run on input $\game$.
Let $(\policy[\outer]^*, \policy[\inner]^*)$ be \recSE{} of $\game$ with value function $\statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$.
Under \Cref{assum:main}, if we initialize $\statevalue[0] (\state) = 0$, for all $\state \in \states$, then for $k \geq \frac{1}{1 - \discount}  \log \frac{ \rewardbound}{\epsilon(1 - \discount)}$, it holds that
% \begin{align*}
    $\statevalue[k](\state)  - \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}](\state) \leq \epsilon$. 
    % \deni{Define $\statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}]$}\amy{done, if that's what you meant?}
% \end{align*}
\end{restatable}


% The subdifferential Benveniste-Scheinkman theorem (\Cref{thm:subdiff_bellman}) can be used to derive an instance of  \citeauthor{goktas2021minmax}'s \cite{goktas2021minmax} nested gradient descent ascent algorithm to compute the generalized min-max operator at each iteration \Cref{alg:value_iter}, i.e., line \ref{algeq:value_iter}.   

% This means that in order to take a gradient descent step for the outer player using the subdifferential given in \Cref{thm:subdiff_bellman}, one has to first run value iteration for the inner player, fixing a strategy of the outer player.


% \begin{algorithm}[H]
% \caption{Value Iteration with Max-oracle}
% \label{alg:value_iter}
% \begin{algorithmic}[1]
% \State Initialize $\statevalue[0]$ arbitrarily, e.g. $\statevalue[0]=0$
% \For{$\iter = 0, \hdots, \numiters$}
%     \For{$\state \in \states$}
%         \For{$\outeriter = 0, \hdots, \outeriters$}
%             \State $\outer[\outeriter+1] = \project[\outerset]\left[ \outer[\outeriter+1] - \learnrate[\outer] \left( \grad[\outer] \lang[\state, {\policy[\outer]^*(\state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) \right)\right]$
%             \State $\displaystyle
%             \statevalue[\iter+1] (\state) = \min_{\outer \in \outerset} 
%             \max_{\inner \in \innerset: \constr(\state, \outer, \inner) \geq \zeros} \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[\iter](\staterv^\prime)  \right]$ \label{algeq:value_iter}
%         \EndFor
%     \EndFor
% \EndFor
% \State \Return $\statevalue[{\numiters}]$ 
% \end{algorithmic}
% \end{algorithm}




==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/related.tex <==
\paragraph{Related Work}

Algorithms for min-max optimization problems (i.e., zero-sum games) with independent strategy sets have been extensively studied 
\cite{tseng1995variational, nesterov2006variational, gidel2020variational, mokhtari2020convergence, ibrahim2019lower, zhang2020lower, lin2020near, alkousa2020accelerated, juditsky2011first, hamedani2018primal, zhao2019optimal, thekumparampil2019efficient, ouyang2018lower, nemirovski2004prox, nesterov2007dual, tseng2008accelerated, sanjabi2018stoch, nouiehed2019solving, lu2019block, jin2020local, ostrovskii2020efficient, lin2020gradient, zhao2020primal, rafique2019nonconvex} (for a summary see, Section G \cite{goktas2021minmax}).
\citeauthor{goktas2021minmax} studied min-max games with dependent strategy sets, proposing polynomial-time nested gradient descent ascent (GDA) \cite{goktas2021minmax} and simultaneous GDA algorithms for such problems \cite{goktas2021robustminmax}.
%\cite{goktas2021minmax} studied zero-sum games with dependent strategy sets, proposing a polynomial-time nested gradient descent ascent (GDA) algorithm for such problems.
%Their work was followed by \cite{goktas2021minmaxgdaamas}, who introduced a polynomial-time simultaneous GDA algorithm.

The computation of Stackelberg equilibrium in two-player stochastic Stackelberg games has been studied in several interesting settings, in which the leader moves before the follower, but without the leader's actions impacting the followers' choice sets.
% \amy{i assume none of these settings consider dependent strategy sets?}\deni{correct, great point, thank you!}
\citeauthor{bensoussan2015maximum} \cite{bensoussan2015maximum} study continuous-time general-sum stochastic Stackelberg games with continuous action spaces, and prove existence of a solution in this setting.
%, but their model, unlike ours, does not account for dependence in the players' strategy sets.
\citeauthor{vorobeychik2012computing} \cite{vorobeychik2012computing} consider a general-sum
%discounted
stochastic Stackelberg game with finite state-action spaces and an infinite horizon.
These authors show that stationary SE policies do not exist in this very general setting, but nonetheless identify a subclass of games, namely team (or potential) Stackelberg games for which stationary Stackelberg equilibrium policies do exist.
% Our paper answer a question asked by \citeauthor{vorobeychik2012computing} \cite{vorobeychik2012computing} \amy{i'm not sure. was it an important question? if so, say what it is. if not, leave this remark out.} and identifies a novel class of stochastic Stackelberg games, namely zero-sum, for which, to our knowledge, we provide the first polynomial-time computation guarantees.
\citeauthor{vu2022stackelberg} \cite{vu2022stackelberg} study the empirical convergence of policy gradient methods in the same setting as \citeauthor{vorobeychik2012computing} \cite{vorobeychik2012computing}, while \citeauthor{ramponi2022learning} \cite{ramponi2022learning} study non-stationary equilibria in this same setting, assuming a finite horizon.
\citeauthor{chang2015leader} \cite{chang2015leader} and \citeauthor{sengupta2020multi} \cite{sengupta2020multi} consider a partially observable version of \citeauthor{vorobeychik2012computing}'s  \cite{vorobeychik2012computing} model, and provide methods to compute Stackelberg equilibria in their setting.

%We note that our setting is more general due to 1) the dependency in the strategy sets of the players at each state, and 2) the possibility to consider continuous action space, hence the above results do not apply to our setting.

Some recent research concerns one leader-many followers Stackelberg games.
\citeauthor{vasal2020stochastic} \cite{vasal2020stochastic} studies a discrete-time, finite horizon one leader-many follower stochastic Stackelberg game
%with independent strategy sets
with discrete action and state spaces, and provides algorithms to solve such games.
\citeauthor{demiguel2009stochastic} \cite{demiguel2009stochastic} consider a stochastic Stackelberg game-like market model with $n$ leaders and $m$ followers; they prove the existence of a SE in their model, and provide (without theoretical guarantees) algorithms that converge to such an equilibrium in experiments.
%, their model does not account for dependencies in the strategy sets of the players.  
Dynamic Stackelberg games \cite{li2017review} have been applied to a wide range of problems, including security \cite{vasal2020stochastic, vorobeychik2012computing}, insurance provision \cite{chen2018new, yuan2021robust}, advertising \cite{he2008cooperative}, robust agent design \cite{rismiller2020stochastic}, allocating goods across time intertemporal pricing \cite{oksendal2013stochastic}. 

The study of algorithms that compute competitive equilibria in Fisher markets was initiated by \citeauthor{devanur2002market}, who provided a polynomial-time method for solving these markets assuming linear utilities.
More recently, there have been efforts to study markets in dynamic settings \cite{cheung2019tracing, gao2021online, goktas2021minmax}, in which the goal is to either track the changing equilibrium of a changing market, or minimize some regret-like quantity for the market.
The models considered in these earlier works differ from ours as they do not have stochastic structure and do not invoke a dynamic solution concept. \deni{Add the work of Michael Jordan's group on stochastic EE.}


==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/subdifferential.tex <==
\section{Subdifferential Envelope Theorems and Optimality Conditions for Recursive Stackelberg Equilibrium}\label{sec:benveniste}
% Benveniste-Scheinkman Theorem and Optimality Conditions for Stackelberg Equilibrium

%In order to build theoretical applications of zero-sum stochastic Stackelberg games, one has to
In this section, we derive optimality conditions for recursive Stackelberg equilibria. 
In particular, we provide necessary conditions for a policy profile to be a \recSE{} of any zero-sum stochastic Stackelberg game, and show that under additional convexity assumptions, these conditions are also sufficient. 
\if 0
Using these results, we prove in the next section that recursive market equilibrium \cite{mehra1977recursive}
%an important solution concept in economics
is an instance of \recSE{} in a large class of stochastic markets. 
\fi

The Benveniste-Scheinkman theorem characterizes the derivative of the optimal value function associated with a recursive optimization problem
%, i.e., the Bellman equation, 
w.r.t.\ its parameters, when it is differentiable \cite{Benveniste1979value}.
Our proofs of the necessary and sufficient optimality conditions rely on a novel subdifferential generalization (\Cref{thm:subdiff_bellman}, \Cref{sec_app:benveniste}) of this theorem, which applies even when the optimal value function is not differentiable.
%
%Although in their seminal work \cite{Benveniste1979value} provide conditions under which the Bellman equation is differentiable w.r.t. its parameters, such conditions are too strict and do not allow us to derive useful optimality conditions for stochastic Stackelberg games. \deni{Need to re-read this sentence and maybe rephrase.}
%
% \amy{delete this paragraph? doesn't seem essential.}
% \Cref{thm:existence_stackelberg} tells us that value iteration converges (\Cref{alg:value_iter}) to the optimal value function associated with a recursive Stackelberg equilibrium of a Stackelberg game. Although \citeauthor{goktas2021minmax} \cite{goktas2021minmax} and \citeauthor{goktas2021robustminmax} \cite{goktas2021robustminmax} provide us with algorithms to compute the generalized min-max operator, the recursive nature of the generalized min-max problem in line \ref{algeq:value_iter} of \Cref{alg:value_iter}, makes it impossible to directly apply such algorithms and requires additional machinery. In particular, the algorithms proposed by \citeauthor{goktas2021minmax} \cite{goktas2021minmax} and \citeauthor{goktas2021robustminmax} \cite{goktas2021robustminmax} require knowledge of a subgradient of $\mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right]$. Although, \citeauthor{goktas2021minmax} \cite{goktas2021minmax} provides a subdifferential envelope theorem to compute such a subgradient, their result does not directly apply to recursive objective functions such as the one in line \ref{algeq:value_iter} of \Cref{alg:value_iter}. Although in their seminal work \citeauthor{Benveniste1979value} \cite{Benveniste1979value} provide conditions under which a recursive optimization problem is differentiable w.r.t. its parameters, such conditions are too strict and to the best of our knowledge there exists no results in the optimization literature that provides us with the subdifferential of $\mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right]$ under looser assumptions. To this end, in this section, we will provide a subdifferential generalization of the well-known \citeauthor{Benveniste1979value} \cite{Benveniste1979value} theorem. 
% An additional benefit of our result will also be a simple and direct derivation of the necessary and sufficient optimality conditions for a policy profile to be a Stackelberg equilibrium of a zero-sum convex-concave Stackelberg game, and necessary optimality conditions for a policy profile to be a Stackelberg equilibrium of a zero-sum Stackelberg game.
%
% % as we will show, in order to solve the min-max problem in line \ref{algeq:value_iter} of \Cref{alg:value_iter} one has to run a nested value iteration algorithm. 
%
% % We now move on to derive the first order necessary conditions for a policy profile $(\policy[\outer], \policy[\inner])$ to be a Stackelberg equilibrium of a zero-sum stochastic Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$.
% %
% %
% % To derive these condition we first provide a generalization of the Benveniste-Scheinkman theorem \cite{Benveniste1979value}. The Benveniste-Scheinkman theorem provides condition under which the Bellman equation associated with the optimization of a function defined recursively is differentiable. We generalize this theorem, by providing conditions under which the Bellman equation is associated with a recursive optimization problem is \emph{subdifferentiable}.
%
% Our result relies on a slightly generalized version of the subdifferential envelope theorem of \citeauthor{goktas2021minmax} \cite{goktas2021minmax}, which we state below. The conclusion of the following theorem is the same as that proven by \citeauthor{goktas2021minmax} \cite{goktas2021minmax} but we notice that their proof goes through with the following weaker conditions:
%
\if 0
\begin{proof}

As $\constr[1], \hdots, \constr[\numconstrs]$ are continuous, and Slater's condition holds,  the constraint correspondence associated with the problem is continuous, non-empty-, and compact-valued. Hence, by \citeauthor{berge1997topological}'s maximum theorem \cite{berge1997topological}, $\marginal(\state, \outer)$ is continuous in $\outer$.
\if 0
    First note that we can re-express the marginal function $\marginal(\state, \outer)$ as follows:
    \begin{align}
        \marginal(\state, \outer) = \max_{\substack{\left\{ \inner[\iter] \in  \innerset: \constr(\state, \outer, \inner[\iter]) \geq \zeros  \right\}_{\iter = 1}^\infty}} \sum_{\iter=0}^\infty \discount^\iter \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \inner[\iter-1])} \left[\reward(\state^\prime, \outer, \inner[\iter]) \right]
    \end{align}
    Since for all $\numiters \in \N_+$, we have that $\sum_{\iter=0}^\numiters \discount^\iter \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer, \inner[\iter-1])} \left[\reward(\state^\prime, \inner[\iter]) \right] \leq \frac{\rewardbound}{1-\discount}$, and the Bellman operator is a contraction mapping, $\left\{\sum_{\iter=0}^\numiters \discount^\iter \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer, \inner[\iter-1])} \left[\reward(\state^\prime, \inner[\iter]) \right]\right\}_\numiters$ passes the Weierstrass M-test \cite{rudin1991functional} which means that $\left\{\sum_{\iter=0}^\numiters \discount^\iter \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer, \inner[\iter-1])} \left[\reward(\state^\prime, \inner[\iter]) \right]\right\}_\numiters$ is a uniformly converging sequence. Since $\reward$ is bounded and continuous, by the Lebesgue dominated convergence theorem \cite{rudin1991functional}, $\left\{ \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer, \inner[\iter-1])} \left[\reward(\state^\prime, \outer, \inner[\iter]) \right]\right\}_\iter$ is a sequence of continuous functions, hence by the uniform limit theorem \cite{munkres2000topology} $\sum_{\iter=0}^\infty \discount^\iter \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer, \inner[\iter-1])} \left[\reward(\state^\prime, \inner[\iter]) \right]$ is continuous in $\outer$. 
    Additionally, 
    
    
   
    Since $\reward(\outer, \inner)$ is concave, and integration preserves concavity (\cite{boyd2004convex}, section 3.2.1), $ \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \inner[\iter-1])} \left[\reward(\state^\prime, \outer, \inner[\iter]) \right]$ is concave in $\outer$.
    \fi
     Since Slater's condition is satisfied, and the KKT theorem \cite{kuhn1951kkt} applies, which means that for all $\outer \in \outerset$ and $\inner \in \innerset$, the optimal KKT multipliers $\left\{{\langmult^{(\iter)}}^*\right\}_{\iter = 1}^\infty$ exist and are well-defined: i.e, there exists $c \in \R_+$ such that $\forall \numconstr \in [\numconstrs], 0 \leq \langmult[\numconstr]^* \leq c < \infty$, we have:
    \begin{align}
        \statevalue(\outer) 
        &=  \max_{\inner \in  \innerset: \constr(\state, \outer, \inner) \geq \zeros} \min_{ \langmult \in  [0, c]^\numconstrs } \left\{\reward(\state, \outer, \inner) + \discount \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer,  \inner)} \left[\marginal(\state^\prime, \inner) \right]  + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr]\constr[\numconstr]( \outer, \inner) \right\}\\
        &=  \max_{\inner \in  \innerset: \constr(\state, \outer, \inner) \geq \zeros} \ \min_{ \langmult \in  [0, c]^\numconstrs } \left\{\reward(\state, \outer, \inner) + \discount \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \outer,  \inner)} \left[\marginal(\state^\prime, \inner) \right]  +  \sum_{\numconstr = 1}^\numconstrs\langmult[\numconstr]\constr[\numconstr]( \outer, \inner) ) \right\}
    \end{align}
    Additionally, as $\constr[1](\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner)$ are concave in $\outer$ for all $\inner \in \innerset$ and $\min_{ \langmult \in  [0, c]^\numconstrs } \left\{\reward(\state, \outer, \inner) + \discount \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \inner)} \left[\marginal(\state^\prime, \inner) \right]  +  \sum_{\numconstr = 1}^\numconstrs\langmult[\numconstr]\constr[\numconstr]( \outer, \inner) ) \right\}$ is the $\min$-projection of $\lang$ w.r.t. $\langmult$ onto the compact set $[0, c]^\numconstrs$, $\statevalue(\state, \outer)$ must be convex in $\outer$ (\cite{rockafellar2009variational}).
\end{proof}
\fi 
%
% \begin{theorem}[Subdifferential Benveniste-Scheinkman Theorem]
% Consider the bellman equation associated with a recursive optimization problem where $\discount \in (0,1)$:
% \begin{align}
%     \statevalue(\state, \outer) = \max_{\inner \in  \innerset: \constr(\state, \outer, \inner) \geq \zeros} \left\{\reward(\state, \outer, \inner) + \discount \statevalue(\transdeter(\state, \outer, \inner), \outer) \right\}\label{eq:bellman_eq_bs_thm}
% \end{align}
% Suppose that  
% 1.~ $\left\|\reward \right\|_\infty < \infty$,
% 2.~ for all $\inner \in \innerset$, $\reward(\outer, \inner)$, $\constr[1](\state, \outer, \inner), \hdots, \constr[\numconstrs](\state, \outer, \inner)$ are continuous  and concave in $\outer$, 
% 3.~ $\grad[\outer] \reward, \grad[\outer] \constr[1], \ldots, \grad[\outer] \constr[\numconstrs]$ exist for all $\state \in \states, \outer \in \outerset, \inner \in \innerset$,
% 4.~ $\transdeter$ is continuous in $(\outer, \inner)$ (Feller property) and CSD concave, and
% 5.~ Slater's condition holds for the optimization problem, i.e., $\forall \outer \in \outerset, \state \in \states, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\state, \outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$. 
% Let $\innerset^*(\outer) = \argmax_{\inner \in  \innerset: \constr( \outer, \inner) \geq \zeros} \left\{\obj(\outer, \inner) + \discount \statevalue(\transdeter(\state, \outer, \inner)) \right\}$. The subdifferential of $\statevalue$ at $\hat{\outer}$, $\subdiff[\outer] \statevalue(\hat{\outer})$ is given by $\subdiff[\outer]\statevalue(\hat{\outer}) =$
% \begin{align}
%     \mathrm{conv} \left( \bigcup_{\inner^*(\widehat{\outer}) \in \innerset^*(\widehat{\outer})}      \bigcup_{\langmult[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer})) \in \langmults[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer}))} \left\{ \grad[\outer] \obj\left( \widehat{\outer}, \inner^{*}(\widehat{\outer})\right) + \discount  \grad[\outer] \statevalue(\transdeter(\state, \outer, \inner), \outer)+  \right. \right. \notag\\ +  \left. \left. \sum_{\numconstr = 1}^{\numconstrs} \langmult[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer})) \grad[\outer] \constr[k]\left(\widehat{\outer}, \inner^{*}(\widehat{\outer})\right) \right\}
%     \right) \enspace .
% \end{align}
% where $\mathrm{conv}$ is the convex hull operator and $\langmult^*(\widehat{\outer}, \inner^*(\widehat{\outer})) = \left(\langmult[1]^*(\widehat{\outer}, \inner^*(\widehat{\outer})), \ldots, \langmult[\numconstrs]^*(\widehat{\outer}, \inner^*(\widehat{\outer})) \right)^T \in \langmults^*(\widehat{\outer}, \inner^*(\widehat{\outer}))$ are the optimal KKT multipliers associated with $\inner^{*}(\widehat{\outer}) \in \innerset^*(\widehat{\outer})$.
% \end{theorem}
%
% The above result more generally applies to recursive optimization problem which are stochastic, with the exact proof, and we have:
% \begin{theorem}[Subdifferential Benveniste-Scheinkman Theorem]
% Consider the bellman equation associated with a stochastic Markov recursive optimization problem where $\discount \in (0,1)$:
% % \footnote{Note that in the recursive equation below, $\statevalue(\state^\prime, \inner)$ could instead be written as $\statevalue(\state^\prime)$ as is standard in the reinforcement learning literature by a reconfiguration of the state space and the probability transition function.}
% \begin{align}
%     \statevalue(\state, \outer, \inner) = \max_{\inner \in  \innerset: \constr( \outer, \inner) \geq \zeros} \left\{\obj(\state, \outer, \inner) + \discount  \statevalue(\state^\prime, \outer, \inner)  \right\}\label{eq:bellman_eq_bs_thm}
% \end{align}
% Suppose that  
% 1.~ $\left\|\reward \right\|_\infty < \infty$,
% 2.~ for all $\inner \in \innerset$ $\reward(\outer, \inner)$, $\constr[1], \hdots, \constr[\numconstrs]$ are continuous and concave in $\state$, 
% 3.~ $\trans(\state \mid \state, \outer, \inner)$ is continuous in $(\outer, \inner)$ (Feller property) and CSD concave, and
% 4.~ Slater's condition holds for the optimization problem, i.e., $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$. Let $\innerset^*(\outer) = \argmax_{\inner \in  \innerset: \constr( \outer, \inner) \geq \zeros} \left\{\obj(\outer, \inner) + \discount \statevalue(\inner) \right\}$, then the subdifferential of $\statevalue$ w.r.t $\outer$ exist for all $\outer \in \outerset$ and is given by:
%
% The subdifferential of $\statevalue$ at $\hat{\outer}$, $\subdiff[\outer] \statevalue(\hat{\outer})$ is given by:
% \begin{align}
%     \subdiff[\outer]\statevalue(\hat{\outer}) =
%     \mathrm{conv} \left( \bigcup_{\inner^*(\widehat{\outer}) \in \innerset^*(\widehat{\outer})}      \bigcup_{\langmult[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer})) \in \langmults[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer}))} \left\{ \grad[\outer] \obj\left( \widehat{\outer}, \inner^{*}(\widehat{\outer})\right) + \sum_{\numconstr = 1}^{\numconstrs} \langmult[\numconstr]^*(\widehat{\outer}, \inner^*(\widehat{\outer})) \grad[\outer] \constr[k]\left(\widehat{\outer}, \inner^{*}(\widehat{\outer})\right) \right\}
%     \right) \enspace .
% \end{align}
%
% \end{theorem}
%
A consequence of our subdifferential version of the Benveniste-Scheinkman theorem is that we can easily derive the first-order necessary 
% and sufficient optimality 
conditions for a policy profile to be a \recSE{} of any zero-sum stochastic Stackelberg game $\game$ satisfying \Cref{assum:main}, under standard regularity conditions.

\begin{restatable}{theorem}{thmnecessaryconditions}
\label{thm:necessary_conditions}
Consider a zero-sum stochastic Stackelberg game $\game$, where $\outerset = \{\outer \in \R^\outerdim \mid \outerconstr[1](\outer)\leq 0, \hdots, \outerconstr[\outernumconstrs](\outer) \leq 0 \}$ and $\innerset = \{\inner \in \R^\innerdim \mid 
\innerconstr[1](\inner)\geq 0, \hdots, \innerconstr[\innernumconstrs](\inner)  \geq 0 \}$ are convex.
Let $\lang[\state, \outer](\inner, \langmult) =  \reward(\state, \outer, \inner) + \discount \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[\statevalue(\staterv^\prime, \outer) \right] +  \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\state, \outer, \inner)$ where $\bellopt \statevalue = \statevalue$.

Suppose that  \Cref{assum:main} holds, and that 
1.~for all $\state \in \states$,
$\max_{\inner \in \innerset: \constr(\state, \outer, \inner) \geq \zeros} \left\{ \reward(\state, \outer, \inner) + \discount \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[\statevalue(\staterv^\prime, \outer) \right] \right\}$
is
% $\reward(\state, \outer, \inner)$, $\constr[1](\state, \outer, \inner), \hdots, \constr[\numconstrs](\state, \outer, \inner)$ are
% continuous and 
concave in $\outer$, 
2.~$\grad[\outer] \reward(\state, \outer, \inner), \grad[\outer] \constr[1](\state, \outer, \inner), \ldots, \grad[\outer] \constr[\numconstrs](\state, \outer, \inner)$, $\grad[\inner] \reward(\state, \outer, \inner), \grad[\inner] \constr[1](\state, \outer, \inner), \ldots, \grad[\inner] \constr[\numconstrs](\state, \outer, \inner)$ exist, for all $\state \in \states, \outer \in \outerset, \inner \in \innerset$,
4.~$\trans(\state^\prime \mid \state, \outer, \inner)$ is continuous
% CSD convex 
and differentiable in $(\outer, \inner)$, and
5.~Slater's condition holds, i.e., $\forall \state \in \states, \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $\constr[\numconstr](\state, \outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$ and $\innerconstr[j](\widehat{\inner})  > 0$, for all $j = 1, \hdots, \innernumconstrs$, and $\exists \outer \in \R^\outerdim$ s.t. $\outerconstr[\numconstr](\outer) < 0$ for all $\numconstr =1 \hdots, \outernumconstrs$.
Then, there exists $\bm{\mu}^*: \states \to \R_+^\outernumconstrs$, $\langmult^* : \states \times \outerset \to \R_+^\numconstrs$, and $\bm{\nu}^* : \states \times \outerset \to \R_+^\innernumconstrs$ s.t.\ a policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a \recSE{} of $\game$ only if it satisfies the following conditions, for all $\state \in \states$:
\begin{align}
    % &\statevalue[][{\policy[\inner]^*}][{\policy[\inner]^*}](\state) = \left( \bellopt \statevalue[][{\policy[\inner]^*}][{\policy[\inner]^*}]\right)(\state) \\%&& \forall \state \in \states\\
    &\grad[\outer] \lang[\state, {\policy[\outer]^*(\state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) + \sum_{\numconstr = 1}^\outernumconstrs \mu^*_\numconstr(\state) \grad[\outer]\outerconstr[\numconstr](\policy[\outer]^*(\state)) = 0\\
    &\grad[\inner] \lang[\state, {\policy[\outer]^*( \state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) + \sum_{\numconstr = 1}^\innernumconstrs \nu^*_\numconstr(\state, \policy[\outer]^*(\state)) \grad[\outer]\innerconstr[\numconstr](\policy[\inner]^*(\state)) = 0
\end{align}
% \end{align}
% \vspace{-7em}
\begin{align}
    &\mu^*_\numconstr(\state)\outerconstr[\numconstr](\policy[\outer]^*(\state)) = 0 &\outerconstr[\numconstr](\policy[\outer]^*(\state)) \leq 0 && \forall \numconstr \in [\outernumconstrs]\\
    % &\outerconstr[\numconstr](\policy[\outer]^*(\state)) \leq 0 && \forall \numconstr \in [\outernumconstrs]\\
    &\constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) \geq 0 &\langmult[\numconstr]^*(\state, \policy[\outer]^*(\state)) \constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) = 0  && \forall \numconstr \in [\numconstrs]\\
    % &\langmult[\numconstr]^*(\state, \policy[\outer]^*(\state)) \constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) = 0 && \forall \numconstr \in [\numconstrs]\\
    &\nu^*_\numconstr(\state, \policy[\outer]^*(\state)) \grad[\outer]\innerconstr[\numconstr](\policy[\inner]^*(\state)) = 0  &\innerconstr[\numconstr](\policy[\outer]^*(\state)) \geq 0 && \forall \numconstr \in [\innernumconstrs]
    % &\innerconstr[\numconstr](\policy[\outer]^*(\state)) \geq 0 && \forall \numconstr \in [\innernumconstrs]
\end{align}
    % \begin{align}
    %  \statevalue(\state^\prime, \policy[\outer]^*(\state)) = \reward(\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) + \discount \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \policy[\outer]^*(\state), \policy[\inner]^*(\state))} \left[\statevalue(\state^\prime, \policy[\outer]^*(\state)) \right]\\
    %   \grad[\outer] \lang[\state, {\policy[\outer]^*(\state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) + \sum_{k = 1}^p \mu^*_k(\state) \grad[\outer]r_p(\policy[\outer]^*(\state)) = 0\\
    %   \grad[\inner] \lang[\state, {\policy[\outer]^*( \state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) = 0\\
    %   \langmult[\numconstr]^*(\state, \policy[\outer]^*(\state)) \constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) = 0 && \forall \numconstr \in [\numconstrs]\\
    %   \constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) \geq 0 && \forall \numconstr \in [\numconstrs]\\
    %   \mu^*_k(\state) r_p(\policy[\outer]^*(\state)) = 0 && \forall \numconstr \in [p]\\
    %   r_p(\policy[\outer]^*(\state)) \leq 0 && \forall \numconstr \in [p]
    % \end{align}
%     \begin{figure*}[[h]
% \noindent\begin{minipage}[t]{.55\textwidth}
%     \begin{align}
%         &\statevalue[][{\policy[\inner]}][{\policy[\inner]^*}](\state) = \left( \bellopt \statevalue[][{\policy[\inner]}][{\policy[\inner]^*}]\right)(\state) \hspace{120pt} \forall \state \in \states\\
%         % \notag \\ &+ \discount \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \policy[\outer]^*(\state), \policy[\inner]^*(\state))} \left[\statevalue(\state^\prime, \policy[\outer]^*(\state)) \right]\\
%       &\grad[\outer] \lang[\state, {\policy[\outer]^*(\state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) + \sum_{k = 1}^p \mu^*_k(\state) \grad[\outer]r_p(\policy[\outer]^*(\state)) = 0\\
%       &\grad[\inner] \lang[\state, {\policy[\outer]^*( \state)}](\policy[\inner]^*(\state), \langmult^*(\state, \policy[\outer]^*(\state))) = 0
%     \end{align}
% \end{minipage}%
% \begin{minipage}[t]{.45\textwidth}
%     \begin{align}
%         &\langmult[\numconstr]^*(\state, \policy[\outer]^*(\state)) \constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) = 0 && \forall \numconstr \in [\numconstrs]\\
%       &\constr[\numconstr](\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state)) \geq 0 && \forall \numconstr \in [\numconstrs]\\
%       &\mu^*_k(\state)r_p(\policy[\outer]^*(\state)) = 0 && \forall \numconstr \in [p]\\
%       &r_p(\policy[\outer]^*(\state)) \leq 0 && \forall \numconstr \in [p]
%     \end{align} 
% \end{minipage}
% \end{figure*}
\end{restatable}

Under the conditions of \Cref{thm:necessary_conditions}, if we additionally assume that
for all $\state \in \states$ and $\outer \in \outerset$, both $\reward(\state, \outer, \inner)$ and $\constr[1](\state, \outer, \inner), \hdots, \constr[\numconstrs](\state, \outer, \inner)$
%\amy{$\constr(\state, \outer, \inner)$}\deni{$\constr$ is vector valued, concavity is ill-defined} 
are concave in $\inner$, and $\trans(\state^\prime \mid \state, \outer, \inner)$ is continuous, CSD concave in $ \inner$, and differentiable in $(\outer, \inner)$, 
% concavity of $\max_{\inner \in \innerset : \constr(\state, \outer, \inner)\geq \zeros} \left\{\reward(\state, \outer, \inner) + \discount \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \statevalue[](\staterv^\prime)  \right] \right\}$ 
% becomes a concave optimization problem
% in $\outer$,
\Crefrange{eq:optimality_inner_1}{eq:optimality_inner_5} become necessary \emph{and sufficient} optimality conditions.
For completeness, the reader can find the necessary and sufficient optimality conditions for convex-concave stochastic Stackelberg games under standard regularity conditions in \Cref{thm:necessary_sufficient_conditions} (\Cref{sec_app:benveniste}).
The proof follows exactly as that of \Cref{thm:fp_bellopt_is_stackelberg}.

% \deni{Add that when it is convex concave this becomes necessary and sufficient.}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/todo.tex <==
% Outline:
% \begin{itemize}
%     \item Intro 
%     \item Preliminaries
%     \item Generalized Stackelberg games existence + Arrow-Debreu exchange markets equivalence with markets
%     \item Stochastic Generalized Stackelberg Games, existence + computation via VI
%     \item Recursive Arrow-Debreu Markets, existence + computation via VI for Recursive Fisher markets
%     \item Experiments: Convergence rates
%     \item Conclusion
% \end{itemize}

==> Zero-Sum Stochastic Stackelberg Games (NeurIPS 2022)/zerosum.tex <==




==> arrowdebreu.tex <==



\section{Arrow-Debreu Exchange Markets as Generalized Stackelberg Games}

In this section, we show that any competitive equilibrium of an Arrow-Debreu Markets are instances of Stackelberg games. An \mydef{Arrow-Debreu Exchange economy} $(\numbuyers, \numgoods, \util, \consendow)$ is a barter economy where a finite set of $\numbuyers$ traders, trade a finite set of $\numgoods$ goods. Every trader $\buyer \in \buyers$ is characterized by a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$, and an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$. For ease of notation, we denote $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and $\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. An instance of an Arrow-Debreu market is given by a tuple $(\numbuyers, \numgoods, \consumptions, \util, \consendow)$. When clear from context, we abbreviate $(\util, \consendow)$.

An \mydef{allocation} $\allocation \in \consumptions$ is a map from goods to buyers, represented as a matrix, s.t. $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$. We define a \mydef{price space} $\pricespace = \left\{ \price \ | \ \ \price[\good] \geq 0, \ \sum_{\good = 1}^{\numgoods} \price[\good] = 1 \right\}$.  Goods are assigned \mydef{prices} $\price \in \pricespace$. 
An outcome of the model is a tuple $\left( \allocation, \price \right) \in \consumptions \times \pricespace$.


A tuple $\left(\allocation^*, \price^* \right) \in \consumptions \times \pricespace$ consisting of allocations and prices respectively is a \mydef{competitive equilibrium} iff 1.~ traders maximize their utility over their \mydef{budget set}, i.e., for all $\buyer \in \buyers$  $\allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, and 2.~ the markets for each good clears and goods that are not entirely cleared are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ (\mydef{feasibility condition}) and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$ (\mydef{Walras' law}).

We formulate a Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ where:
%
\begin{align}\label{eq:stackelberg_arrow_debreu_game1}
    \util[\price](\price, \allocation) &= \sum_{\good \in \goods}  \min \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\
    \util[\allocation](\price, \allocation) &= \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
    \constr(\price, \allocation) &= \consendow \price - \allocation \price\label{eq:stackelberg_arrow_debreu_game3}
    % \\\pricespace = \pricespace \cap \{\sum_{\buyer \in \buyers} \bu \}
\end{align} 
%
\noindent
whose set of Stackelberg equilibria is equal to the set of Arrow-Debreu equilbria $(\util, \consendow)$ of a corresponding market. We note that for ease of exposition, we restrict ourselves to the Arrow-Debreu exchange market but the Stackelberg game we propose can easily be extended to Arrow-Debreu production economies by adding to the payoff function of the inner player, the profits of the firms, as well as the associated production constraints to the function $\constr$.

\begin{assumption}\label{assum:arrow_debreu}
Suppose that for all $\buyer \in \buyers$, 
1.~$\util[\buyer]$ is a continuous, and concave utility function representing locally non-satiated preferences,
2.~$\consumptions[\buyer]$ is non-empty, compact, and convex, 
3.~and that there exists an interior point for each consumer's utility maximization problem, i.e., $\exists \allocation \in \consumptions$ s.t. $\allocation[\buyer] \cdot \price < \consendow[\buyer] \cdot \price$
\end{assumption}

Before introducing the main theorems regarding this Stackelberg game, we introduce some important lemmas. First, we note that a Stackelberg equilibrium is guaranteed to exist in this game.

\begin{lemma}
Under \Cref{assum:arrow_debreu}, the set of Stackelberg equilibria of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ as defined in \Crefrange{eq:stackelberg_arrow_debreu_game1}{eq:stackelberg_arrow_debreu_game3} is non-empty and compact.\deni{Make sure the compactness theorem is correct}
\end{lemma}
\begin{proof}
    Since the $\min$ and $\max$ operators preserve continuity, $\util[\price]$ is also continuous. Additionally, under \Cref{assum:arrow_debreu}, $\util[\allocation]$ is also continuous since it is a sum of continuous functions and $\consumptions$ is non-empty and compact since it is a product of non-empty and compact sets. Finally, since $\constr$ is continuous, and $\pricespace$ is non-empty and compact, by \Cref{thm:exitence_stackelberg} a Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is guaranteed to exist.
\end{proof}

The following lemma states important properties of the inner player's Stackelberg equilibrium strategies.
\begin{lemma}\label{lemma:inner_arrow_debreu_optimality}
Consider the solution to the inner player's optimization problem $\allocation^* \in \argmax_{\allocation \in \consumptions: \allocation \price^* \leq \consendow \price^*} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])$ for the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ given an arbitrary strategy of the outer player $\price^*$. Suppose that \Cref{assum:arrow_debreu} holds, then $\allocation^*$ is optimal for the outer player iff we have that for all buyers $\buyer \in \buyers$:

1.~ $\allocation[\buyer]^*$ is a utility maximizing allocation over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, 
% i.e., $\allocation[\buyer]^* \in \argmax_{\allocation[ ]\in \consumptions[\buyer] : \allocation[ ] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \util[\buyer](\allocation[ ])$, and
2.~ $\allocation[\buyer]^*$ consumes the entire budget of consumer $\buyer$, i.e., $\allocation[\buyer]^* \cdot \price^* = \consendow[\buyer] \cdot \price^*$.
\end{lemma}
\begin{proof}

Consider the inner player's optimization problem for the Stackelberg equilibrium strategy of the outer player $\price^*$ $\max_{\allocation \in \consumptions: \allocation \price^* \leq \consendow \price^*} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])$. By the assumption of existence of an interior point in the budget set of all consumers, Slater's condition is satisfied for the inner player's problem, and there exists KKT multlipliers $\bm \lambda^* \in \R^\numbuyers_+$ which satisfy the necessary and sufficient KKT conditions. From the first order optimality conditions, we have:
\begin{align}
    \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \util[\allocation](\allocation) \right]_{\allocation = \allocation^*} + \sum_{\buyer \in \buyers} \lambda^*_\buyer \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \constr[\buyer](\price^*, \allocation[\buyer])\right]_{\allocation = \allocation^*} &\doteq 0 && \forall \buyer \in \buyers, \good \in \goods\\
    \frac{\partial }{\partial \allocation[\buyer][\good]} \left[ \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\right]_{\allocation = \allocation^*} + \sum_{\buyer \in \buyers} \lambda^*_\buyer \frac{\partial }{\partial \allocation[\buyer][\good]}  \left[ \consendow[\buyer] \cdot \price^* - \allocation[\buyer] \cdot \price^*\right]_{\allocation[\buyer] = \allocation[\buyer]^*} &= 0  && \forall \buyer \in \buyers, \good \in \goods\\
    \left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]} \right]_{\allocation[\buyer] = \allocation[\buyer]^*}- \lambda^*_\buyer \price[\good]^* &= 0  && \forall \buyer \in \buyers, \good \in \goods\\
    \lambda^*_\buyer &= \frac{\left[\frac{\partial \util[\buyer]}{\partial \allocation[\buyer][\good]}\right]_{\allocation[\buyer] = \allocation[\buyer]^*}}{\price[\good]^*} && \forall \buyer \in \buyers, \good \in \goods
\end{align}
where the last line is the equimarginal principle and implies that for all $\buyer \in \buyers$  $\allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$. 
% Hence, $(\price^*, \allocation^*)$ satisfies the first condition of being a competitive equilibrium.

Similarly, from the KKT necessary and sufficient complementarity conditions, we have that for all $\buyer \in \buyers$:
\begin{align}
    \lambda_\buyer^* \constr[\buyer](\price^*, \allocation[\buyer]^*) = 0\\
    \lambda_\buyer^* \left(\consendow[\buyer] \cdot \price^* - \allocation[\buyer]^* \cdot \price^* \right) = 0
\end{align}
It is well-known that for all traders $\buyer \in \buyers$, $\lambda^*$ corresponds to the marginal utility of money, i.e, the derivative of the indirect utility function of buyer $\buyer$ w.r.t. their budget. Since the utility function of each trader is locally non-satiated, we must have that $\lambda_\buyer^* > 0$, which gives us:
%
\begin{align}
    \left(\consendow[\buyer] \cdot \price^* - \allocation[\buyer]^* \cdot \price^* \right) = 0\\
    \price^* \cdot\left(\consendow[\buyer]  - \allocation[\buyer]^*  \right) = 0\label{eq:lower_level_walras_law}
\end{align}
% Summing over all the buyers, we obtain that $(\price^*, \allocation^*)$ satisfies the second part of the second condition to be a competitive equilibrium.
\end{proof}


\begin{lemma}\label{lemma:outer_player_max_utility_arrow_debreu}
The utility achieved by the outer player in the game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is upper bounded by 0 for any feasible strategy profile $(\price, \allocation)$, i.e.,  $\util[\price](\price, \allocation) \leq 0$ for all $(\price, \allocation) \in \pricespace \times \left\{ \allocation \ | \ \ \allocation \in \consumptions \ \ \allocation  \price^* \leq \consendow \price^*  \right\}$.
\end{lemma}
\begin{proof}
\begin{align}
    \util[\price](\price^*, \allocation^*) &= \sum_{\good \in \goods}  \min \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\
    &\leq 0 - \sum_{\good \in \goods}  \price[\good] \max \left\{ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right\} \\ 
    &\leq - \sum_{\good \in \goods}  \price[\good] \cdot (0) \\
    &= 0
\end{align}
\deni{Make sure to add that $\price$ is feasible so  equation 16 holds.}
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_price_zero}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. Then, at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ if for any $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$.
\end{lemma}

\begin{proof}
For notational clarity, define the excess supply function associated with an optimistic best-response of the inner player $\s(\price) = \sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price)$ where: 
\begin{align}
\calD^*(\price) &= \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) &\in \argmax_{\allocation \in \calD^*(\price)} \left\{ \sum_{\good \in \goods}  \min \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) - \sum_{\good \in \goods}  \price[\good] \max \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) \right\}
\end{align}
% For the sake of contradiction, suppose that $\util[\price](\price^*, \allocation*) < 0$. Then, there must exist a set of good $\calG$ such that for all $k \in \calG$ either $s_k(\price^*) < 0$ or  $s_k(\price^*) > 0$ and $\price[k] > 0$.
By the necessary optimality conditions for the outer player's Stackelberg equilibrium strategy over the set $\pricespace$ \cite{} \deni{Cite Dempe theorem 5.6} we have:

\begin{align}
     \subdiff[{\price[\good]}] \util[\price](\price^*, \allocation^*(\price^*)) &\doteq 0\\
    \sum_{\good \in \goods} \subdiff[{\price[\good]}]\left( \min \left\{ s_\good(\price^*), 0 \right\}\right) - \max\left\{ s_\good(\price^*), 0\right\} - \sum_{\good \in \goods} \price[\good] \subdiff[{\price[\good]}] \max\left\{ s_\good(\price^*), 0\right\} &= 0
\end{align}\deni{note: above $\subdiff[{\price[\good]}]$ is the generalized Clark derivative, which is a generalization of subgradients.}
Suppose that $s_\good(\price^*) > 0$, the above condition then reduces to:
\begin{align}
    \sum_{\good \in \goods} \subdiff[{\price[\good]}] (0)  - s_\good(\price^*) - \sum_{\good \in \goods} \price[\good]  \subdiff[{\price[\good]}] s_\good(\price^*) = 0\\
    - s_\good(\price^*) - \sum_{\good \in \goods} \price[\good]  \subdiff[{\price[\good]}] s_\good(\price^*) = 0\\
    - s_\good(\price^*) + \sum_{\good \in \goods} \price[\good] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good](\price^*) = 0
\end{align}

\noindent
For the above equation to be true it must be that either $\price[\good] = 0$ or 
\begin{align}
    \price[\good] &> 0\\
      \sum_{\good \in \goods} \price[\good]  \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}]  \allocation[\buyer][\good](\price^*) &= s_\good(\price^*) \enspace .\label{eq:case2_price_zero_excess_supply}
\end{align} 

We will show that the later case occuring is a contradiction.

\noindent
Recall from \Cref{lemma:outer_player_max_utility_arrow_debreu} that for any $\price \in \pricespace$:
\begin{align}
    \sum_{k \in \goods} \allocation[\buyer][k]^*(\price) \price[k] = \sum_{k \in \goods} \consendow[\buyer][k] \price[k]
\end{align}
Taking the generalized Clarke derivative of both sides, we obtain:
\begin{align}
    \allocation[\buyer][\good]^*(\price) + \sum_{k \in \goods} \price[k] \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) = \consendow[\buyer][\good]
\end{align}
Re-organizing expressions and summing over all $\buyer \in \buyers$, we obtain:
\begin{align}
   \sum_{k \in \goods}\price[k] \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) =  \consendow[\buyer][\good] - \allocation[\buyer][\good]^*(\price) \\
    \sum_{k \in \goods} \price[k] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][k]^*(\price) =  \sum_{\buyer \in \buyers}\consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price)
\end{align}
Note that we have $\sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good]^*(\price)  = \subdiff[{\price[\good]}] s_\good(\price)$ by the definition of $\s$. Hence, we can re-write the above as:
\begin{align}
    \sum_{\good \in \goods} \price[\good] \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \allocation[\buyer][\good]^*(\price)  = s_\good(\price) 
\end{align}
which is in contradiction with \Cref{eq:case2_price_zero_excess_supply} and the assumption that $s_\good > 0$ implying that if $s_\good(\price^*) > 0$, we must have $\price[\good] = 0$.
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_feasible}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. Then, at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ then, for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$.
\end{lemma}

\begin{proof}
For notational clarity, let $\excessdemand(\price) = \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price)$ where: 
\begin{align}
\calD^*(\price) &= \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) &\in \argmax_{\allocation \in \calD^*(\price)} \left\{ \sum_{\good \in \goods}  \min \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) - \sum_{\good \in \goods}  \price[\good] \max \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good], 0\right) \right\}
\end{align}
Suppose for contradiction, that there exists a maximal set of goods $\calG \subset \goods$ such that for all $\good \in \calG$ $\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* = - \excessdemand[\good](\price^*) < 0$ or equivalently $\excessdemand[\good](\price^*) > 0$. Recall by \Cref{lemma:outer_player_max_utility_arrow_debreu} we have for any $\price \in \pricespace$:
\begin{align}
    \sum_{\good \in \goods} \price[\good]^* \left(\allocation[\buyer][\good]^* - \consendow[\buyer][\good] \right) = 0 && \forall \buyer \in \buyers
\end{align}
Summing up over all $\buyer \in \buyers$, we obtain Walras' law:
\begin{align}
    \sum_{\good \in \goods} \sum_{\buyer \in \buyers} \price[\good]^* \left(\allocation[\buyer][\good]^* - \consendow[\buyer][\good] \right) = 0 \\
    \sum_{\good \in \goods} \price[\good] \excessdemand[\good](\price^*) = 0 \\
    \sum_{\good \in \calG} \price[\good] \excessdemand[\good](\price^*) + \sum_{\good \in (\goods - \calG)} \price[\good] \excessdemand[\good](\price^*) = 0 \\
\end{align}
Note that by \Cref{lemma:stackelberg_arrow_debreu_price_zero}, we have that $\sum_{\good \in (\goods - \calG)} \price[\good] \excessdemand[\good](\price^*) = 0$ where $(\goods - \calG) \subset \goods$ is the set of good such that for all $\good \in (\goods - \calG), \excessdemand[\good](\price^*) \leq 0$.
\begin{align}
    \sum_{\good \in \calG} \price[\good] \excessdemand[\good](\price^*) = 0 
\end{align}
which is a contradiction. 
\end{proof}

\begin{lemma}\label{lemma:stackelberg_arrow_debreu_value}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. The payoff of the outer player at any Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ is 0, i.e., $\util[\price](\price^*, \allocation^*) = 0$. Additionally, a strategy of the outer player $\price^*$ is Stackelberg equilibrium strategy for $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ iff 
1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$.
\end{lemma}

\begin{proof}
Combining \Cref{lemma:stackelberg_arrow_debreu_feasible} and \Cref{lemma:stackelberg_arrow_debreu_price_zero} we see that . For the other direction, we note that $\util[\price](\price^*, \allocation^*) = 0$. Additionally, this also means that if 1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then the utility of the outer player is $0$, which means that $\price^*$ is a Stackelberg equilibrium strategy.

To obtain the other direction, we simply note that $\util[\price](\allocation^*, \price^*)  = 0$, which is only possible if 1.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, then we have $\price[\good] = 0$, and
2.~ for all $\good \in \goods$, $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* > 0$, which
\end{proof}

\begin{theorem}
Consider the Stackelberg game $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$ and suppose that \Cref{assum:arrow_debreu} holds. 
Any competitive equilibrium $(\allocation^*, \price^*)$ of the Arrow-Debreu Market $(\util, \consendow)$ is also a Stackelberg equilibrium $(\price^*, \allocation^*)$ of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$. 
% \deni{Need the outer player's action set to be the intersection of the prices space and prices that satisfy walras' law.}
\end{theorem}
% \deni{Need some Slater like condition \`a la Arrow-Debreu}

\begin{proof}

(Set of Arrow-Debreu Equilibria  $\subseteq$ Set of Stackelberg equilibria):

Let $(\allocation^*, \price^*)$ be an Arrow-Debreu equilibrium of  $(\consendow, \util)$, then the by the feasibility requirement of a competitive equilibrium, we have that for all $\good \in \goods$: $\sum_{\buyer \in \buyers} \allocation[\buyer][\good] - \sum_{\buyer \in \buyers}  \consendow[\buyer][\good] \leq 0$ or equivalently $ \sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good] \geq 0$. Additionally, by Walras' law we know that $\price \cdot \left(\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer] \geq 0 \right) = 0$. Combining these two facts, we must have that $\util[\price](\allocation^*, \price^*) = 0$. Since the payoff of the outer player at s Stackelberg equilibrium is $0$ (\Cref{lemma:stackelberg_arrow_debreu_value}), we must have that $\price^*$ is a Stackelberg equilibrium strategy for the outer player. Additionally, since $\allocation^*$ is utility maximizing constrained by budget and Walras' law is satisfied by \Cref{lemma:inner_arrow_debreu_optimality} we have that $\allocation^*$ is a best-response of the inner player for $\price^*$. Hence, $(\price^*, \allocation^*)$ is a Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$.  
 
\noindent
(Set of Stackelberg equilibria  $\subseteq$ Set of Arrow-Debreu Equilibria):

Let $(\price^*, \allocation^*)$ be Stackelberg equilibrium of $(\pricespace, \consumptions, \util[\price], \util[\allocation], \constr)$, then by \Cref{lemma:stackelberg_arrow_debreu_value} the second condition of a competitive equilibrium is fullfilled. Additionally, by \Cref{lemma:inner_arrow_debreu_optimality} $\allocation^*$ is the budget constrained utility maximizing allocation associated with with $\price^*$, fulfilling the first condition of a competitive equilibrium. Hence, $(\price^*, \allocation^*)$ is a competitive equilibrium.






\if 0

Suppose the following:
\begin{align}
\calD^*(\price) = \argmax_{\allocation \in \consumptions: \allocation \price \leq \consendow \price} \sum_{\buyer \in \buyers} \util[\buyer](\allocation[\buyer])\\
\allocation^*(\price) \in \argmax_{\allocation \in \calD^*(\price)} - \sum_{\good \in \goods} (\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price))^2
\end{align}
 The necessary optimality condition for the outer player's Stackelberg equilibirium strategy, is given by the first order optimality condition for $\max_{\price \in \pricespace}- \frac{1}{2} \left\|\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer](\price)\right\|_2^2$. 
%  $\allocation[\buyer][\good]^*(\price) \in \argmax_{\allocation \in D(\price)} - \sum_{\good \in \goods} (\sum_{\buyer \in \buyers} \consendow[\buyer][\good] - \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price))^2$, that is:
\begin{align}
    \frac{\partial }{\partial \price[\good]} \left( - \frac{1}{2} \left\|\sum_{\buyer \in \buyers} \consendow[\buyer] - \sum_{\buyer \in \buyers} \allocation[\buyer]\right\|_2^2\right) &\doteq 0 && \forall \good \in \goods\\
    \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) &= 0  && \forall \good \in \goods\\
    % \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) \price[\good] &= 0  && \forall \good \in \goods
    % \left( \sum_{\buyer \in \buyers} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*)\right) \left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]}\right) &= 0
\end{align}
% Summing the above for all goods $\good \in \goods$, we obtain:
% \begin{align}
%     \left( \sum_{\buyer \in \buyers} \consendow[\buyer] -  \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price^*)\right) \sum_{\good \in \goods}\left( \sum_{\buyer \in \buyers} \price[\good] \frac{\partial\allocation[\buyer]^*(\price^*)}{\partial \price[\good]}\right) &= 0\\
% \end{align}
If $\sum_{\good \in \good} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*) = 0$ or if $ \sum_{\good \in \good} \consendow[\buyer][\good] -  \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\price^*) = 0$ \emph{and} $\sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = 0$, then the first part of the second condition for a competitive equilibrium is satisfied. We are left to check that if we only have $\sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price^*)}{\partial \price[\good]} = 0$, the good must be not demanded.
Suppose that $\left( \sum_{\buyer \in \buyers} \frac{\partial\allocation[\buyer][\good]^*(\price)}{\partial \price[\good]}\right) > 0$,   the good is not demanded by any buyer, in which case 

\fi 
\end{proof}

\subsection{Recursive Arrow-Debreu Markets}


A \mydef{recursive Arrow-Debreu Exchange market} consists of:
\begin{enumerate}
    \item A set of states $\states$, describing the state in which the market is.
    \item A initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
    \item A transition function $\trans: \states \times \states \times \R_+^\numgoods \times \R_+^{\numgoods \times \numbuyers} \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when prices $\price \in  \R_+^{\numgoods} $ and allocations $\allocation \in  \R_+^{\numgoods \times \numbuyers} $ are determined by the supply and demand sides respectively, is denoted by $\trans(\state^\prime \mid \price, \allocation)$.
    \item A set of $\numgoods$ goods.
    \item A set of $\numbuyers$ buyers. Each buyer $\buyer \in \buyers$ has a 
    \begin{enumerate}
        \item a continuous and concave utility function $\util[\buyer]: \states \times \R^\numgoods \to \R$
        \item an endowment at each state $\consendow[\buyer]: \states \to \R_+$
    \end{enumerate}
    \item a probability $\discount$ that the market will continue
\end{enumerate}

A recursive Fisher market is denoted by a tuple $(\numbuyers, \numgoods, \states, \initstates, \util, \budget, \supply, \discount)$. When clear from context, we simply write $(\states, \initstates, \util, \budget, \discount)$.

An \mydef{allocation} $\allocation \in \R^{\numbuyers \times \numgoods}_+$ is a mapping from buyers to goods such that $\allocation[\buyer][\good] \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$.
%
An \mydef{allocation system} $\allocation: \states \to \R^{\numbuyers \times \numgoods}$ is a mapping from states to allocations of goods to buyers such that $\allocation[\buyer][\good](\state) \geq 0$ denotes the quantity of good $\good$ allocated to buyer $\buyer$ in state $\state$. 
%
Goods are assigned anonymous \mydef{prices} $\price \in \R_+^\numgoods$ such that $\price[\good] \geq 0 $ denotes the cost of one unit of good $\good$ for any buyer.
%
A \mydef{price system} is a mapping $\price: \states \to \R^\numgoods_+$ from states to prices such that for all $\good \in \goods$ and $\state \in \states$, $\price[\good](\state) \geq 0$ denotes the price of good $\good$ in state $\state$.
A \mydef{recursive competitive equilibrium} is a tuple $(\allocation^*, \price^*)$. which consists of an allocation system and a price system such that:
\begin{enumerate}
    \item The buyers are expected utility maximizing: 
    \begin{align}
        \forall \buyer,\;\allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \R^{\numgoods \times \states} : \forall \state \in \states \allocation[\buyer](\state) \cdot \price(\state) \leq \consendow[\buyer](\state) \cdot \price(\state)} \E \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer](\staterv[\iter])) \right]
    \end{align}
    \item The market clears in each state and goods that are unallocated in each state are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\state \in \states$:
    \begin{align}
        \price[\good](\state) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good](\state) = \sum_{\buyer \in \buyers} \consendow[\buyer][\good]\\
        \price[\good](\state) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good](\state) \leq \sum_{\buyer \in \buyers} \consendow[\buyer][\good]
    \end{align}
\end{enumerate}

==> generalsum.tex <==
A \mydef{(generalized) Stackelberg game}, $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$, is a two-player, general-sum game, where one player, who we call the outer, or $\outer$-, player (resp.\ the inner, or $\inner$-, player)\deni{Might want to replace outer and inner with follower and leader}, is trying to maximize their payoff, defined by a \emph{continuous} \mydef{payoff function} $\util[\outer]: X \times Y \rightarrow \mathbb{R}$ (resp. $\util[\inner]: X \times Y \rightarrow \mathbb{R}$), by taking an action from their non-empty and compact \mydef{\sdeni{strategy}{action} set}\deni{first player's action set is equal to their strategy set but this is not the case for the second player. For the second player, the action set is $\innerset$, while the strategy set is $\outerset \times \innerset$, i.e., it is the set of all possible contingent plans.} $\outerset \subset \R^\outerdim$, and (resp. $\innerset \subset \R^\innerdim$) s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1](\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$ continuous. A \mydef{strategy profile} $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff for all $\numconstr \in [\numconstrs]$, $\constr[\numconstr](\outer, \inner) \geq 0$. A Stackelberg game is said to be convex if the actions sets $\outerset, \innerset$ are convex, and for all $(\outer, \inner) \in \outerset \times \innerset$ the payoff functions $\util[\outer](\ \cdot \, \inner), \util[\inner](\outer, \ \cdot \ )$ as well as the constraints $\constr[1](\outer, \ \cdot \ ), \hdots, \constr[\numconstrs](\outer, \ \cdot \ )$, are concave.\deni{Maybe switch from payoff functions to loss functions so that this is more consistent?}
For each outer player's action $\outer \in \outerset$, we define the best-response set of the inner player as $\br(\outer) = \argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)$.
In Stackelberg games, the outer player seeks to maximize their payoff assuming the inner player chooses a feasible best response that maximizes the outer player's payoff, i.e., the outer player maximizes their \mydef{marginal function} \cite{berge1997topological}, is defined as $\marginal[\outer](\outer) = \max_{\inner \in \br(\outer) }  \util[\outer](\outer, \inner)$. Note that for the purposes of our expositions to ensure that $\marginal[\outer]$ is a well-defined function, we assumed in this definition that the follower breaks ties amongst their best-responses in the leader’s favor. This is known as \mydef{optimistic tie breaking} and provides a best-case guarantee for the leader. 
% The inner player's value function, $\val[\innerset]: \outerset \to \R$, which they seek to maximize, is simply the objective function given the outer player's action $\hat{\outer}$: i.e., $\val[\innerset](\inner; \hat{\outer}) = \obj(\hat{\outer}, \inner)$.

A strategy profile $\left(\outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ s.t.\ $\constr(\outer^{*}, \inner^{*}) \geq \zeros$ is an $(\epsilon, \delta)$-\mydef{Stackelberg equilibrium} if
\begin{align}
    \util[\outer](\outer^*, \inner^*) \geq \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner) - \varepsilon && \forall \outer \in \outerset\\
    \util[\inner](\outer^*, \inner^*) \geq \util[\inner](\outer^*, \inner) - \delta 
    && \forall  \inner \in \innerset  \text{ s.t. } \constr(\outer^*, \inner) \geq \zeros
\end{align}

Intuitively, a $(\varepsilon, \delta)$-Stackelberg equilibrium is a point at which the $\outer$-player's (resp.\ $\inner$-player's) payoff is no more than $\varepsilon$ (resp.\ $\delta$) away from its optimum.
A $(0,0)$-Stackelberg equilibrium is guaranteed to exist in Stackelberg games by the following theorem.

\begin{remark}
Note that, to guarantee existence of a Stackelberg equilibrium we assumed \mydef{optimistic tie breaking}. An alternative but as valid way of defining a Stackelberg equilibrium would have been to assume that the follower breaks ties against the leader's favor, i.e., \mydef{pessimistic tie breaking}, in such a case one can similarly show the existence of a Stackelberg equilibrium \cite{}. Historically, the literature on bi-level optimization has focused on the optimistic tie breaking rule as it allows for easier tractability
% However, while pessimistic  tie-breaking guarantees that the set of Stackelberg equilibria is non-empty and compact, optimistic tie-breaking guarantees that the set of Stackelberg equilibria is non-empty, compact, and \emph{convex}, as shown by the following theorem. 
\end{remark}

% The convexity of the set of Stackelberg equilibria allows 
% \subsection{Prperties of Stackelberg Equilibrium in Generalized Stackelberg Games}

% \deni{This assumption is not needed for static setting}

In general, a Nash equilibrium is not guaranteed to exist in convex Stackelberg games but a Stackelberg equilibrium always exists as shown by the following theorem. The following theorem is a slight variant of pre-existing results in the literature as it also shows that the set of Stackelberg equilbiria is compact. 

\begin{theorem}\label{thm:exitence_stackelberg}
% Suppose that parts 2 and 3 of \Cref{assum:stackelberg_general_sum} hold, then t
The set of Stackelberg equilibria of any Stackelberg game $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$ is non-empty and compact.
\end{theorem}

\begin{proof}
First, we note that since for all $\outer \in \outerset$, $\util[\inner](\outer, \inner ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer,\inner )$ are continuous in $\inner$, for all $\outer \in \outerset$, the correspondence $ \calC(\outer) = \{\inner \in  \innerset  \mid \constr(\outer, \inner) \geq \zeros\}$ is compact-valued and continuous. As a result, by the maximum theorem \cite{berge1997topological}, the best-response correspondence $\br$ is non-empty, upper hemicontinuous, compact-valued. Additionally, by Weierstrass's theorem, the set of optimistic best-responses of the inner player for any strategy of the outer player $\outer \in \outerset$, i.e., $\argmax_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ , is compact since $\util[\outer](\outer, \inner)$ is continuous and $\br(\outer)$ is compact. 

Now, we note that since $\br$ is non-empty, upper hemicontinuous, and compact-valued in $\outer$, and $\util[\outer](\outer, \inner)$ is continuous, by Theorem 2 of \citeauthor{berge1997topological} \cite{berge1997topological} the marginal function $\util[\outer]^*(\outer) = \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is upper semi continuous in $\outer$. Since for all $\outer \in \outerset$, $\br(\outer)$ is compact and  $\util[\outer](\outer, \inner)$  is continuous in $\inner$, $\util[\outer]^*(\outer)$ is well-defined for all $\outer \in \outerset$ such that for all $\outer \in \outerset, \left| \util[\outer]^*(\outer) \right| < \infty$, i.e., it is
%  a proper function. and 
level-bounded. By Theorem 1.9 of \citeauthor{rockafellar2009variational} \cite{rockafellar2009variational}, since $\util[\outer]^*$ is upper semicontinuous,
% proper, 
and level-bounded, the set $\argmax_{\outer \in \outerset}  \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is non-empty and compact.
% %
% \noindent
% Since we have shown that $\argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)$ is compact and non-empty, and $\util[\outer]( \ \cdot \, \inner)$ is concave, we have that $\max_{\inner \in \argmax_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \util[\inner](\outer, \inner)} \util[\outer](\outer, \inner)$ is concave in $\outer$.
\end{proof}

\if 0

Next, we prove that the set of Stackelberg equilibria of a Stackelberg game are also convex. Our result depends on the following technical lemma which is a slight more general variant of known results.

\begin{lemma}\label{lemma:max_thm_var}
Consider a parametric optimization problem $\obj^*(\outer) = \max_{\inner \in \calC(\outer)} \obj(\outer, \inner)$. Suppose that $\calC: \outerset \rightrightarrows  \innerset$ is upper hemicontinuous, compact-convex valued, $\outerset \subset \R^\outerdim$ is convex, and $\obj$ is continuous and concave, then 1) $\obj^*(\outer)$ is upper semicontinuous and concave, and 2) $\calC^*(\outer) = \argmax_{\inner \in \calC(\outer)} \obj(\outer, \inner)$ is non-empty-, convex-, and compact-valued.
\end{lemma}

\begin{proof}
By Theorem 2 of \citeauthor{berge1997topological} \cite{berge1997topological} $\obj^*(\outer) = \max_{\inner \in \calC(\outer)} \obj(\outer, \inner)$ is upper semicontinuous in $\outer$ since $\calC$ is upper hemi-continuous and $\obj$ is continuous.

Since for all $\outer \in \R^\outerdim$, $\calC(\outer)$ is compact and  $\obj(\outer, \inner)$  is continuous in $\inner$, $\obj^*(\outer)$ is well-defined for all $\outer \in \R^\outerdim$ such that for all $\outer \in \R^\outerdim, \left| \obj^*(\outer) \right| < \infty$, i.e., $\obj^*$ is a proper function and level-bounded. By Theorem 1.9 of \citeauthor{rockafellar2009variational} \cite{rockafellar2009variational}, since $\obj^*$ is upper semicontinuous, proper, and level-bounded, for all $\outer \in \outerset$, $\calC^*(\outer)$ is non-empty and compact. 

We now prove that $\calC^*(\outer)$ is convex for all $\outer \in \outerset$. Pick $\bar{\inner}, \tilde{\inner} \in \calC^*(\outer^\prime)$, and let $\inner^\prime = \lambda \bar{\inner} + (1-\lambda) \tilde{\inner}$ for $\lambda \in [0,1]$. Note that we have $\inner^\prime \in \calC(\outer^\prime)$ since $\calC(\outer)$ is convex for all $\outer \in \outerset$. We then have by the concavity of $\obj$: 
\begin{align}
    \obj(\outer^\prime, \inner^\prime) &= \obj(\outer^\prime, \lambda \bar{\inner} + (1-\lambda) \tilde{\inner})\\
    &\geq  \lambda \obj(\outer^\prime,\bar{\inner} ) + (1-\lambda) \obj(\outer^\prime,   \tilde{\inner})\\ 
    &= \lambda \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner ) + (1-\lambda) \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner)\\
    &= \max_{\inner \in \calC(\outer^\prime)} \obj(\outer^\prime, \inner)
\end{align}
%
\noindent
which means that $\inner^\prime \in \calC^*(\outer^\prime)$, i.e., $\calC^*$ is convex-valued.


Pick any $\bar{\outer}, \tilde{\outer} \in \outerset$ and let $\outer^\prime = \lambda \bar{\outer} + (1-\lambda)\tilde{\outer}$ for $\lambda \in [0,1]$. By the convexity of $\outerset$, we then have $\outer^\prime \in \outerset$.  Let $\bar{\inner} \in \calC^*(\bar{\outer}) =  \argmax_{\inner \in \calC(\bar{\outer})} \obj(\bar{\outer}, \inner)$,  $\tilde{\inner} \in \calC^*(\tilde{\outer}) = \argmax_{\inner \in \calC(\tilde{\outer})} \obj( \tilde{\outer}, \inner)$, and $\inner^\prime = \lambda \bar{\inner} + (1-\lambda)\tilde{\inner}$. Since $\calC$ is convex-valued and $\outerset$ is convex, $\calC$ has a convex graph and we have $\inner^\prime \in \calC(\outer^\prime)$, which gives us:
\begin{align}
    \obj^*(\outer^\prime) &\geq \obj(\outer^\prime, \inner^\prime) && \text{(By definition of $\obj^*$)} \\
    &= \obj\left(\lambda \bar{\outer} + (1-\lambda)\tilde{\outer},  \lambda \bar{\inner} + (1-\lambda)\tilde{\inner}\right)\\
    &\geq \lambda \obj\left( \bar{\outer}, \bar{\inner} \right) + (1-\lambda) \obj(\tilde{\outer}, \tilde{\inner}) && \text{(Convexity of $\obj$)}\\
    &= \lambda \obj^*(\bar{\outer}) + (1-\lambda) \obj^*(\tilde{\outer})
\end{align}
%
which establishes that $\obj^*$ is concave.
\end{proof}


\deni{Seperate existence and convexity proofs. Existence requires continuous concave in each player's variable + convex constraints, while convex set of solutions requires outer player's payoff to be entire concave. This means that we get existence for both pessimistic and optimistic tie breaking, but we get convexity only for optimisitc tie breaking.}
\begin{theorem}
Suppose that \Cref{assum:stackelberg_general_sum} holds, then the set of Stackelberg equilibria of any convex Stackelberg game $(\outerset, \innerset, \util[\outer], \util[\inner], \constr)$ is non-empty, compact and convex.
\end{theorem}

\begin{proof}
First, we note that since for all $\outer \in \outerset$, $\util[\inner](\outer, \inner ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer,\inner )$ are continuous and concave in $\inner$, 
% for all $\outer \in \outerset$, we have that the set $\{\inner \in  \innerset  \mid \constr(\outer, \inner) \geq \zeros\}$ is compact and convex, and 
by the maximum theorem \cite{berge1997topological}, the best-response correspondence $\br$ is non-empty, upper hemicontinuous, compact-, and convex-valued. Hence, by \Cref{lemma:max_thm_var} the set of optimistic best-responses of the inner player for any strategy of the outer player $\outer \in \outerset$, i.e., $\argmax_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$, is non-empty, convex, and compact since $\util[\outer](\outer, \inner)$ is continuous and concave, and $\br(\outer)$ is compact. Similarly, by \Cref{lemma:max_thm_var} $\util[\outer]^*(\outer) = \max_{\inner \in \br(\outer)} \util[\outer](\outer, \inner)$ is upper semicontinuous and concave.

By \Cref{thm:exitence_stackelberg}, we know that the set of Stackelberg equilibrium strategies of the outer player, \\ i.e. $\argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, is non-empty, and compact, we will show it also is convex.
Pick $\bar{\outer}, \tilde{\outer} \in \argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, and let $\outer^\prime = \lambda \bar{\outer} + (1-\lambda) \tilde{\outer}$ for $\lambda \in [0,1]$. Note that we have $\outer^\prime \in \outerset$ since $\outerset$ is convex for all $\outer \in \outerset$. We then have by the concavity of $\util[\outer]^*$: 
\begin{align}
    \util[\outer]^*(\outer^\prime) &= \util[\outer]^*(\lambda \bar{\outer} + (1-\lambda) \tilde{\outer})\\
    &\geq  \lambda \util[\outer]^*(\bar{\outer} ) + (1-\lambda) \util[\outer]^*(\tilde{\outer})\\ 
    &= \lambda \max_{\outer \in \outerset} \util[\outer]^*(\outer) + (1-\lambda) \max_{\outer \in \outerset} \util[\outer]^*(\outer)\\
    &= \max_{\outer \in \outerset} \util[\outer]^*(\outer)
\end{align}
which means that $\outer^\prime \in \argmax_{\outer \in \outerset} \util[\outer]^*(\outer)$, i.e., the set of Stackelberg equilibrium strategies of the outer player is convex. 
\end{proof}

\fi


In general Stackelberg equilibria are not convex, and the broadest conditions known for the set of Stackelberg equilibria to be additionally is that $\util[\outer], \util[\inner], \constr[1], \hdots, \constr[\numconstrs]$ are all affine. \cite{} \deni{Corollary of thm 3.1 of Dempe + convex optimization's solutions being convex property}



\section{Stochastic Stackelberg Games}


\if 0
\begin{itemize}
    \item A discrete set of states $\states$, such that each $\state \in \states$ describes the state in which the game is.
    \item A continuous set of actions $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ for the $\outer$- and $\inner$- players respectively, which denote the actions the players can take throughout the game.
    \item An initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
    \item A reward function $\reward[\outer]: \states \times \outerset \times \innerset \to \R$ (resp. $\reward[\inner]: \states \times \outerset \times \innerset \to \R$) which takes as input the state of the game, the actions of the players, and outputs a reward for the outer (inner) player.
    \item A constraint function $\constr: \states \times \outerset \times \innerset \to \R^\numconstrs$ which denotes the constraints the players' actions have to satisfy in each state. In particular, for each state $\state \in \states$, we require that $(\outer, \inner) \in \outerset \times \innerset$ be picked such that $\constr(\state, \outer, \inner) \geq \zeros$.
    \item A transition function $\trans: \states \times \states \times \outerset \times \innerset \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when actions $\outer \in \outerset$ and $\inner \in \innerset$ are played by the inner and outer player respectively, is denoted by $\trans(\state^\prime \mid \state, \outer, \inner)$.
    \item A discount rate $\discount \in [0,1)$, which can be understood as the probability that the game will continue after an action is played by any player
\end{itemize}
\fi
% We denote a stochastic min-max Stackelberg game by a tuple .



A \mydef{stochastic Stackelberg game} $(\states, \outerset, \innerset, \initstates, \reward[\outer], \reward[\inner], \constr, \trans, \discount)$ is a dynamic two-player sequential, i.e., Stackelberg, game where one player we call the outer- or $\outer$-player  (resp. inner- or $\inner$-player) (or outer and inner players respectively) moves through a set of states $\states$ picking an action to play from their continuous set of actions $\outerset \subset \R^\outerdim$ ($\innerset \subset \R^\innerdim$). Players start the game at an initial state determined by an initial state distribution $\initstates: \states \to [0, 1]$ such that for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$. At each state the action $\outer \in \outerset$ picked by outer player determines the set of \mydef{feasible} actions $\inner \in \innerset$ such that $\constrs(\outer, \inner)$ that the inner player can in turn play. Once the outer and inner players made their moves they receive rewards $\reward[\outer]: \outerset \times \innerset \to \R$ and $\reward[\inner]: \outerset \times \innerset \to \R$ respectively, then the game either ends with probability $(1-\discount)$, where $\discount \in (0,1)$ is called the \mydef{discount rate}, or transitions to a new state $\state^\prime \in \states$ according to a \mydef{transition} probability function $\trans: \states \times \states \times \outerset \times \innerset \to [0,1]$ such that the probability of transitioning to state $\state^\prime \in \states$, from state $\state \in \states$, when actions $\outer \in \outerset$ and $\inner \in \innerset$ are played by the inner and outer player respectively, is denoted by $\trans(\state^\prime \mid \state, \outer, \inner)$.  

The goal of the outer (resp. inner) player is to pick an action at each state given by a \mydef{policy}, i.e., a mapping from states to pobability distributions over actions $\policy[\outer]: \states \to \Delta(\outerset)$ (resp. $\policy[\inner]: \states \to \simplex(\innerset)$) which maximizes their cumulative expected reward.\footnote{We focus on deterministic policies over continuous action spaces which maximizes their cumulative expected reward. A special case of our setting is stochastic policies over discrete action spaces for Stackelberg games with bilinear payoffs.} 
The cumulative reward function for any player $\player \in \players$, $\cumul[\player]: \outerset^\states \times \innerset^\states \to \R$ denotes the total expected reward of the player for given policies of the players and is given by:
\begin{align}
    \cumul[\player](\policy[\outer], \policy[\inner]) = \mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\outer]( \staterv[\iter]), \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]) \right]
\end{align}
For simplicity, we will denote the expected reward for at a particular state under a policy profile $(\policy[\outer], \policy[\inner])$: $$\int_{(\outer,\inner) \in \outerset \times \innerset}  \reward[\player]\left(\state, \outer, \inner\right) d\policy[\outer](\state) d\policy[\inner](\state)$$ simply by $\reward[\player](\state, \policy[\outer](\state), \policy[\inner](\state))$. 
% An \mydef{outcome} of a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ is a policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ consisting of policies for the outer and inner players respectively. 
We require any policy profile $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ to be \mydef{feasible}, i.e.,  for all states $\state \in  \states$, and for all actions $(\outer, \inner) \in \outerset \times \innerset$ such that $(\policy[\outer](\state))(\outer) (\policy[\inner](\state))(\inner) > 0$, we require $\constr(\state, \outer, \inner) \geq 0$. For simplicity, we define $\constrs : \simplex(\outerset)^\states \times \simplex(\innerset)^\states \to \R^{\states \times \outerset \times \innerset \times \numconstrs}$ such that $\constrs(\policy[\outer], \policy[\inner]) = ((\policy[\outer](\state))(\outer) (\policy[\inner](\state))(\inner) \constr(\state, \outer, \inner))_{\state, \outer, \inner}$, and define feasible outcomes as those $(\policy[\outer], \policy[\inner]) \in  \outerset^\states \times \innerset^\states$ such that $\constrs(\policy[\outer], \policy[\inner]) \geq \zeros$\deni{To improve.}. We define the best response \emph{policy} correspondence of the inner player as $\br(\policy[\outer]) = \argmax_{\policy[\inner] \in \simplex(\innerset)^\states : \constrs(\policy[\outer], \policy[\inner]) \geq \zeros} \cumul[\inner](\policy[\outer], \policy[\inner])$.\footnote{Although the notation for the best-response action  and best-response policy correspondences coincide, the reader can distinguish the two from context and input types to the correspondences.} The relevant solution concept for stochastic Stackelberg games is the \mydef{Stackelberg equilibrium}.

\begin{definition}
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \outerset^\states \times \innerset^\states$ is a Stackelberg equilibrium of a stochastic Stackelberg game iff 
\begin{align}
    \cumul[\outer](\policy[\outer]^*, \policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer])} \cumul[\outer](\policy[\outer], \policy[\inner]) && \forall \policy[\outer] \in \simplex(\outerset)^\states\\
    \cumul[\inner](\policy[\outer]^*, \policy[\inner]^*) \geq \cumul[\outer](\policy[\outer]^*, \policy[\inner]) 
    && \forall  \policy[\inner] \in \simplex(\innerset)^\states  \text{ s.t. } \constrs(\policy[\outer]^*, \policy[\inner]) \geq \zeros
\end{align}
\end{definition}
%
\noindent
% \sadie{Should this be $\policy[\outer]^*\in \argmin \max$ and $\policy[\inner]^* \in \argmax$? And why we use $g$ instead of $G$ here?}
\begin{remark}
We note that this is a stronger definition of a Stackelberg equilibrium then is required since we require the constraints $\constr(\state, \policy[\outer], \policy[\inner]) \geq \zeros$ to be satisfied for all states $\state \in \states$. Technically, at a Stackelberg equilibrium it would be enough for the constraints to be satisfied only for states which have a strictly positive probability of being reached by the strategy profile. 
% However, since the game is Markovian, i.e., the transition probabilities and reward function only depend on the current state and action, the actions outputted for states reached by the Stackelberg equilibrium policies with a strictly positive probability are the same under both definitions.
\amy{writing unclear to me}\deni{Fixed!}
\end{remark}

The results we derive in the rest of this paper rely on the two set of assumptions which apply to general-sum and zero-sum settings respectively.
\begin{assumption}\label{assum:stackelberg_general_sum}
1.~$\outerset$ and $\innerset$ are convex 
2.~for all $\outer \in \outerset$, $\util[\inner](\outer, \ \cdot \ ), \constr[1](\outer, \inner ), \hdots, \constr[\numconstrs](\outer, \ \cdot \ )$ are concave, and 
3.~for all $\inner \in \innerset$ $\util[\outer]$ is concave in $\inner$,
4.~with $\reward$ bounded, i.e., $\left\|\reward\right\|_{\infty} \leq \rewardbound < \infty$.
\end{assumption}

\begin{assumption}\label{assum:main}
1.~$\outerset$ and $\innerset$ are convex
2.~For all states $\state \in \states$, $\reward(\state, \cdot, \cdot), \constr[1](\state, \cdot, \cdot), \ldots, \constr[\numconstrs](\state, \cdot, \cdot)$ are continuous and convex-concave;
3.~(Slater's condition) $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\state, \outer, \widehat{\inner}) > 0$, for all $\numconstr = 1, \ldots, \numconstrs$, and
4.~with $\reward$ bounded, i.e., $\left\|\reward\right\|_{\infty} \leq \rewardbound < \infty$.
\end{assumption}


We now define the state-value and action-value functions and analyze their properties. These results will then be used to prove existence of Stackelberg equilibria and the convergence of algorithms to Stackelberg equilibria.

The \mydef{action value function} for each player $\player \in \players$, $\actionvalue[][][][\player]: \states \times \outerset \times \innerset \to \R$, is defined as:
\begin{align}\label{eq:action_value}
    \actionvalue[][][][\player](\state, \outer, \inner; \policy[\outer], \policy[\inner]) = \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty (1- \discount) \discount^\iter \reward[\inner](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\player]( \staterv[\iter]),  \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]), \right. \notag \\ \left. \staterv[0] = \state, \outerrv[0] = \outer, \innerrv[0] = \inner \right]
\end{align}

The \mydef{state-value function} for each player $\player \in \players$, $\statevalue[][][][\player]: \states \times \outerset^\states \times \innerset^\states \to \R$, is given by:
\begin{align}\label{eq:state_value}
    \statevalue[][][][\player](\state; \policy[\outer], \policy[\inner] ) &= \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])}\left[\sum_{\iter = 0}^\infty (1- \discount)\discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] \sim \policy[\outer]( \staterv[\iter]), \innerrv[\iter] \sim \policy[\inner](\staterv[\iter]), \staterv[0] = \state \right]\\
    &= \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state); \policy[\outer], \policy[\inner])
\end{align}
\sadie{Do you think we can adopt the notation  $\E^{\policy[]}$ in the note to indicate the expected value given we act according to $\policy[]$. For example, $\statevalue(\state; \policy[\outer], \policy[\inner] ) = \mathop{\E}_{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter])} ^{\policy[\outer]\policy[\inner]}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward(\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \staterv[0] = \state \right]$? Will this make the notations more concise?}
% \sadie{For the part under $\E$, should that be $\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \outerrv[\iter], \innerrv[\iter])$?}
For clarity, we will often denote the state value and action value function by $\statevalue[][{\policy[\outer]}][{ \policy[\inner]}](\state)$ and $\actionvalue[][{\policy[\outer]}][{ \policy[\inner]}](\state, \outer, \inner)$ respectively. Additionally, we denote $\statevalfuncs  = [-\rewardbound, \rewardbound]^{2 \times \states}$ as the the space of all state value functions of the form $\statevalue: \states \to [-\rewardbound, \rewardbound]^2$, and $\actionvalfuncs = [-\rewardbound, \rewardbound]^{2 \times \times \states \times \outerset \times \innerset}$ as the space of all action value functions $\actionvalue: \states \times \outerset \times \innerset \to [-\rewardbound, \rewardbound]^2$. Note that by \Cref{assum:main} the range of the state and action value functions are $[-\rewardbound, \rewardbound]$.

\if 0
The cumulative reward function for any player $\player \in \players$, $\cumul[\player]: \outerset^\states \times \innerset^\states \to \R$ denotes the total expected reward of the player for given policies of the players and is given by:
\begin{align}
    \cumul[\player](\policy[\outer], \policy[\inner]) = \mathop{\E}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \outerrv[\iter], \innerrv[\iter]) \\ \staterv[0] \sim \initstates}}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \outerrv[\iter], \innerrv[\iter]) \mid \outerrv[\iter] = \policy[\outer]( \staterv[\iter]), \innerrv[\iter] = \policy[\inner](\staterv[\iter]) \right]
\end{align}
\fi
% For any policy of the outer player $\policy[\outer] \in \outerset$, we define the best-response set of the inner player as $\br(\policy[\outer]) = \argmax_{\policy[\inner] \in \innerset^\states : \constrs(\policy[\outer], \policy[\inner]) \geq \zeros} \cumul[\inner](\policy[\outer], \policy[\inner])$.

We first note the following fundamental relationship between the state-value and action-value functions which is an analog of Bellman’s Theorem \cite{} and which follows from the definitions of \crefrange{eq:state_value}{eq:action_value}:
\begin{theorem}
Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, for all $\player \in \players$, $\statevalue \in \statevalfuncs$, $\actionvalue \in \actionvalfuncs$, $\policy[\outer] \in \outerset^\states$, and $\policy[\inner] \in \innerset^\states$, $\statevalue[][][][\player] = \statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$ 
% \amy{$\statevalue(\state) = \statevalue(\state ;  \policy[\outer], \policy[\inner]) $}
and $\actionvalue[][][][\player] = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$ iff:
\begin{align}
    &\statevalue[][][][\player](\state) = \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state))\label{eq:belman_q_to_v}\\
    &\actionvalue[][][][\player](\state, \outer, \inner) = (1 - \discount) \reward[\player](\state, \outer, \inner) + \discount \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[    \statevalue[][][][\player](\staterv^\prime)  \right] \label{eq:belman_v_to_q}
\end{align}
\end{theorem}

\begin{proof}
By the definition of the state value function we have $\statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player] = \actionvalue[][][][\player](\state, \policy[\outer](\state), \policy[\inner](\state))$, hence by \Cref{eq:belman_q_to_v} we must have that $\statevalue[][][][\player] = \statevalue[][{\policy[\outer]}][{\policy[\inner]}][\player]$. Additionally, by \Cref{eq:belman_v_to_q} and the definition of the action-value functions this also implies that $\actionvalue[][][][\player](\state, \outer, \inner) = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\player](\state, \outer, \inner)$
\end{proof}
% \amy{add proof}
A stronger equilibrium concept for stochastic min-max Stackelberg games would be one that would require that the strategy profile be a Stackelberg equilibrium of each subgame of the stochastic min-max Stackelberg game, aptly called subgame perfect Stackelberg equilibrium. a feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a \mydef{Markov perfect Stackelberg equilibrium} of a stochastic Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward[\outer], \reward[\inner], \constr, \trans, \discount)$ if for all $\state \in \states, \iter \in \N, \statedist[\iter+1](\state) = \sum_{\state^\prime \in \states} \trans(\state \mid \state^\prime, \policy[\outer]^*(\state^\prime), \policy[\inner]^*(\state^\prime)) \statedist[\iter ](\state^\prime)$, $(\policy[\outer]^*, \policy[\inner]^*)$ is a Stackelberg equilibrium of $(\states, \outerset, \innerset, \statedist[\iter], \reward[\outer], \reward[\inner], \constr, \trans, \discount)$. By definition, the set of Markov perfect Stackelberg equilibria of a stochastic min-max Stackelberg game is a subset of the set of Stackelberg equilibria of the game. However, it is not directly clear whether if the inclusion holds the other way round as well. 


\begin{theorem}\label{thm:equiv_def_stackelberg}
A feasible policy profile $(\policy[\outer]^*, \policy[\inner]^*) \in \states^\outerset \times \states^\innerset$ is a Stackelberg equilibrium of a stochastic Stackelberg game  $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ iff for all $\state \in \states$ :
\begin{align}
    \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\state) \geq \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner) && \forall \outer \in \outerset \\
    \statevalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\inner](\state) \geq \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\inner](\policy[\outer]^*(\state), \inner)
    && \forall  \inner \in \innerset  \text{ s.t. } \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros
\end{align}
\end{theorem}
% \sadie{for the constraint, should we do $\constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros$ and $\constr(\state, \outer, \inner) \geq \zeros?$}\deni{Fixed, does it look good now?}\sadie{It looks good to me!}
\begin{proof}
($\leftarrow$):
We prove the first inequality, the right hand side follow similarly. For all states $\state \in \states$, we have:
\begin{align}
    \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner) && \forall \outer \in \outerset\\
    \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \sum_{\state \in \states} \initstates[  ](\state) \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]^*}][\outer](\outer, \inner)  && \forall \outer \in \outerset \\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\sum_{\state \in \states} \initstates[  ](\state)  \actionvalue[][{\policy[\outer]^*}][{\policy[\inner]}][\outer](\outer, \policy[\inner](\state))  && \forall \outer \in \outerset\\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\sum_{\state \in \states} \initstates[  ](\state)  \actionvalue[][{\policy[\outer]}][{\policy[\inner]}][\outer](\policy[\outer](\state), \policy[\inner](\state))  && \forall \policy[\outer] \in \outerset^\states \\
    \cumul[\outer](\policy[\outer]^*,\policy[\inner]^*) \geq \max_{\policy[\inner] \in \br(\policy[\outer]^*) }\cumul(\policy[\outer], \policy[\inner]) && \forall \policy[\outer] \in \outerset^\states 
\end{align}

% \begin{align}
%     \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) \geq \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner)  \\
%     % \max_{\policy[\inner] \in \states^\innerset : \constr(\state, \policy[\outer]^*(\state), \policy[\inner](\state)) \geq 0}
%     \sum_{\state \in \states} \initstates[  ](\state) \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \sum_{\state \in \states} \initstates[  ](\state) \max_{\policy[\inner] \in \states^\innerset : \constr(\state, \policy[\outer]^*(\state), \policy[\inner](\state)) \geq 0} \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]}] \left(\state\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \max_{\policy[\inner] \in \states^\innerset : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros} \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]}] \left(\state\right) 
%     \leq \sum_{\state \in \states} \initstates[  ](\state) \statevalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}](\state)
%     \\
%     \max_{\policy[\inner] \in \states^\innerset : \constrs( \policy[\outer]^*, \policy[\inner]) \geq \zeros}  \cumul \left( \policy[\outer]^*, \policy[\inner] \right) 
%     \leq \cumul \left( \policy[\outer]^*, \policy[\inner]^* \right)  
% \end{align}
% Similarly, for the right hand side inequality, for all states $\state \in \states$ we have:
% \begin{align}
%     \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)  \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)
% \end{align}
($\rightarrow$): We prove the first inequality, the right-hand side follows similarly.
\begin{align}
    \policy[\outer]^* &\in \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \cumul[\outer](\policy[\outer], \policy[\inner]) \\
    &\in  \sum_{\state \in \states} \initstates[  ](\state) \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \statevalue[][{\policy[\outer]}][{ \policy[\inner]}] \left(\state\right) \\
    &\in  \argmax_{\policy[\outer] \in \outerset^\states} \max_{\policy[\inner] \in \br(\policy[\outer])} \statevalue[][{\policy[\outer]}][{ \policy[\inner]}] \left(\state\right)
\end{align}
where the second line follows from the Markovian property of the game which ensures that the optimal action in a particular state is independent of the actions taken in other states.
Re-stating the above in terms of action-value function, we get for all states $\state \in \states$:
\begin{align}
    \policy[\inner]^*(\state) &\in \argmax_{\outer \in \outerset} \max_{\inner \in \br(\outer)} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) 
\end{align}
% \sadie{I'm a little confused about this step. How did we transfer from $\statevalue[][][]$ to $\actionvalue[][][][]$? When we should use $\constr$ and when we should use $\constrs$?} \deni{add proposition 2.3 for us.} 
% Hence, by the definition of the maximum, we have for all states $\state \in \state$:
% \begin{align}
%     \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state),\inner\right) \leq \actionvalue[][{\policy[\outer]^*}][{ \policy[\inner]^*}] \left(\state, \policy[\outer]^*(\state), \policy[\inner]^*(\state) \right) \leq  \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state) 
% \end{align}
\end{proof}


Since the condition given in the above theorem is independent of the initial state distribution of the game, that Stackelberg equilibria are independent of the initial state distribution. As a result, for all $\initstates, {\initstates}^\prime \in [0,1]^\states$, we have that the Stackelberg equilibria of $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ and $(\states, \outerset, \innerset, {\initstates}^\prime, \reward, \constr, \trans, \discount)$ are the same. Hence, a corollary of the above theorem is that in stochastic min-max Stackelberg games, the set of Stackelberg equilibria coincides with the set of subgame perfect Stackelberg equilibria.

\begin{corollary}
The set of Stackelberg equilibria and subgame perfect Stackelberg equilibria coincide in stochastic min-max Stackelberg games.
\end{corollary}

We now move on to investigate the existence properties of Stackelberg equilibria. To this end, we first define the following operators: $\statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states]: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to \statevalfuncs$, $\actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states]: \statevalfuncs \times \outerset^\states \times \innerset^\states \to \actionvalfuncs$, and $\argval[\actionvalfuncs] : \actionvalfuncs \to \outerset^\states \times \innerset^\states$: 
\begin{align}
    \left(\statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states](\actionvalue, \policy[\outer], \policy[\inner])\right)(\state) = \actionvalue(\state, \policy[\outer](\state), \policy[\inner](\state))\label{eq:v_operator}
\end{align}

\begin{align}
    \left(\actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states](\statevalue, \policy[\outer], \policy[\inner])\right)(\state, \outer, \inner) = \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) + \discount \statevalue(\staterv^\prime) \right]\label{eq:q_operator}
\end{align}

\begin{align}
    \argval[\actionvalfuncs](\actionvalue) = \left\{(\policy[\outer]^*, \policy[\inner]^*) 
    % \in \outerset^\states \times \innerset^\states
    \mid  \forall \state,  \max_{\inner \in \innerset : \constr(\state, \policy[\outer]^*(\state), \inner) \geq \zeros}  \actionvalue[][{\policy[\outer]^*} ][{\policy[\inner]^*}](\state, \policy[\outer]^*(\state), \inner) \leq \statevalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state)  \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\state, \outer, \inner) \geq \zeros} \actionvalue[][{\policy[\outer]^*}][ {\policy[\inner]^*}](\state, \outer, \inner)\right\}
\end{align}


% \begin{theorem}
% Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, if there exists $\actionvalue \in \actionvalfuncs$, $\policy[\outer] \in \outerset^\states$, and $\policy[\inner] \in \innerset^\states$ such that
% %
% $\statevalue = \statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states](\actionvalue, \policy[\outer], \policy[\inner])$, 
% %
% $\actionvalue = \actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states](\statevalue, \policy[\outer], \policy[\inner])$,
% %
% and
% $(\policy[\outer],  \policy[\inner]) \in \argval[\actionvalfuncs](\actionvalue)$, then $(\policy[\outer]^*, \policy[\inner]^*)$ is a Stackelberg equilibrium of $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ and we have
% $\statevalue = \statevalue[][{\policy[\outer]}][{\policy[\inner]}]$, $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$.
% %  
% \end{theorem}

% \begin{proof}
% By \Crefrange{eq:v_operator}{eq:q_operator} we have for all states $\state \in \states$:
% \begin{align}
%     &\statevalue[](\state) = \actionvalue[](\state, \policy[\outer](\state), \policy[\inner](\state))\\
%     &\actionvalue[](\state, \outer, \inner) = \mathop{\E}_{\staterv^\prime \sim \trans(\cdot \mid \state, \outer, \inner)} \left[ \reward(\state, \outer, \inner) +  \discount \statevalue[](\staterv^\prime)  \right]
% \end{align}
% Therefore, by \Cref{thm:bellman}, we have that $\statevalue = \statevalue[][{\policy[\outer]}][{\policy[\inner]}]$, $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$. Additionally, by 
%  \Cref{thm:equiv_def_stackelberg} and the definition of $\argval[\actionvalfuncs](\actionvalue)$, we know that $(\policy[\outer],  \policy[\inner])$ is a Stackelberg equilibrium.
% \end{proof}

% Using the above, we construct a function $\policyfp: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to  \actionvalfuncs \times \outerset^\states \times \innerset^\states$ such that $\policyfp = \left(I \times \argval[\actionvalfuncs]\right) \circ \actionvalue[][][][\statevalfuncs \times \outerset^\states \times \innerset^\states] \circ \statevalue[][][][\actionvalfuncs \times \outerset^\states \times \innerset^\states]$ where $I$ is the identity operator. The following corollary of \Cref{thm:bellman} applies to to $\policyfp$:

% \begin{corollary}\label{corr:fp_stackelberg}
% Given a stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$, if there exists a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$, then $(\policy[\outer], \policy[\inner])$ is a Stackelberg equilibrium, and $\actionvalue = \actionvalue[][{\policy[\outer]}][{\policy[\inner]}]$.
% \end{corollary}



% \begin{lemma}
% The set of Stackelberg equilibria of any min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$ is non-empty, compact, and convex.
% \end{lemma}
% \begin{proof}
% By proposition B.2 from \cite{goktas2021minmax}, the set of Stackelberg equilibria of any min-max Stackelberg game is non-empty. Additionally, under \Cref{assum:main}, we have that for all $\outer \in \outers$, $\obj(\outer, \cdot)$ is concave, and $\{\inner \innerset \mid \constr(\outer, \inner) \geq \zeros\}$ is convex. Hence, by \cite{} the set of solutions $\outerset^*(\outer) = \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is compact- and convex- valued.
% %
% Similarly, under \Cref{assum:main}, by proposition B.1 from \cite{goktas2021minmax}, $\max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is continuous and convex. Hence, the set of solutions $\innerset^* = \argmin_{\outer \in \outerset} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is compact- and convex-valued. Since the carthesian product of two compact-convex-valued correspondences is compact-convex-valued, we have that the set of Stackelberg equilbiria $\outerset^*\left(\innerset^*\right)$ is also compact-convex-valued.
% \end{proof}

% \begin{corollary}
% The correspondence $\argval[\actionvalfuncs]$ is non-empty-, compact-, convex-valued.
% \end{corollary}

% \begin{proof}
% For any $\actionvalue \in \actionvalfuncs$ and for all states $\state \in \states$, we have that $\left( \argval[\actionvalfuncs](\actionvalue) \right)(\state)$ is the set of Stackelberg equilibria of the min-max Stackelberg game $(\outerset, \innerset, \actionvalfuncs, \constr(\state, \cdot, \cdot))$ which is non-empty-compact-convex-valued. Hence, $\argval[\actionvalfuncs](\actionvalue)$ must be non-empty-compact-convex valued as well since it is the product of multiple non-empty-compact-convex sets.
% \end{proof}

% \begin{lemma}\label{lemma:fp_existence}
% The correspondence $\policyfp$ has a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$.
% \end{lemma}
% \begin{proof}
% $\policyfp: \actionvalfuncs \times \outerset^\states \times \innerset^\states \to \actionvalfuncs \times \outerset^\states \times \innerset^\states$ is non-empty-, and convex-valued. It is also compact-valued, i.e., its graph is closed. Hence, by Kakutani's fixed point a fixed point $(\actionvalue, \policy[\outer], \policy[\inner])$ such that $(\actionvalue, \policy[\outer], \policy[\inner]) \in \policyfp(\actionvalue, \policy[\outer], \policy[\inner])$ exists.
% \end{proof}

% \amy{Deni's conjecture: we don't need to assume boundedness in zero-sum games, only in non-zero-sum games}

% Combining \Cref{lemma:fp_existence} and \Cref{corr:fp_stackelberg}, we obtain:
\begin{theorem}\label{thm:stackelberg_existence}
Any stochastic min-max Stackelberg game $(\states, \outerset, \innerset, \initstates, \reward, \constr, \trans, \discount)$ has at least one Stackelberg equilibrium 
\end{theorem}

\begin{proof}
Let $\calK = \statevalfuncs \times \simplex(\outerset)^\states \times \simplex(\innerset)^\states$.  Note that since $\calK$ is a carthesian product of compact convex sets, it is also compact convex set (of a locally convex space).
Consider a correspondence $\fp: \left(\v, \policy[\outer], \policy[\inner] \right) \in \left(\calK \right) \rightrightarrows (\w(\v, \policy[\outer], \policy[\inner]), \phi(\v, \policy[\outer], \policy[\inner])))$ where $\w, \phi$ are defined respectively as:

\begin{align}
    w_\outer\left(\v, \policy[\outer], \policy[\inner] \right)(\state) = \max_{\policy \in \simplex(\outerset)^\states} \left[  \reward[\outer](\state, \policy(\state), \policy[\inner](\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy(\state) d\policy[\inner](\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states\\
    w_\inner\left(\v, \policy[\outer], \policy[\inner] \right)(\state) = \max_{\policy \in \simplex(\innerset)^\states : \constrs(\policy[\outer], \policy) \geq \zeros} \left[  \reward[\inner](\state, \policy[\outer](\state), \policy(\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy[\outer](\state) d\policy[](\state)  \statevalue[][][][\inner](\state^\prime)\right] && \forall \state \in \states\\\
    \phi_\outer(\v, \policy[\outer], \policy[\inner])(\state) = \argmax_{\policy \in \simplex(\outerset)^\states} \left[  \reward[\outer](\state, \policy(\state), \policy[\inner](\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy(\state) d\policy[\inner](\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states\\
    \phi_\inner(\v, \policy[\outer], \policy[\inner])(\state) = \argmax_{\policy \in \br(\policy[\outer])} \left[  \reward[\outer](\state, \policy[\outer](\state), \policy(\state)) + \sum_{\state^\prime \in \states} \int_{\outerset \times \innerset} \trans(\state^\prime \mid \state, \outer, \inner) d\policy[\outer](\state) d\policy(\state) \statevalue[][][][\outer](\state^\prime)\right] && \forall \state \in \states
\end{align}

Note that the objective of all of the optimization problems above are linear in their inputs since they are the sum of two expectations. Hence, by \Cref{assum:stackelberg_general_sum} since $\constr(\state, \outer, \inner)$ is convex in $\inner$ for all $\state \in \states$, Berge's maximum theorem  \cite{berge1997topological} applies and we have that $\w\left(\v, \policy[\outer], \policy[\inner] \right)$ is continuous. Similarly, since $\simplex(\outerset)^\states$ is compact, by Berge's maximum theorem $\phi_\outer$ is upper hemicontinuous and convex-valued.

Note that by Berge's maximum theorem under \Cref{assum:stackelberg_general_sum}, $\br$ is upper hemicontinuous, and nonempty-compact valued.
Hence, by theorem 4.2.1 of \citeauthor{bank1983non} \cite{bank1983non} since the best-response correspondence is upper hemicontinuous and the marginal function of the outer player is upper semicontinuous, $\phi_\outer$ must be upper hemicontinuous.

Hence, by Kakutani's fixed point theorem a fixed point of $\fp$ exists.
% \begin{align}
% \fp
% \begin{pmatrix}
%     \statevalue[][][][\outer]\\
%     \statevalue[][][][\inner]\\
%     \policy[\outer]\\
%     \policy[\inner]
% \end{pmatrix}
% =
% \begin{pmatrix}
%     \max_{\policy \in \simplex(\outerset)^\states} \left\{ \reward(\state) \right\}\\
%     \statevalue[][][][\inner]\\
%     \policy[\outer]\\
%     \policy[\inner]
% \end{pmatrix}
% \end{align}
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> todo.tex <==
% Outline:
% \begin{itemize}
%     \item Intro 
%     \item Preliminaries
%     \item Generalized Stackelberg games existence + Arrow-Debreu exchange markets equivalence with markets
%     \item Stochastic Generalized Stackelberg Games, existence + computation via VI
%     \item Recursive Arrow-Debreu Markets, existence + computation via VI for Recursive Fisher markets
%     \item Experiments: Convergence rates
%     \item Conclusion
% \end{itemize}

==> zerosum.tex <==



